Leximin Approximation: From Single-Objective to Multi-Objective

Leximin is a common approach to multi-objective optimization, frequently employed in fair division applications. In leximin optimization, one first aims to maximize the smallest objective value; subject to this, one maximizes the second-smallest objective; and so on. Often, even the single-objective problem of maximizing the smallest value cannot be solved accurately. What can we hope to accomplish for leximin optimization in this situation? Recently, Henzinger et al. (2022) defined a notion of \emph{approximate} leximin optimality. Their definition, however, considers only an additive approximation. In this work, we first define the notion of approximate leximin optimality, allowing both multiplicative and additive errors. We then show how to compute, in polynomial time, such an approximate leximin solution, using an oracle that finds an approximation to a single-objective problem. The approximation factors of the algorithms are closely related: an $(\alpha,\epsilon)$-approximation for the single-objective problem (where $\alpha \in (0,1]$ and $\epsilon \geq 0$ are the multiplicative and additive factors respectively) translates into an $\left(\frac{\alpha^2}{1-\alpha + \alpha^2}, \frac{\epsilon}{1-\alpha +\alpha^2}\right)$-approximation for the multi-objective leximin problem, regardless of the number of objectives.

==> files/abs-prev-2304.tex <==

\begin{abstract}
Leximin is a common approach to multi-objective optimization,
frequently employed in fair division applications.
In leximin optimization, one first aims to maximize the smallest objective value; subject to this, one maximizes the second-smallest objective; and so on. 
Often, even the single-objective problem of maximizing the smallest value cannot be solved accurately, e.g. due to computational hardness. 
What can we hope to accomplish for leximin optimization in this situation?
Recently, Henzinger et al (2022) defined a notion of \emph{approximate} leximin optimality, and showed how it can be computed for the problem of representative cohort selection. 
However, their definition considers only an additive approximation in the single-objective problem.

In this work, we define approximate leximin optimality allowing approximations that have multiplicative and additive errors. 
We show how to compute a solution that approximates leximin in polynomial time, using an oracle that finds an approximation to the single-objective problem.  
The approximation factors of the algorithms are closely related: a factor of $(\multApprox,\additiveApprox)$ for the single-objective problem (where $\multApprox$ and $\additiveApprox$ describe the multiplicative and additive factors respectively) translates into a factor of $\left(\frac{\multApprox^2}{1-\multApprox + \multApprox^2}, \frac{\multApprox(2-\multApprox)\additiveApprox}{1-\multApprox +\multApprox^2}\right)$ for the multi-objective leximin problem, regardless of the number of objectives. 
\eden{I combined between the paragraphs because APPROX requires 2-paragraphs}
As a usage example, we apply our algorithm to the problem of \emph{stochastic allocations of indivisible goods}.  
For this problem, assuming sub-modular objectives functions, the single-objective egalitarian welfare can be approximated, with only a multiplicative error, to an optimal $1-\frac{1}{e}\approx 0.632$ factor w.h.p.
We show how to extend the approximation to leximin, over all the objective functions, to a multiplicative factor of $\frac{(e-1)^2}{e^2-e+1} \approx 0.52$ 
w.h.p or $\frac{1}{3}$ deterministically. 
\end{abstract}

==> files/abs-to-sub.tex <==

\begin{abstract}
Leximin is a common approach to multi-objective optimization, frequently employed in fair division applications. In leximin optimization, one first aims to maximize the smallest objective value; subject to this, one maximizes the second-smallest objective; and so on.  Often, even the single-objective problem of maximizing the smallest value cannot be solved accurately.  What can we hope to accomplish for leximin optimization in this situation? Recently, Henzinger et al. (2022) defined a notion of \emph{approximate} leximin optimality. Their definition, however, considers only an additive approximation.   

In this work, we first define the notion of approximate leximin optimality, allowing both multiplicative and additive errors. We then show how to compute, in polynomial time, such an approximate leximin solution, using an oracle that finds an approximation to a single-objective problem. The approximation factors of the algorithms are closely related: an $(\alpha,\epsilon)$-approximation for the single-objective problem (where $\alpha \in (0,1]$ and $\epsilon \geq 0$ are the multiplicative and additive factors respectively) translates into an $\left(\frac{\alpha^2}{1-\alpha + \alpha^2}, \frac{\epsilon}{1-\alpha +\alpha^2}\right)$-approximation for the multi-objective leximin problem, regardless of the number of objectives. 

Finally, we apply our algorithm to obtain an approximate leximin solution for the problem of \emph{stochastic allocations of indivisible goods}. For this problem, assuming sub-modular objectives functions, the single-objective egalitarian welfare can be approximated, with only a multiplicative error, to an optimal $1-\frac{1}{e}\approx 0.632$ factor w.h.p. We show how to extend the approximation to leximin, over all the objective functions, to a multiplicative factor of $\frac{(e-1)^2}{e^2-e+1} \approx 0.52$ w.h.p or $\frac{1}{3}$ deterministically.
\end{abstract}


==> files/algo-rand.tex <==
\subsection{Randomized Approximation Algorithms}
\eden{TO myself: maybe to add motivation...}
Another question is what happens when we consider approximation procedures that are also randomized?
We saw that if \textsf{OP} is a $(1-\beta)$ approximation algorithm to \eqref{eq:vsums-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-1-\frac{\beta}{1-\beta +\beta^2})$ approximately-optimal solution.
If \textsf{OP} is a $(1-\beta)$ approximation algorithm to \eqref{eq:vsums-OP} that s

So, using an approximate solver to \eqref{eq:vsums-OP}, what guarantee can we provide for the overall resulting solution? 
\begin{theorem}
\label{th:main}
Let $\beta<1/2$, and \textsf{OP} be a procedure that outputs a $(1-\beta)$ approximation to \eqref{eq:vsums-OP}. Then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-\frac{\beta}{1-\beta +\beta^2})$-approximate Leximin solution.  
\end{theorem}

==> files/app.tex <==

\section{Stochastic Allocations of Indivisible Goods}\label{sec:app}
% title: what is the purpose of this section
In this section, we consider a particular application of our results, for the problem of \textit{stochastic allocations of indivisible goods}. 
We prove that, under the setting described bellow, a leximin approximation with \emph{only} a multiplicative error can be obtained in polynomial time.
Specifically, we prove that a $\frac{1}{3}$-approximation\footnote{This section discusses only multiplicative approximations; so, for brevity, we use the term "$\multApprox$-approximation" to refer to "$(\multApprox,0)$-approximation".} can be obtained deterministically, whereas a $\frac{(e-1)^2}{e^2-e+1} \approx 0.52$-approximation can be obtained w.h.p.
As a reference point, it is worth noting that the problem of maximizing the egalitarian welfare in the same settings has been shown to be NP-hard to approximate to a (multiplicative) factor better than $1-\frac{1}{e} \approx 0.632$~\cite{kawase_max-min_2020}.
% \eden{should we say, as \textcite{kawase_max-min_2020}, that given an approximation algorithm with a multiplicative error of $\multError$ for welfare maximization, we obtain a approximate leximin with a multiplicative error of $\frac{\multError}{1-\multError +\multError^2}$?}.
However, as an $\multApprox$-approximation to leximin is first and foremost an $\multApprox$-approximation to the egalitarian welfare\displayEcai{\footnote{See Observation \ref{obs:rppeox-lex-generalizes-approx-egal}.}}, the same hardness result applies to our problem as well.


% title: basic model  
The setting postulates a set of $n$ agents $1,\ldots,n,$ and $m$ items, $1,\ldots,m,$ to be distributed amongst the agents.
A \emph{deterministic allocation} of the items to the agents is a mapping $A:[m]\rightarrow [n]$, determining which agent gets each item.
Note that as the term "deterministic" is used in this section also when discussing algorithms, we will use the term \emph{simple allocation} from now on.
% Given an allocation $A$, we denote by $A_i=A^{-1}(i)$ - the set of items allocated to $i$ in $A$. 
We denote by $\mathcal{A}$ the set of simple allocations. 
Each agent $j$ is associated with a function $u_j \colon \mathcal{A} \to \mathbb{R}_{\geq 0}$ that describes its utility from a simple allocation.

A \emph{stochastic allocation}, $d$, is a distribution over the simple allocations.  The set of all possible stochastic allocations is: 
\begin{align*}
    \mathcal{D} = \{d \mid p_d \colon \mathcal{A} \to [0,1], \sum_{A \in \mathcal{A}} p_d(A) = 1\}
\end{align*}  
\displayComsoc{
\eden{I'm not sure whether to move the formal definitions to the appendix (if so, where?) or to omit them.}
Agents are assumed to assign a positive utility to the set of all items and to care only about their own share (allowing us to use the following abuse of notation in which $u_j$ takes a bundle $b$ of items). 
Their utilities are assumed to be normalized ($u_j(\emptyset) = 0$), monotone ($u_j(b_1) \leq u_j(b_2)$ if $b_1 \subseteq b_2$), and submodular ($u_j(b_1) + u_j(b_2) \geq u_j(b_1 \cup b_2) + u_j(b_1 \cap b_2)$ for any bundles $b_1,b_2$); and to be given in the \emph{value oracle model} --- that is, we do not have a direct access to them, but only to an oracle that indicates the value of an agent from a given simple allocation.
}
\displayEcai{
Agents are assumed to care only about their own share (allowing us to use the following abuse of notation in which $u_j$ takes a bundle $b$ of items), their utilities are assumed to be normalized ($u_j(\emptyset) = 0$), monotone ($u_j(b_1) \leq u_j(b_2)$ if $b_1 \subseteq b_2$), and submodular ($u_j(b_1) + u_j(b_2) \geq u_j(b_1 \cup b_2) + u_j(b_1 \cap b_2)$ for any bundles $b_1,b_2$).
It is assumed that each agent assigns a positive utility to the set of all items.
The utilities $(u_i)_{i=1}^n$ are assumed to be given in the \emph{value oracle model}, meaning that we do not have a direct access to them, but only to an oracle that indicates the value of an agent from a given simple allocation.
}
% \eden{z1 > 0}
Lastly, the agents are assumed to be risk-neutral. This means that, given a stochastic allocation $d$, the utility of each agent $j$ is given by the expected value:
\begin{align*}
	E_j(d) = \sum_{A\in \mathcal{A}}p_d(A)\cdot u_j(A).
\end{align*}
The goal is to find a stochastic allocation that maximizes the set of functions $E_1,\ldots,E_n$. 
Formally, we consider the following problem:
\begin{align*}
	\lexmaxmin \quad &\{E_1(d), E_2(x), \dots E_n(d)\} \\
	s.t. \quad  & d \in \mathcal{D}
\end{align*}
% \eden{maybe $\maxlexmin$?} 
That is, the feasible region is the set of stochastic allocations ($S = \mathcal{D}$) and the objective functions are the expected utilities ($f_i = E_i$ for any $i\in [N]$).


% \begin{lemma}
%     If a solution is an $\multApprox$-approximation to leximin, then it is also an $\multApprox$-approximation to the egalitarian welfare.
% \end{lemma}

% \eden{I removed the proof for now due to lack of space}
% \begin{proof}
%     Let $d \in \mathcal{D}$ be a stochastic allocation, and assume that it is an $\multApprox$-approximation to leximin. 
%     By definition, there is no solution that is $(\multApprox,0)$-preferred over it --- $d' \nAlphaBetaPreferredParams{\multApprox}{0} d$ for any $d' \in \mathcal{D}$.
%     Suppose by contradiction that $d$ is \emph{not} an $\multApprox$-approximation to the egalitarian welfare, and let $d^*$ be the optimal solution to this problem.
%     This means that the smallest objective value of $d'$ is less than smallest objective value of $d^*$ times $\multApprox$ --- $\valBy{1}{d} < \multApprox \cdot\valBy{1}{d^*}$.
%     But it follows that $d^*\alphaBetaPreferredParams{\multApprox}{0} d $;
%     for $k=1$, the required for $j<k$ is vacuously true 
%     and $\valBy{1}{d^*} > \frac{1}{\multApprox}\valBy{1}{d}$.
%     However, we know that the $d' \nAlphaBetaPreferredParams{\multApprox}{0} d$ for any $d' \in \mathcal{D}$, so it is true in particular for $d^*$. This is a contradiction.
% \end{proof}
% As the proof is straightforward, it is omitted.


Kawase and Sumita~\cite{kawase_max-min_2020} present an approximation algorithm, which relates the problem of finding a stochastic allocation that approximates the egalitarian welfare, to the problem of finding a \emph{simple} allocation that approximates the \emph{utilitarian welfare} 
(i.e., the sum of utilities):
\begin{align*}
 \max \quad &\sum_{i=1}^n u_i(A)   \;\;
        \quad s.t. \quad   A \in \mathcal{A}.
        \tag{U1}\label{eq:utilitarian}
\end{align*}
% \erel{Can you write the maximization problem for utilitarian welfare?}

We adapt their algorithm to find an approximately leximin-optimal allocation as follows:
\begin{theorem}
\label{th:app-main}
Given a (randomized) algorithm that returns a simple allocation that $\multApprox$-approximates the utilitarian welfare (with success probability $p$).
Then, Algorithm \ref{alg:basic-ordered-Outcomes} can be used to obtain a $ \frac{\multApprox^2}{1-\multApprox +\multApprox^2}$-leximin-approximation for the problem of stochastic allocations (with the same probability).
% \eden{previous version: Then, Algorithm \ref{alg:basic-ordered-Outcomes} can be used to obtain a stochastic allocation that approximates leximin with a multiplicative error of at most $\frac{\multError}{1-\multError +\multError^2}$ (with the same probability).}
\end{theorem}

A complete proof is given in Appendix \appendixName{\ref{sec:app-sec-proofs}}{C}\fullVer.
Here we provide an outline.
We start by taking \eqref{eq:vsums-OP} and replacing the constraint (\progLinear.1) with the constraints describing a feasible stochastic allocation. 
Here we face a computational challenge: the number of variables describing a stochastic allocation is exponential in the input size, as we need a variable for each simple allocation. 
We address this challenge by moving to the dual of a closely related program.
The dual has polynomially-many variables but exponentially-many constraints.
However, we prove that a randomized approximate separation-oracle for this program can be designed and used within a variant of the ellipsoid method to approximate \eqref{eq:vsums-OP}.

Theorem \ref{th:app-main} yields two immediate corollaries, using  known algorithms to approximate the utilitarian welfare when the agents' utility functions are monotone and submodular.

First, there are deterministic $\frac{1}{2}$-approximation algorithms~\cite{Buchbinder2019, Fisher1978}, and therefore:
\begin{corollary}
    Algorithm \ref{alg:basic-ordered-Outcomes} can be used to obtain a $\frac{0.5^2}{1-0.5 +0.5^2} = \frac{1}{3}$-leximin-approximation for the problem of stochastic allocations.
    % \eden{previous version: a stochastic allocation that approximates leximin with a multiplicative error at most     $\frac{0.5}{1-0.5+0.5^2} =     \frac{2}{3}$.}
\end{corollary}
\noindent Second, there is a randomized $(1-\frac{1}{e})$-approximation algorithm w.h.p~\cite{vondrak_optimal_2008}, and therefore:
\begin{corollary}
    Algorithm \ref{alg:basic-ordered-Outcomes} can be used to obtain $\frac{(1-1/e)^2}{1-(1-1/e) +(1-1/e)^2} = \frac{(e-1)^2}{e^2-e+1 }\approx 0.52$-leximin-approximation for the problem of stochastic allocations w.h.p.
    % \eden{previous version:     a stochastic allocation that approximates leximin with a multiplicative error at most $\frac{e}{e^2-e+1} \approx 0.48$ w.h.p.}
\end{corollary}

\eden{I couldn't find the reference to the thesis where the result for gross-substitutes utilities is proven, so I gave up on presenting this result}
% It should also be noted that when the utilities are gross-substitutes, there exists an exact polynomial-time algorithm for calculating utilitarian welfare~\cite{bertelsen2005substitutes,kawase_max-min_2020}. Together with Theorem \ref{th:main}, this implies that Algorithm \ref{alg:basic-ordered-Outcomes} can be used to find an exact leximin-optimal solution to the problem of stochastic allocation in this case.

% The proof of Theorem \ref{th:app-main} is provided in Appendix \ref{sec:app-sec-proofs}. 


\eden{should we say that in the case of additive and gross-substitute utilities this means that a leximin optimal solution can be found?}

% \eden{I'm not sure "with success probability" or "with \emph{a} success probability"?}







==> files/backups/algo-2202.tex <==

\section{Approximation Algorithm}\label{sec:algo-short}
We now present an algorithm for computing a multiplicative approximate leximin \eden{optimal?}. The algorithm is an adaptation of one of the algorithms of \textcite{Ogryczak_2006} for finding exact Leximin solutions. 

% \eden{yonatan}
% Following the \emph{definition} of Leximin, the core \emph{algorithm} for finding a Leximin optimal solution is interative, wherein one first maximizes the least objective function, then the second, and so forth. 
% Specifically, donating by $z_i$ the $i$-th smallest objective value, in each iteration, $t$, one seeks to maximize $z_t$, given the already calculated optimal values for $z_1,\ldots,z_{t-1}$.  The core, single-valued, optimization problem is thus:
%
% \eden{erel} 
% Following the definition of leximin, the core algorithm for finding a leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
% Denote by $z_t$ the value of the $i$-th smallest objective in the leximin-optimal solution, where $t\in\{1,\ldots,n\}$. Suppose we have already computed the optimal values $z_1,\ldots, z_{t-1}$. \eden{I'm not sure about it.. since we use the $z_t$ value later as the \textbf{approximation} value I think it could be a bit confusing}
% Then,  $z_t$ is the solution to the following single-objective optimization problem (where the variables are the scalar $z$ and the vector $x$):

\eden{how is this? I tried to combine the two versions}
Following the definition of Leximin, the core algorithm for finding a Leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
In each iteration, $t=1,\ldots,n$, it looks for the value that maximizes the $t$-th smallest objective, $z_t$, given that for any $i < t$ the $i$-th smallest objective is at least $z_i$ (the value that was computed in the $i$-th iteration).
The core, single-objective optimization problem is thus:
\begin{align}
 \max \quad &\ztVar{x}  \;\;
        s.t. &\quad  & (1) \quad x \in S  \tag{P1}\label{eq:basic-OP}\\
              &     & & (2) \quad \valBy{\ell}{x}\geq z_{\ell} & \ell = 1,\ldots,t-1\nonumber \\
               &    & & (3) \quad \valBy{t}{x} \geq \ztVar{x} \nonumber   
\end{align} 
where the variables are the scalar $\ztVar{x}$ and the vector $x$, and $z_1, \ldots z_{t-1}$ are constants.

Suppose we are given a procedure $\textsf{OP}(z_1,\ldots,z_{t-1})$, which, given  $z_1,\ldots,z_{t-1},$ outputs $(x,z)$ that is the exact optimal solution to \eqref{eq:basic-OP}.  
Then, the \emph{leximin} optimal solution is obtained by iterating this process for $t=1,\ldots,n$, as described in Algorithm \ref{alg:basic-ordered-Outcomes}.
\begin{algorithm}[!tbp]
\caption{The Ordered Outcomes Algorithm}
\label{alg:basic-ordered-Outcomes}
\begin{algorithmic}[1] %[1] enables line numbers
\FOR{$t=1$ to n}
\STATE \( %\begin{align*}
(x_t,z_t)\leftarrow \textsf{OP}(z_1,\ldots,z_{t-1})
\) %\end{align*} 
\ENDFOR
\STATE return $(z_1,\ldots,z_n)$ 
\end{algorithmic}
\end{algorithm}

However, it might be difficult to solve the problem \eqref{eq:basic-OP} as is, since constraints (2) and (3) are not linear even with respect to the objective-functions. 
\erel{I suggest to move P2-Compact here: it is a natural step between P1 and P2.}
\eden{}
 Thus, \cite{Ogryczak_2006} suggest using a variant of the problem that considers sums instead of individual values, which described as follows (similarly, the variables are $\ztVar{x}$ and $x$, and $z_1, \ldots z_{t-1}$ are constants):  
% \eden{maybe we should say it is not a linear program \textbf{with respect to the objective functions}?}
% \erel{I agree. Since the objective functions themselves may be non-linear.}
\begin{align*}
    \max \quad &\ztVar{x} \tag{P2}\label{eq:sums-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                    & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
Here, the constraints $(2)$ and $(3)$ are replaced with constraints $(\hat{2})$ and $(\hat{3})$, respectively. 
Constraint $(\hat{2})$ says that for any $\ell<t$, the sum of any $\ell$ objective functions is at least the sum of the first $\ell$ $z_i$'s. Similarly, $(\hat{3})$ says that the sum of any $t$  objective functions is at least the $t$ first $z_i$'s.  So, since we seek to maximize $z_t$, the optimal solution to \eqref{eq:sums-OP} and \eqref{eq:basic-OP} are provably identical (as in both $z_i$ is the $i$-th least objective value, see \cite{Ogryczak_2006} for a formal proof \eden{I'm actually not sure which of the papers to cite as I didn't find a formal proof (only the claim in given in \cite{Ogryczak_2006} and in \cite{Ogryczak2004TelecommunicationsND} Theorem 4)}). As such, in Algorithm \ref{alg:basic-ordered-Outcomes}, a solver for \eqref{eq:sums-OP} can be used (instead of for \eqref{eq:basic-OP}), and the algorithm will still output a Leximin optimal solution. 

Alas, while \eqref{eq:sums-OP} is linear with respect to the objective-functions, it has an exponential number of constraints. 
To overcome this problem, \cite{Ogryczak_2006} employ auxiliary variables ($y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$) to obtain a polynomial-sized program that is provably equivalent to \eqref{eq:sums-OP}:\eden{To myself: should explain "equivalent" in more detail, maybe to add the alternative proof}
% (where the variables are $\ztVar{x}$, $x$, and $y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$; and $z_1, \ldots z_{t-1}$ are constants)
\begin{align}
    \max \quad &z_t\tag{P3}\label{eq:vsums-OP}\\
        s.t. \quad  & (1) \quad x \in S \nonumber\\
                    & (2) \quad \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq \sum_{i=1}^{\ell}  z_i && \ell = 1, \ldots,t-1 \nonumber \\
                    & (3) \quad t y_t - \sum_{j=1}^{n} m_{t,j} \geq \sum_{i=1}^{t}  z_i  \nonumber \\
                    & (4) \quad m_{\ell,j} \geq y_{\ell} - f_j(x)  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber \\
                    & (5) \quad m_{\ell,j} \geq 0  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber
\end{align}
So, in Algorithm \ref{alg:basic-ordered-Outcomes} using a solver for \eqref{eq:vsums-OP}, the algorithm will output a Leximin optimal solution. 

All of the above is for exact solutions.  
The question is what happens when we consider approximation procedures? It is easy to see that if \textsf{OP} is a $(1-\beta)$ approximation algorithm to \eqref{eq:basic-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-\beta)$ approximation of the Leximin. 
\erel{
To say this, we first have to define the notion of "approximation algorithm". It is known, but we still have to define it formally. Maybe in the "preliminaries" section.
} 
However, for approximations, \eqref{eq:sums-OP}, and the equivalent \eqref{eq:vsums-OP}, are no longer equivalent to \eqref{eq:basic-OP}. Indeed, the following example shows that if \textsf{OP} is a $(1-\beta)$ approximation procedure for \eqref{eq:vsums-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} may output a solution that is \emph{not} a $1-\beta$ approximation to the Leximin.
% \erel{Maybe it is better to move the example to here, to motivate our proof.}
Consider the following multi-objective optimization problem with $n=2$:
\begin{align*}
    \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
    s.t. \quad  & x_1 \leq 100\\
                & x_1 + x_2 \leq 200\\
                & x \in \mathbb{R}^2_{+}
\end{align*}
Accordingly, the problem \eqref{eq:vsums-OP} becomes:
\begin{align*}
    \max \quad &z_t \\
    s.t. \quad  & (1.1) \quad  x_1 \leq 100\\
                & (1.2) \quad  x_1 + x_2 \leq 200\\
                & (1.3) \quad  x \in \mathbb{R}^2_{+}\\
                & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
The following is a possible run of the algorithm with \textsf{OP} that is a $(1-\beta)$ approximate solver for $\beta=0.1$. 
In the first iteration, $t=1$, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
Then, in the second iteration, $t=2$, given that $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained (for example) with  $x_1=x_2=94.5$.  
\erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}\eden{is it more clear now?}
Since $n=2$, the algorithm ends after this iteration and returns this solution $(94.5,94.5)$.
But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,105.5)\xPreferred{\frac{1}{0.9}}(94.5,94.5)$.
Therefore, by definition, the returned solution $(94.5,94.5)$ is \emph{not} a $0.9$ approximately-optimal solution.
% \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5)  \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition  $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}

 %On the other hand, \eqref{eq:vsums-OP} is the most solvable variant of the problem.  
So, using an approximate solver to \eqref{eq:vsums-OP}, what guarantee can we provide for the overall resulting solution? 
\begin{theorem}
\label{th:main}
Let $\beta<1/2$, and \textsf{OP} be a procedure that outputs a $(1-\beta)$ approximation to \eqref{eq:vsums-OP}. Then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-2\beta)$-approximate Leximin solution.  
\end{theorem}

\eden{maybe we should also include the proof of the additive variant somewhere? if so. where?}
\erel{
Since the proof is not explicitly mentioned anywhere, I think it is good to include a proof for comparison. Maybe in an appendix.
}
\eden{if we want to do so we should also describe the additive variant definition, maybe to put them both in the appendix? I added appendix \ref{sec:additive}}
The remainder of this section is dedicated to proving the theorem.
To this end, we use another equivalent representation of \eqref{eq:sums-OP}, which was also introduced by \cite{Ogryczak_2006}. 
\erel{This variant should move upwards, between P1 and P2.}
% (here also, the variables are $\ztVar{x}$ and $x$, and $z_1, \ldots z_{t-1}$ are constants)
\begin{align*}
    \max \quad &z_t \tag{P2-compact}\label{eq:compact-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\Tilde{2}) \quad \sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell}  z_i && \ell = 1,\ldots, t-1 \nonumber\\
                    & (\Tilde{3}) \quad \sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t}  z_i
\end{align*}
In this program, constraints $(\hat{2})$ and $(\hat{3})$ are replaced by  $(\Tilde{2})$ and $(\Tilde{3})$, respectively.  In  $(\hat{2})$, for each $\ell$, one gives a lower bound on the sum for \emph{any} set of $\ell$ objective functions.  In $(\Tilde{2})$, on the other hand, one only considers the sum of the $\ell$ \emph{smallest} such values.  However, since the constraints set the same lower bound on this sum, the constraints are equivalent.  Similarly for $(\hat{3})$ and $(\Tilde{3})$.  So, \eqref{eq:compact-OP} and \eqref{eq:sums-OP} are equivalent, which, in turn, is equivalent to \eqref{eq:vsums-OP}.  So, in proving the theorem we may assume that \textsf{OP} is an approximation procedure for \eqref{eq:compact-OP}.  This will simplify the proofs.

\erel{*** I do not understand. We say that P1 and P2 are equivalent with an exact solver, but not with an approximate solver. 
Here, we claim that P3 and P2-compact are equivalent, but this is true only with an exact solver. Don't we have to prove that they are equivalent also with an approximate solver? ***}

We denote $\retSol := x_n$ = the solution $x$ attained at the last iteration ($t=n$) of the algorithm.
Also, the optimal value of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$ is denoted by $\sOptT{t}$. 

Following are some observations regarding the problem \eqref{eq:compact-OP} and the solution $\retSol$ that will be useful later.
First, notice that any solution $x \in S$ that satisfies constraint $(\Tilde{2})$ of \eqref{eq:compact-OP} is feasible to this problem.
This is because any solution $x \in S$ can satisfy constraint $(\Tilde{3})$ with a small enough assignment to the variable $z_t$. \eden{I'm not sure how to explain it....}
\begin{observation}\label{obs:feasi-and-constraint2}
Any solution $x \in S$ that satisfies constraint $(\Tilde{2})$ is feasible to \eqref{eq:compact-OP}.
\end{observation}

Since $\retSol$ is a feasible solution of \eqref{eq:compact-OP} in iteration $n$, and as each
iteration only adds new constraints to $(\Tilde{2})$, it follows that $\retSol$ is also a feasible solution of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$. 
\begin{observation}\label{obs:retSol-solves-any-t}
$\retSol$ is a feasible solution of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$.
\end{observation}

Now, consider the problem \eqref{eq:compact-OP} that was solved in iteration $t$.
Here, $z_t$ is a \emph{variable} and $z_1, \ldots z_{t-1}$ are constants.
The objective of this problem is $(\max z_t)$ and the only constraint that includes the variable $z_t$ is constraint $(\Tilde{3})$.
Therefore, rearranging it to $\sum_{i=1}^{t} \valBy{i}{x} - \sum_{i=1}^{t-1}  z_i\geq z_t$, allows us to conclude that the objective value is determined by the left side of this inequality (as $z_k$ is maximized when the inequality turns to equality).
\begin{observation}\label{obs:obj-value}
The objective value obtained by a feasible solution $x$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is $\sum_{i=1}^{t} \valBy{i}{x} - \sum_{i=1}^{t-1}  z_i$.
\end{observation}

This conclusion also implies that for any $1 \leq t \leq n$, the solution $(x_t, z_t)$ that that was outputted for \eqref{eq:compact-OP} in iteration $t$, satisfies constraint $(\Tilde{3})$ as equality. That is:
\begin{observation}\label{obs:equality-xt-zt}
For any $1 \leq t \leq n$,  $\sum_{i=1}^{t} \valBy{i}{x_t} = \sum_{i=1}^{t}  z_i$.
\end{observation}



%%%
% OVERALL EXPLANATION
%We first establish our motivation by demonstrating, in Lemma \ref{lemma:not-beta-approx}, that $\retSol$ is not necessarily a $1-\beta$ Leximin approximation.\eden{wasn't sure were to put lemma \ref{lemma:not-beta-approx}, before or after}
% However, we then prove it is actually not that far off, it is a $1-2\beta$ approximation. 
We start by Lemma \ref{lemma:retSol-approx-all-t} \eden{To myself: to do}
Then, Lemmas \ref{lemma:mult-fk-lower-bound}-\ref{lemma:mult-special-z_k-upper-bound} establish a relationship between the $k$-th least objective value at 
% the returned solution ($\retSol$)
$\retSol$
% solution  returned by Algorithm \ref{alg:basic-ordered-Outcomes} ($\retSol$) 
and the value $z_k$. 
% In particular, the main conclusion is that the first is at least $\frac{1-2\beta}{1-\beta}$ of the second.
Theorem \ref{th:main} then uses this relation to prove that the existence of another solution that would be $\frac{1}{1-2\beta}$-preferred over $\retSol$ would lead to a contradiction.

% LEMMAS.
% BLAH BLAH.

 

\begin{lemma}\label{lemma:retSol-approx-all-t}
    Let $1 \leq t \leq n$. Then, the objective value obtained by $\retSol$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is a $(1-\beta)$ approximation.
\end{lemma}

\begin{proof}
    First, Observation \ref{obs:retSol-solves-any-t} ensures that $\retSol$ is a feasible solution for \eqref{eq:compact-OP} that was solved in  iteration $t$. 
    
    In addition, as $\retSol$ is a feasible solution of \eqref{eq:compact-OP} that was solved in iteration $n$, it is easy to see that $\sum_{i=1}^t \valBy{i}{\retSol} \geq \sum_{i=1}^{t} z_i$ (by constraint $(\Tilde{2})$ if $t<n$ and $(\Tilde{3})$ otherwise).
    By Observation \ref{obs:equality-xt-zt}, the solution $(x_t,z_t)$ obtained in iteration $t$ satisfies $\sum_{i=1}^t \valBy{i}{x_t} = \sum_{i=1}^{t} z_i$.
    We can conclude that:
    \begin{align}\label{equ:retSol-higher-than-xt}
        \sum_{i=1}^t \valBy{i}{\retSol} \geq \sum_{i=1}^t \valBy{i}{x_t}
    \end{align}
    The same Observation implies that $\sum_{i=1}^{t} \valBy{i}{x_t} - \sum_{i=1}^{t-1}  z_i = z_t$.
    However, $z_t$ is a $(1-\beta)$ approximation of $\sOptT{t}$, and so:
    \begin{align}\label{equ:xt-and-opt-t}
         \sum_{i=1}^{t} \valBy{i}{x_t} - \sum_{i=1}^{t-1}  z_i = z_t \geq (1-\beta) \sOptT{t}
     \end{align}
     
    Lastly, as Observation \ref{obs:obj-value} says that the objective values obtained by $\retSol$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is $\sum_{i=1}^{t} \valBy{i}{\retSol} - \sum_{i=1}^{t-1}  z_i$, we can conclude that this value is also a $(1-\beta)$ approximation of $\sOptT{t}$:
    \begin{align*}
        \sum_{i=1}^{t} \valBy{i}{\retSol} - \sum_{i=1}^{t-1}  z_i &\geq \sum_{i=1}^{t} \valBy{i}{x_t} - \sum_{i=1}^{t-1}  z_i && \text{equation \ref{equ:retSol-higher-than-xt}}\\
        &\geq (1-\beta) \sOptT{t} && \text{equation \ref{equ:xt-and-opt-t}}
    \end{align*}
\end{proof}




\begin{lemma}\label{lemma:mult-fk-lower-bound}
    For any $1 < k \leq n \colon \quad \valBy{k}{\retSol} \geq (1-\beta)\sOptT{k} - \frac{\beta}{1-\beta} z_{k-1}$.
\end{lemma}

\begin{proof}
    First, by Observation \ref{obs:retSol-solves-any-t}, $\retSol$ is also a feasible solution of \eqref{eq:compact-OP} in any iteration $t\in [n]$.
    By Observation \ref{obs:obj-value} the objective value that $\retSol$ yields in the problem solved in iteration $t$ is $\sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i$.
    However, during the algorithm run, the value obtained as a $(1 - \beta)$ approximation for this problem is $z_t$.
    This implies that the objective value of any feasible solution, in particular of $\retSol$, is at most $\frac{1}{1-\beta} z_t$.
    Therefore: 
    \begin{align}\label{equ:mult-other-sol-to-OP-upper-bound}
        \sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i \leq \frac{1}{1-\beta} z_t.
    \end{align}

    Now, let $1 < k \leq n$. 
    By Observation \ref{obs:equality-xt-zt}, the solution $(x_k,z_k)$ obtained in iteration $k$ satisfies  $\sum_{i=1}^k \valBy{i}{x_k} = \sum_{i=1}^{k} z_i$.
    On the one hand, as the value $z_k$ is a $(1-\beta)$ approximation of $\sOptT{k}$, this implies the following:
    \begin{align*}
        \sum_{i=1}^k \valBy{i}{x_k} - \sum_{i=1}^{k-1} z_i = z_k \geq (1-\beta) \sOptT{k}
    \end{align*}
    On the other hand, it is easy to see that $\sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^{k} z_i$ (by constraint $(\Tilde{2})$ if $k<n$ and $(\Tilde{3})$ otherwise), which also means that $\sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^{k} \valBy{i}{x_t}$. 
    The following can be concluded:
    \begin{align}
        \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i \geq \sum_{i=1}^k \valBy{i}{x_k} - \sum_{i=1}^{k-1} z_i = z_k \geq (1-\beta) \sOptT{k}
    \end{align}
    % Notice that by Observation \ref{obs:obj-value} this means that $\retSol$ also yields a $(1-\beta)$ approximation for $\sOptT{k}$.
    
    Now, the claim can concluded by isolating $\valBy{k}{\retSol}$:
    \begin{align*}
        \valBy{k}{\retSol} &\geq \sum_{i=1}^k z_i - \sum_{i=1}^{k-1} \valBy{i}{\retSol} \\
        & = z_k + z_{k-1} - \Bigr[\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-2} z_i \Bigr] \\
        & \geq z_k + z_{k-1} - \frac{1}{1-\beta}z_{k-1}  && \text{(by equation \eqref{equ:mult-other-sol-to-OP-upper-bound})}
        \\
        & = z_k - \frac{\beta}{1-\beta} z_{k-1}
    \end{align*}
\end{proof}


% ----- lemma 2 
\begin{lemma}\label{lemma:mult-zk-upper-bound}
    For any $1 < k \leq n \colon \quad z_k \leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol}$.
\end{lemma}


\begin{proof}
    The proof is by induction on $k$.
    For $k=2$, applying Lemma \ref{lemma:mult-fk-lower-bound} and rearranging it results in $z_2 \leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} z_{1}$. 
    However, constraint $(\Tilde{2})$ for $\ell = 1$ in the problem solved in iteration $n$ ensures that $\valBy{1}{\retSol} \geq z_1$.
    % \erel{In iteration $t=1$? In what constraint?}
    Accordingly, the claim can easily concluded:
    \begin{align*}
        z_2 &\leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} z_{1} \leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} \valBy{1}{\retSol} = \sum_{i=1}^2 \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{2-i+1}{\retSol}
    \end{align*}
    Next, assuming that the claim holds for $2, \dots, k-1$, by rearranging Lemma \ref{lemma:mult-fk-lower-bound}, it follows that it also holds for $k$:
    \begin{align*}
        z_k &\leq \valBy{k}{\retSol} + \frac{\beta}{1-\beta} z_{k-1}\\
        & \leq \valBy{k}{\retSol} + \frac{\beta}{1-\beta} \sum_{i=1}^{k-1} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-1-i+1}{\retSol} && \text{induction assumption}\\
        & \leq \valBy{k}{\retSol} + \sum_{i=1}^{k-1} \biggr[\frac{\beta}{1-\beta}\biggr]^{(i+1)-1} \valBy{k-(i+1)+1}{\retSol}\\
        & = \valBy{k}{\retSol} + \sum_{i=2}^{k} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol} && \text{index change (sum)}\\
        & = \sum_{i=1}^{k} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol}
    \end{align*}
\end{proof}


% ---------- lemma 3 
\begin{lemma}\label{lemma:mult-special-z_k-upper-bound}
    For any $1 \leq k \leq n \colon \quad 
        \frac{1-\beta}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl) \valBy{k}{\retSol} \geq z_k$
\end{lemma}

% \eden{we should decide if we include the following: \textit{"We prove a slightly stronger result: the approximation ratio is at most $\phi\cdot \beta$, where $\phi=$..."} I'm not sure where to put it....}

\begin{proof}
    Let $1 \leq k \leq n$. 
    First, observe that the expression $\sum_{i=1}^k \Bigr[\frac{\beta}{1-\beta}\Bigr]^{i-1}$ describes the sum of the geometric series with a first element $1$, a ratio $\frac{\beta}{1-\beta}$, and a length $k$. 
    As $\beta >1/2$, the ratio $\frac{\beta}{1-\beta} \neq 1$.
    Therefore, we can conclude the following:
    \begin{align*}
        \sum_{i=1}^k \Bigr[\frac{\beta}{1-\beta}\Bigr]^{i-1} = \frac{\biggr[\frac{\beta}{1-\beta}\biggr]^k - 1}{\frac{\beta}{1-\beta}-1}= \frac{1-\beta}{2\beta - 1} \Biggl(\biggr[\frac{\beta}{1-\beta}\biggr]^k - 1\Biggl) = \frac{1-\beta}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl)
    \end{align*}
    
    In addition, since $k-i+1 \leq k$ for any $1\leq i \leq k$, also $\valBy{k-i+1}{\retSol} \leq \valBy{k}{\retSol}$.
    Accordingly, the claim can be concluded from Lemma \ref{lemma:mult-zk-upper-bound}:
    \begin{align*}
        z_k &\leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol} \leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k}{\retSol} \\
        &\leq \frac{1-\beta}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl) \valBy{k}{\retSol} 
    \end{align*}
\end{proof}

%------
% thm.

We are now ready to prove the Theorem \ref{th:main}.
\begin{proof}[Proof of Theorem \ref{th:main}]
We prove a slightly stronger result: the returned solution is a $(1 - \mu \beta)$ approximately-optimal, where $\mu=\biggl(2- \frac{1}{\beta} \biggr[\frac{\beta}{1-\beta}\biggr]^n\biggl)/\biggl(1-\biggr[\frac{\beta}{1-\beta}\biggr]^n\biggl)$.
Notice that since $\biggr[\frac{\beta}{1-\beta}\biggr] < 1$, when the numbers of objective $n$ increases and tends to infinity the value of $ \biggr[\frac{\beta}{1-\beta}\biggr]^n$ tends to zero and therefore $\mu$ tends to $2$.\eden{is this clear enough?}
Specifically, since $\mu < 2$, by applying Lemma \ref{lemma:beta1-beta2-approx}, we get that if a solution is $(1 - \mu \beta)$ approximately-optimal then it is also $(1 - 2 \beta)$ approximately-optimal.
Therefore, proving that $\retSol$ is $(1 - \mu \beta)$ approximately-optimal  gives us a tighter bound on the approximation ratio with respect to $n$, while at the same time implies the original claim ---  $\retSol$ is $(1 - 2 \beta)$ approximately-optimal regardless of the number of objectives.
% $\phi=\frac{2- \beta \biggr[\frac{\beta}{1-\beta}\biggr]^k}{1-\biggr[\frac{\beta}{1-\beta}\biggr]^k}$.
% 

We first prove the following equation that will be helpful later:
\begin{align}\label{equ:mu}
\frac{1}{1 - \mu \beta } = \frac{1}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl)
\end{align}
This is true because:
\begin{align*}
    \mu &= \biggl(2- \frac{1}{\beta} \biggr[\frac{\beta}{1-\beta}\biggr]^n\biggl)/\biggl(1-\biggr[\frac{\beta}{1-\beta}\biggr]^n\biggl)  && \text{definition of $\mu$}\\
    & = \biggl(2- \frac{\beta^{n-1}}{(1-\beta)^n}\biggl)/\biggl(1-\frac{\beta^n}{(1-\beta)^n}\biggl) = \frac{2(1-\beta)^n - \beta^{n-1}}{(1-\beta)^n - \beta^{n}}
\end{align*}
and therefore,
\begin{align*}
    \frac{1}{1 - \mu \beta } &= \frac{1}{1 - \frac{2\beta(1-\beta)^n - \beta^{n}}{(1-\beta)^n - \beta^{n}}} = 
    \frac{1}{\frac{(1-\beta)^n - \beta^{n} - 2\beta(1-\beta)^n + \beta^{n}}{(1-\beta)^n - \beta^{n}}} \\
    & = \frac{(1-\beta)^n - \beta^{n}}{ (1 - 2\beta)(1-\beta)^n}= \frac{1}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^n\Biggl)
\end{align*}

Now, suppose for contradiction that $\retSol$ is not a $(1 - \mu \beta)$-approximate Leximin solution.
    By definition, this means there exists a solution $y \in S$  that is $\frac{1}{(1 - \mu\beta)}$-preferred over it.
    That is, there exists an integer $1 \leq k \leq n$ such that:
    \begin{align*}
        \forall j < k \colon &\valBy{j}{y} \geq \valBy{j}{\retSol};\\
        & \valBy{k}{y} > \frac{1}{(1 - \mu\beta)} \cdot \valBy{k}{\retSol}.
    \end{align*}
    
    As mentioned before, since $\retSol$ is a feasible solution to the optimization problem that was solved in iteration $n$, it is also feasible for the problem that was solved in iteration $k$ (as constraints were only added).
    As $y$'s $k$ least objective values are at least as those of $x$, this implies that $y$ 
    % satisfies all the constraints of this problem \eden{should we say something about constraint $(\Tilde{3})$? I'm mot sure how to explain it} 
    is feasible for this problem as well. 
    Since the objective of this problem is $(\max z_k)$ and the variable $z_k$ is included only in constraint $(\Tilde{3})$, the objective value of $y$ is determined by $\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i$.
    However, the approximation obtained for this problem during the algorithm run is $z_k$. 
    This implies that the optimal value value for this problem is at most $\frac{1}{(1-\beta)}z_k$.
    But, as we shall see, the objective of $y$ in this problem is higher than the optimal value, which is of course a contradiction.
    \begin{align*}
        &\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i\\
        &=  \valBy{k}{y} + \Bigr[\sum_{i=1}^{k-1} \valBy{i}{y} - \sum_{i=1}^{k-1} z_i\Bigr] \\
        & \geq  \valBy{k}{y} +0&& \text{constraint ($\Tilde{2}$) for } \ell=k-1\\
        &> \frac{1}{(1 - \mu\beta)} \cdot \valBy{k}{\retSol} && \text{$y$'s definition for } k\\
        & = \frac{1}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^n\Biggl) \valBy{k}{\retSol} && \text{equation \ref{equ:mu}}\\
        &\geq\frac{1}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl) \valBy{k}{\retSol} && k \leq n \\
        & = \frac{1}{1-\beta} \biggr[\frac{1-\beta}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl) \valBy{k}{\retSol}\biggr]\\
        &\geq \frac{1}{1-\beta} z_k && \text{Lemma \ref{lemma:mult-special-z_k-upper-bound}}
    \end{align*}
\end{proof}
\iffalse
Finally, to complete the picture, the following is an example that shows that the algorithm need not output a $(1-\beta)$ approximate Leximin.
Consider the following example with $n=2$:
    \begin{align*}
        \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
        s.t. \quad  & x_1 \leq 100\\
                    & x_1 + x_2 \leq 200\\
                    & x \in \mathbb{R}^2_{+}
    \end{align*}
    Consider a run of the algorithm with \textsf{OP} that is a $(1-\beta)$ approximate solver, for $\beta=0.1$. 
    In the first iteration, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
    Then, in the second iteration, given $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained with  $x_1=x_2=94.5$.  
    \erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}
    But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,94.5)$ is \emph{not} a $0.9$ approximation of $(94.5,105.5)$.
    \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5) \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition 
    $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}
\fi



==> files/backups/algo-2402-almost.tex <==

\section{Approximation Algorithm}\label{sec:algo-short}
We now present an algorithm for computing a multiplicative approximate leximin \eden{optimal?}. The algorithm is an adaptation of one of the algorithms of \textcite{Ogryczak_2006} for finding exact Leximin solutions. 

% \eden{yonatan}
% Following the \emph{definition} of Leximin, the core \emph{algorithm} for finding a Leximin optimal solution is interative, wherein one first maximizes the least objective function, then the second, and so forth. 
% Specifically, donating by $z_i$ the $i$-th smallest objective value, in each iteration, $t$, one seeks to maximize $z_t$, given the already calculated optimal values for $z_1,\ldots,z_{t-1}$.  The core, single-valued, optimization problem is thus:
%
% \eden{erel} 
% Following the definition of leximin, the core algorithm for finding a leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
% Denote by $z_t$ the value of the $i$-th smallest objective in the leximin-optimal solution, where $t\in\{1,\ldots,n\}$. Suppose we have already computed the optimal values $z_1,\ldots, z_{t-1}$. \eden{I'm not sure about it.. since we use the $z_t$ value later as the \textbf{approximation} value I think it could be a bit confusing}
% Then,  $z_t$ is the solution to the following single-objective optimization problem (where the variables are the scalar $z$ and the vector $x$):

\eden{how is this? I tried to combine the two versions}
Following the definition of Leximin, the core algorithm for finding a Leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
In each iteration, $t=1,\ldots,n$, it looks for the value that maximizes the $t$-th smallest objective, $z_t$, given that for any $i < t$ the $i$-th smallest objective is at least $z_i$ (the value that was computed in the $i$-th iteration).
The core, single-objective optimization problem is thus:
\begin{align}
 \max \quad &\ztVar{x}  \;\;
        s.t. &\quad  & (1) \quad x \in S  \tag{P1}\label{eq:basic-OP}\\
              &     & & (2) \quad \valBy{\ell}{x}\geq z_{\ell} & \ell = 1,\ldots,t-1\nonumber \\
               &    & & (3) \quad \valBy{t}{x} \geq \ztVar{x} \nonumber   
\end{align} 
where the variables are the scalar $\ztVar{x}$ and the vector $x$, and $z_1, \ldots z_{t-1}$ are constants.

Suppose we are given a procedure $\textsf{OP}(z_1,\ldots,z_{t-1})$, which, given  $z_1,\ldots,z_{t-1},$ outputs $(x,z)$ that is the exact optimal solution to \eqref{eq:basic-OP}.  
Then, the \emph{leximin} optimal solution is obtained by iterating this process for $t=1,\ldots,n$, as described in Algorithm \ref{alg:basic-ordered-Outcomes}.
\begin{algorithm}[!tbp]
\caption{The Ordered Outcomes Algorithm}
\label{alg:basic-ordered-Outcomes}
\begin{algorithmic}[1] %[1] enables line numbers
\FOR{$t=1$ to n}
\STATE \( %\begin{align*}
(x_t,z_t)\leftarrow \textsf{OP}(z_1,\ldots,z_{t-1})
\) %\end{align*} 
\ENDFOR
\STATE return $(z_1,\ldots,z_n)$ 
\end{algorithmic}
\end{algorithm}

However, it might be difficult to solve the problem \eqref{eq:basic-OP} as is, since constraints (2) and (3) are not linear even with respect to the objective-functions. 
\erel{I suggest to move P2-Compact here: it is a natural step between P1 and P2.}
\eden{}
 Thus, \cite{Ogryczak_2006} suggest using a variant of the problem that considers sums instead of individual values, which described as follows (similarly, the variables are $\ztVar{x}$ and $x$, and $z_1, \ldots z_{t-1}$ are constants):  
% \eden{maybe we should say it is not a linear program \textbf{with respect to the objective functions}?}
% \erel{I agree. Since the objective functions themselves may be non-linear.}
\begin{align*}
    \max \quad &\ztVar{x} \tag{P2}\label{eq:sums-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                    & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
Here, the constraints $(2)$ and $(3)$ are replaced with constraints $(\hat{2})$ and $(\hat{3})$, respectively. 
Constraint $(\hat{2})$ says that for any $\ell<t$, the sum of any $\ell$ objective functions is at least the sum of the first $\ell$ $z_i$'s. Similarly, $(\hat{3})$ says that the sum of any $t$  objective functions is at least the $t$ first $z_i$'s.  So, since we seek to maximize $z_t$, the optimal solution to \eqref{eq:sums-OP} and \eqref{eq:basic-OP} are provably identical (as in both $z_i$ is the $i$-th least objective value, see \cite{Ogryczak_2006} for a formal proof \eden{I'm actually not sure which of the papers to cite as I didn't find a formal proof (only the claim in given in \cite{Ogryczak_2006} and in \cite{Ogryczak2004TelecommunicationsND} Theorem 4)}). As such, in Algorithm \ref{alg:basic-ordered-Outcomes}, a solver for \eqref{eq:sums-OP} can be used (instead of for \eqref{eq:basic-OP}), and the algorithm will still output a Leximin optimal solution. 

Alas, while \eqref{eq:sums-OP} is linear with respect to the objective-functions, it has an exponential number of constraints. 
To overcome this problem, \cite{Ogryczak_2006} employ auxiliary variables ($y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$) to obtain a polynomial-sized program that is provably equivalent to \eqref{eq:sums-OP}:\eden{To myself: should explain "equivalent" in more detail, maybe to add the alternative proof}
% (where the variables are $\ztVar{x}$, $x$, and $y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$; and $z_1, \ldots z_{t-1}$ are constants)
\begin{align}
    \max \quad &z_t\tag{P3}\label{eq:vsums-OP}\\
        s.t. \quad  & (1) \quad x \in S \nonumber\\
                    & (2) \quad \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq \sum_{i=1}^{\ell}  z_i && \ell = 1, \ldots,t-1 \nonumber \\
                    & (3) \quad t y_t - \sum_{j=1}^{n} m_{t,j} \geq \sum_{i=1}^{t}  z_i  \nonumber \\
                    & (4) \quad m_{\ell,j} \geq y_{\ell} - f_j(x)  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber \\
                    & (5) \quad m_{\ell,j} \geq 0  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber
\end{align}
So, in Algorithm \ref{alg:basic-ordered-Outcomes} using a solver for \eqref{eq:vsums-OP}, the algorithm will output a Leximin optimal solution. 

All of the above is for exact solutions.  
The question is what happens when we consider approximation procedures? It is easy to see that if \textsf{OP} is a $(1-\beta)$ approximation algorithm to \eqref{eq:basic-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-\beta)$ approximation of the Leximin. 
\erel{
To say this, we first have to define the notion of "approximation algorithm". It is known, but we still have to define it formally. Maybe in the "preliminaries" section.
} 
However, for approximations, \eqref{eq:sums-OP}, and the equivalent \eqref{eq:vsums-OP}, are no longer equivalent to \eqref{eq:basic-OP}. Indeed, the following example shows that if \textsf{OP} is a $(1-\beta)$ approximation procedure for \eqref{eq:vsums-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} may output a solution that is \emph{not} a $1-\beta$ approximation to the Leximin.
% \erel{Maybe it is better to move the example to here, to motivate our proof.}
Consider the following multi-objective optimization problem with $n=2$:
\begin{align*}
    \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
    s.t. \quad  & x_1 \leq 100\\
                & x_1 + x_2 \leq 200\\
                & x \in \mathbb{R}^2_{+}
\end{align*}
Accordingly, the problem \eqref{eq:vsums-OP} becomes:
\begin{align*}
    \max \quad &z_t \\
    s.t. \quad  & (1.1) \quad  x_1 \leq 100\\
                & (1.2) \quad  x_1 + x_2 \leq 200\\
                & (1.3) \quad  x \in \mathbb{R}^2_{+}\\
                & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
The following is a possible run of the algorithm with \textsf{OP} that is a $(1-\beta)$ approximate solver for $\beta=0.1$. 
In the first iteration, $t=1$, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
Then, in the second iteration, $t=2$, given that $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained (for example) with  $x_1=x_2=94.5$.  
\erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}\eden{is it more clear now?}
Since $n=2$, the algorithm ends after this iteration and returns this solution $(94.5,94.5)$.
But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,105.5)\xPreferred{\frac{1}{0.9}}(94.5,94.5)$.
Therefore, by definition, the returned solution $(94.5,94.5)$ is \emph{not} a $0.9$ approximately-optimal solution.
% \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5)  \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition  $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}

 %On the other hand, \eqref{eq:vsums-OP} is the most solvable variant of the problem.  
So, using an approximate solver to \eqref{eq:vsums-OP}, what guarantee can we provide for the overall resulting solution? 
\begin{theorem}
\label{th:main}
Let $\beta<1/2$, and \textsf{OP} be a procedure that outputs a $(1-\beta)$ approximation to \eqref{eq:vsums-OP}. Then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-2\beta)$-approximate Leximin solution.  
\end{theorem}

\eden{maybe we should also include the proof of the additive variant somewhere? if so. where?}
\erel{
Since the proof is not explicitly mentioned anywhere, I think it is good to include a proof for comparison. Maybe in an appendix.
}
\eden{if we want to do so we should also describe the additive variant definition, maybe to put them both in the appendix? I added appendix \ref{sec:additive}}
The remainder of this section is dedicated to proving the theorem.
To this end, we use another equivalent representation of \eqref{eq:sums-OP}, which was also introduced by \cite{Ogryczak_2006}. 
\erel{This variant should move upwards, between P1 and P2.}
% (here also, the variables are $\ztVar{x}$ and $x$, and $z_1, \ldots z_{t-1}$ are constants)
\begin{align*}
    \max \quad &z_t \tag{P2-compact}\label{eq:compact-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\Tilde{2}) \quad \sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell}  z_i && \ell = 1,\ldots, t-1 \nonumber\\
                    & (\Tilde{3}) \quad \sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t}  z_i
\end{align*}
In this program, constraints $(\hat{2})$ and $(\hat{3})$ are replaced by  $(\Tilde{2})$ and $(\Tilde{3})$, respectively.  In  $(\hat{2})$, for each $\ell$, one gives a lower bound on the sum for \emph{any} set of $\ell$ objective functions.  In $(\Tilde{2})$, on the other hand, one only considers the sum of the $\ell$ \emph{smallest} such values.  However, since the constraints set the same lower bound on this sum, the constraints are equivalent.  Similarly for $(\hat{3})$ and $(\Tilde{3})$.  So, \eqref{eq:compact-OP} and \eqref{eq:sums-OP} are equivalent, which, in turn, is equivalent to \eqref{eq:vsums-OP}.  So, in proving the theorem we may assume that \textsf{OP} is an approximation procedure for \eqref{eq:compact-OP}.  This will simplify the proofs.

\erel{*** I do not understand. We say that P1 and P2 are equivalent with an exact solver, but not with an approximate solver. 
Here, we claim that P3 and P2-compact are equivalent, but this is true only with an exact solver. Don't we have to prove that they are equivalent also with an approximate solver? ***}

We denote $\retSol := x_n$ = the solution $x$ attained at the last iteration ($t=n$) of the algorithm. 

Following are some observations regarding the problem \eqref{eq:compact-OP} and the solution $\retSol$ that will be useful later.
First, notice that any solution $x \in S$ that satisfies constraint $(\Tilde{2})$ of \eqref{eq:compact-OP} is feasible to this problem.
This is because any solution $x \in S$ can satisfy constraint $(\Tilde{3})$ with a small enough assignment to the variable $z_t$. \eden{I'm not sure how to explain it....}
\begin{observation}\label{obs:feasi-and-constraint2}
Any solution $x \in S$ that satisfies constraint $(\Tilde{2})$ is feasible to \eqref{eq:compact-OP}.
\end{observation}

Since $\retSol$ is a feasible solution of \eqref{eq:compact-OP} in iteration $n$, and as each
iteration only adds new constraints to $(\Tilde{2})$, it follows that $\retSol$ is also a feasible solution of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$. 
\begin{observation}\label{obs:retSol-solves-any-t}
$\retSol$ is a feasible solution of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$.
\end{observation}

Now, consider the problem \eqref{eq:compact-OP} that was solved in iteration $t$.
Here, $z_t$ is a \emph{variable} and $z_1, \ldots z_{t-1}$ are constants.
The objective of this problem is $(\max z_t)$ and the only constraint that includes the variable $z_t$ is constraint $(\Tilde{3})$.
Therefore, rearranging it to $\sum_{i=1}^{t} \valBy{i}{x} - \sum_{i=1}^{t-1}  z_i\geq z_t$, allows us to conclude that the objective value is determined by the left side of this inequality (as $z_k$ is maximized when the inequality turns to equality).
\begin{observation}\label{obs:obj-value}
The objective value obtained by a feasible solution $x$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is $\sum_{i=1}^{t} \valBy{i}{x} - \sum_{i=1}^{t-1}  z_i$.
\end{observation}

Lastly, since the value obtained as a $(1 - \beta)$ approximation for this problem is the \emph{constant} $z_t$, the objective value of any feasible solution is at most $\frac{1}{1-\beta} z_t$.
It is particularly true for $\retSol$ since it is feasible for any iteration $t$ (Observation \ref{obs:retSol-solves-any-t}).
Since its objective is $\sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i$ (Observation \ref{obs:obj-value}) we can conclude:

\begin{observation}\label{obs:obj-xt-to-zt}
    The objective value obtained by $\retSol$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is at most $\frac{1}{1-\beta} z_t$. That is:
    \begin{align*}
        \sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i \leq \frac{1}{1-\beta} z_t
    \end{align*}
\end{observation}

% This conclusion also implies that for any $1 \leq t \leq n$, the solution $(x_t, z_t)$ that that was outputted for \eqref{eq:compact-OP} in iteration $t$, satisfies constraint $(\Tilde{3})$ as equality. That is:
% \begin{observation}\label{obs:equality-xt-zt}
% For any $1 \leq t \leq n$,  $\sum_{i=1}^{t} \valBy{i}{x_t} = \sum_{i=1}^{t}  z_i$.
% \end{observation}



%%%
% OVERALL EXPLANATION
%We first establish our motivation by demonstrating, in Lemma \ref{lemma:not-beta-approx}, that $\retSol$ is not necessarily a $1-\beta$ Leximin approximation.\eden{wasn't sure were to put lemma \ref{lemma:not-beta-approx}, before or after}
% However, we then prove it is actually not that far off, it is a $1-2\beta$ approximation. 
We start by Lemma \ref{lemma:retSol-approx-all-t} \eden{To myself: to do}
Then, Lemmas \ref{lemma:mult-fk-lower-bound}-\ref{lemma:mult-special-z_k-upper-bound} establish a relationship between the $k$-th least objective value at 
% the returned solution ($\retSol$)
$\retSol$
% solution  returned by Algorithm \ref{alg:basic-ordered-Outcomes} ($\retSol$) 
and the value $z_k$. 
% In particular, the main conclusion is that the first is at least $\frac{1-2\beta}{1-\beta}$ of the second.
Theorem \ref{th:main} then uses this relation to prove that the existence of another solution that would be $\frac{1}{1-2\beta}$-preferred over $\retSol$ would lead to a contradiction.

% LEMMAS.
% BLAH BLAH.

\begin{lemma}\label{lemma:beta-vk}
    Let $1 \leq k \leq n$. Then:
    \begin{align*}
        \beta \valBy{k}{\retSol} \geq \biggl(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\biggl) -\beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl)
    \end{align*}
\end{lemma}

\begin{proof}
    The claim follows from Observation \ref{obs:obj-xt-to-zt}:
    \begin{align*}
         &\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i \leq \frac{1}{1-\beta} z_k\\
         &\Rightarrow z_k \geq (1-\beta) \biggl(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\biggl)\\
        &\Rightarrow z_k \geq \biggl(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\biggl) - \beta \biggl(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\biggl)\\
        &\Rightarrow \beta \valBy{k}{\retSol} \geq \biggl(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\biggl) -\beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl)
    \end{align*}
\end{proof}


\begin{lemma}\label{lemma:beta-sums-to-diff}
    Let $1 \leq k \leq n$. Then:
    \begin{align*}
        \sum_{i=1}^k \beta^{i} \valBy{k-i+1}{\retSol} \geq \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k} z_i
    \end{align*}
\end{lemma}

\begin{proof}
    The proof is by induction on $k$.
    For $k=1$ the claim follows directly from Lemma \ref{lemma:beta-vk}.
    Assuming that the claim is true for $1,\ldots k-1$, then it is true also for $k$:
    \begin{align*}
        &\sum_{i=1}^k \beta^{i} \valBy{k-i+1}{\retSol} = \beta \valBy{k}{\retSol} + \sum_{i=2}^k \beta^{i} \valBy{k-i+1}{\retSol}\\
        &= \beta \valBy{k}{\retSol} + \sum_{i=1}^{k-1} \beta^{i+1} \valBy{k-(i+1)+1}{\retSol} \\
        &= \beta \valBy{k}{\retSol} + \beta \sum_{i=1}^{k-1} \beta^{i} \valBy{(k-1) -i+1}{\retSol}\\
        &= \beta \valBy{k}{\retSol} + \beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl) && \text{induction assumption}\\
        &\geq \biggl(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\biggl) -\beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl)  && \text{Lemma \ref{lemma:beta-vk}} \\
        & \quad +  \beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl)\\
        &\geq \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k} z_i
    \end{align*}
\end{proof}

\begin{lemma}\label{lemma:zk-to-beta-sums}
    Let $1 \leq k \leq n$. Then, $z_k \leq \sum_{i=1}^k \beta^{i-1} \valBy{k-i+1}{\retSol}$.
\end{lemma}

\begin{proof}
    Assume by contradiction that this is not true.
    This allows us to conclude that $\sum_{i=1}^k \valBy{i}{\retSol} < \sum_{i=1}^k z_i$:
    \begin{align*}
        &z_k > \sum_{i=1}^k \beta^{i-1} \valBy{k-i+1}{\retSol} = \valBy{k}{\retSol} +  \sum_{i=2}^k \beta^{i-1} \valBy{k-i+1}{\retSol}\\
        & = \valBy{k}{\retSol} +  \sum_{i=1}^{k-1} \beta^{i} \valBy{k-(i+1)+1}{\retSol} = \valBy{k}{\retSol} +  \sum_{i=1}^{k-1} \beta^{i} \valBy{(k-1)-i+1}{\retSol}\\
        &\geq \valBy{k}{\retSol} + \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i && \text{Lemma \ref{lemma:beta-sums}}
    \end{align*}
    However, the opposite, $\sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^k z_i$, is a constraint of \eqref{eq:compact-OP} that was solved in iteration $n$ (when $\retSol$ was obtained) --- a contradiction.
\end{proof}

%---- part 2
\begin{lemma}\label{lemma:fk-to-zk-zk-1}
    Let $1 < k \leq n$. Then, $\valBy{k}{\retSol} \geq z_k - \frac{\beta}{1-\beta} z_{k-1}$.
\end{lemma}

\begin{proof}
    Since $\retSol$ was obtained in \eqref{eq:compact-OP} that was solved in the last iteration $n$, $\sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^{k} z_i$ (by constraint $(\Tilde{2})$ if $k<n$ and $(\Tilde{3})$ otherwise).
    Accordingly, by isolating $\valBy{k}{\retSol}$, the claim can be concluded:
    \begin{align*}
        &\valBy{k}{\retSol} \geq \sum_{i=1}^k z_i - \sum_{i=1}^{k-1} \valBy{i}{\retSol} \\
        & = z_k + z_{k-1} - \Bigr[\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-2} z_i \Bigr] \geq \\
        & \geq z_k + z_{k-1} - \frac{1}{1-\beta}z_{k-1}  && \text{Observation \eqref{obs:obj-xt-to-zt} for $(k-1)$}
        \\
        & = z_k - \frac{\beta}{1-\beta} z_{k-1}
    \end{align*}
\end{proof}


\begin{lemma}\label{lemma:new-lower-bound}
    Let $1 < k \leq n$. Then:
    \begin{align*}
        z_k \leq \biggl(1 + \frac{\beta(1-\beta^k)}{(1-\beta)^2}\biggl)\valBy{k}{\retSol}
    \end{align*}
\end{lemma}

\begin{proof}
    First, notice that since $(k-1)-i+1 \leq k$ for any $1\leq i \leq k$ and as the function $\valBy{i}$ represents the $i$-th smallest objective value, also:
    \begin{align}\label{eq:increase-by-obj-size}
        \forall 1\leq i \leq k \colon \quad \valBy{(k-1)-i+1}{\retSol} \leq \valBy{k}{\retSol}
    \end{align}.
    In addition, consider the geometric series with a first element $1$, a ratio $\beta$, and a length $k-1$. 
    As $\beta \neq 1$, its sum can be described as:
    \begin{align}\label{eq:geometric-series-beta}
        \sum_{i=1}^{k-1} \beta^{i-1} = \frac{1-\beta^k}{1-\beta}
    \end{align}
    
    Now, the claim can be concluded as follows:
    \begin{align*}
        & z_k \leq \valBy{k}{\retSol} + \frac{\beta}{1-\beta} z_{k-1} && \text{Lemma \ref{lemma:fk-to-zk-zk-1}}\\
        & \leq \valBy{k}{\retSol} +  \frac{\beta}{1-\beta} \sum_{i=1}^{k-1} \beta^{i-1} \valBy{(k-1)-i+1}{\retSol} && \text{Lemma \ref{lemma:zk-to-beta-sums} (for $k-1$)}\\
        & \leq \valBy{k}{\retSol} +  \frac{\beta}{1-\beta} \sum_{i=1}^{k-1} \beta^{i-1} \cdot \valBy{k}{\retSol}  && \text{equation \ref{eq:increase-by-obj-size}}\\
        & \leq \valBy{k}{\retSol} +  \frac{\beta}{1-\beta} \frac{1-\beta^k}{1-\beta} \valBy{k}{\retSol} && \text{equation \ref{eq:geometric-series-beta}} \\
        & \leq \biggl(1 + \frac{\beta(1-\beta^k)}{(1-\beta)^2}\biggl) \valBy{k}{\retSol}
    \end{align*}
\end{proof}



\begin{lemma}\label{lemma:new-fk-lower-bound}
    Let $1 < k \leq n$. Then:
    \begin{align*}
        z_k \leq \valBy{k}{\retSol} +  \frac{\beta}{1-\beta} \frac{1-\beta^k}{1-\beta} \valBy{k}{\retSol}
    \end{align*}
    \begin{align*}
        z_k \leq \biggl(1 + \frac{\beta(1-\beta^k)}{(1-\beta)^2}\biggl)\valBy{k}{\retSol}
    \end{align*}
\end{lemma}



\begin{lemma}\label{lemma:mult-fk-lower-bound}
    For any $1 < k \leq n \colon \quad \valBy{k}{\retSol} \geq (1-\beta)\sOptT{k} - \frac{\beta}{1-\beta} z_{k-1}$.
\end{lemma}

\begin{proof}
    First, by Observation \ref{obs:retSol-solves-any-t}, $\retSol$ is also a feasible solution of \eqref{eq:compact-OP} in any iteration $t\in [n]$.
    By Observation \ref{obs:obj-value} the objective value that $\retSol$ yields in the problem solved in iteration $t$ is $\sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i$.
    However, during the algorithm run, the value obtained as a $(1 - \beta)$ approximation for this problem is $z_t$.
    This implies that the objective value of any feasible solution, in particular of $\retSol$, is at most $\frac{1}{1-\beta} z_t$.
    Therefore: 
    \begin{align}\label{equ:mult-other-sol-to-OP-upper-bound}
        \sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i \leq \frac{1}{1-\beta} z_t.
    \end{align}

    Now, let $1 < k \leq n$. 
    By Observation \ref{obs:equality-xt-zt}, the solution $(x_k,z_k)$ obtained in iteration $k$ satisfies  $\sum_{i=1}^k \valBy{i}{x_k} = \sum_{i=1}^{k} z_i$.
    On the one hand, as the value $z_k$ is a $(1-\beta)$ approximation of $\sOptT{k}$, this implies the following:
    \begin{align*}
        \sum_{i=1}^k \valBy{i}{x_k} - \sum_{i=1}^{k-1} z_i = z_k \geq (1-\beta) \sOptT{k}
    \end{align*}
    On the other hand, it is easy to see that $\sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^{k} z_i$ (by constraint $(\Tilde{2})$ if $k<n$ and $(\Tilde{3})$ otherwise), which also means that $\sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^{k} \valBy{i}{x_t}$. 
    The following can be concluded:
    \begin{align}
        \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i \geq \sum_{i=1}^k \valBy{i}{x_k} - \sum_{i=1}^{k-1} z_i = z_k \geq (1-\beta) \sOptT{k}
    \end{align}
    % Notice that by Observation \ref{obs:obj-value} this means that $\retSol$ also yields a $(1-\beta)$ approximation for $\sOptT{k}$.
    
    Now, the claim can concluded by isolating $\valBy{k}{\retSol}$:
    \begin{align*}
        \valBy{k}{\retSol} &\geq \sum_{i=1}^k z_i - \sum_{i=1}^{k-1} \valBy{i}{\retSol} \\
        & = z_k + z_{k-1} - \Bigr[\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-2} z_i \Bigr] \\
        & \geq z_k + z_{k-1} - \frac{1}{1-\beta}z_{k-1}  && \text{(by equation \eqref{equ:mult-other-sol-to-OP-upper-bound})}
        \\
        & = z_k - \frac{\beta}{1-\beta} z_{k-1}
    \end{align*}
\end{proof}


% ----- lemma 2 
\begin{lemma}\label{lemma:mult-zk-upper-bound}
    For any $1 < k \leq n \colon \quad z_k \leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol}$.
\end{lemma}


\begin{proof}
    The proof is by induction on $k$.
    For $k=2$, applying Lemma \ref{lemma:mult-fk-lower-bound} and rearranging it results in $z_2 \leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} z_{1}$. 
    However, constraint $(\Tilde{2})$ for $\ell = 1$ in the problem solved in iteration $n$ ensures that $\valBy{1}{\retSol} \geq z_1$.
    % \erel{In iteration $t=1$? In what constraint?}
    Accordingly, the claim can easily concluded:
    \begin{align*}
        z_2 &\leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} z_{1} \leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} \valBy{1}{\retSol} = \sum_{i=1}^2 \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{2-i+1}{\retSol}
    \end{align*}
    Next, assuming that the claim holds for $2, \dots, k-1$, by rearranging Lemma \ref{lemma:mult-fk-lower-bound}, it follows that it also holds for $k$:
    \begin{align*}
        z_k &\leq \valBy{k}{\retSol} + \frac{\beta}{1-\beta} z_{k-1}\\
        & \leq \valBy{k}{\retSol} + \frac{\beta}{1-\beta} \sum_{i=1}^{k-1} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-1-i+1}{\retSol} && \text{induction assumption}\\
        & \leq \valBy{k}{\retSol} + \sum_{i=1}^{k-1} \biggr[\frac{\beta}{1-\beta}\biggr]^{(i+1)-1} \valBy{k-(i+1)+1}{\retSol}\\
        & = \valBy{k}{\retSol} + \sum_{i=2}^{k} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol} && \text{index change (sum)}\\
        & = \sum_{i=1}^{k} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol}
    \end{align*}
\end{proof}


% ---------- lemma 3 
\begin{lemma}\label{lemma:mult-special-z_k-upper-bound}
    For any $1 \leq k \leq n \colon \quad 
        \frac{1-\beta}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl) \valBy{k}{\retSol} \geq z_k$
\end{lemma}

% \eden{we should decide if we include the following: \textit{"We prove a slightly stronger result: the approximation ratio is at most $\phi\cdot \beta$, where $\phi=$..."} I'm not sure where to put it....}

\begin{proof}
    Let $1 \leq k \leq n$. 
    First, observe that the expression $\sum_{i=1}^k \Bigr[\frac{\beta}{1-\beta}\Bigr]^{i-1}$ describes the sum of the geometric series with a first element $1$, a ratio $\frac{\beta}{1-\beta}$, and a length $k$. 
    As $\beta >1/2$, the ratio $\frac{\beta}{1-\beta} \neq 1$.
    Therefore, we can conclude the following:
    \begin{align*}
        \sum_{i=1}^k \Bigr[\frac{\beta}{1-\beta}\Bigr]^{i-1} = \frac{\biggr[\frac{\beta}{1-\beta}\biggr]^k - 1}{\frac{\beta}{1-\beta}-1}= \frac{1-\beta}{2\beta - 1} \Biggl(\biggr[\frac{\beta}{1-\beta}\biggr]^k - 1\Biggl) = \frac{1-\beta}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl)
    \end{align*}
    
    In addition, since $k-i+1 \leq k$ for any $1\leq i \leq k$, also $\valBy{k-i+1}{\retSol} \leq \valBy{k}{\retSol}$.
    Accordingly, the claim can be concluded from Lemma \ref{lemma:mult-zk-upper-bound}:
    \begin{align*}
        z_k &\leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol} \leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k}{\retSol} \\
        &\leq \frac{1-\beta}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl) \valBy{k}{\retSol} 
    \end{align*}
\end{proof}

%------
% thm.

We are now ready to prove the Theorem \ref{th:main}.
\begin{proof}[Proof of Theorem \ref{th:main}]
We prove a slightly stronger result: the returned solution is a $(1 - \mu \beta)$ approximately-optimal, where $\mu=\biggl(2- \frac{1}{\beta} \biggr[\frac{\beta}{1-\beta}\biggr]^n\biggl)/\biggl(1-\biggr[\frac{\beta}{1-\beta}\biggr]^n\biggl)$.
Notice that since $\biggr[\frac{\beta}{1-\beta}\biggr] < 1$, when the numbers of objective $n$ increases and tends to infinity the value of $ \biggr[\frac{\beta}{1-\beta}\biggr]^n$ tends to zero and therefore $\mu$ tends to $2$.\eden{is this clear enough?}
Specifically, since $\mu < 2$, by applying Lemma \ref{lemma:beta1-beta2-approx}, we get that if a solution is $(1 - \mu \beta)$ approximately-optimal then it is also $(1 - 2 \beta)$ approximately-optimal.
Therefore, proving that $\retSol$ is $(1 - \mu \beta)$ approximately-optimal  gives us a tighter bound on the approximation ratio with respect to $n$, while at the same time implies the original claim ---  $\retSol$ is $(1 - 2 \beta)$ approximately-optimal regardless of the number of objectives.
% $\phi=\frac{2- \beta \biggr[\frac{\beta}{1-\beta}\biggr]^k}{1-\biggr[\frac{\beta}{1-\beta}\biggr]^k}$.
% 

We first prove the following equation that will be helpful later:
\begin{align}\label{equ:mu}
\frac{1}{1 - \mu \beta } = \frac{1}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^k\Biggl)
\end{align}
This is true because:
\begin{align*}
    \mu &= \biggl(2- \frac{1}{\beta} \biggr[\frac{\beta}{1-\beta}\biggr]^n\biggl)/\biggl(1-\biggr[\frac{\beta}{1-\beta}\biggr]^n\biggl)  && \text{definition of $\mu$}\\
    & = \biggl(2- \frac{\beta^{n-1}}{(1-\beta)^n}\biggl)/\biggl(1-\frac{\beta^n}{(1-\beta)^n}\biggl) = \frac{2(1-\beta)^n - \beta^{n-1}}{(1-\beta)^n - \beta^{n}}
\end{align*}
and therefore,
\begin{align*}
    \frac{1}{1 - \mu \beta } &= \frac{1}{1 - \frac{2\beta(1-\beta)^n - \beta^{n}}{(1-\beta)^n - \beta^{n}}} = 
    \frac{1}{\frac{(1-\beta)^n - \beta^{n} - 2\beta(1-\beta)^n + \beta^{n}}{(1-\beta)^n - \beta^{n}}} \\
    & = \frac{(1-\beta)^n - \beta^{n}}{ (1 - 2\beta)(1-\beta)^n}= \frac{1}{1 - 2\beta} \Biggl(1 - \biggr[\frac{\beta}{1-\beta}\biggr]^n\Biggl)
\end{align*}

Now, suppose for contradiction that $\retSol$ is not a $(1 - \mu \beta)$-approximate Leximin solution.
    By definition, this means there exists a solution $y \in S$  that is $\frac{1}{(1 - \mu\beta)}$-preferred over it.
    That is, there exists an integer $1 \leq k \leq n$ such that:
    \begin{align*}
        \forall j < k \colon &\valBy{j}{y} \geq \valBy{j}{\retSol};\\
        & \valBy{k}{y} > \frac{1}{(1 - \mu\beta)} \cdot \valBy{k}{\retSol}.
    \end{align*}
    
    As mentioned before, since $\retSol$ is a feasible solution to the optimization problem that was solved in iteration $n$, it is also feasible for the problem that was solved in iteration $k$ (as constraints were only added).
    As $y$'s $k$ least objective values are at least as those of $x$, this implies that $y$ 
    % satisfies all the constraints of this problem \eden{should we say something about constraint $(\Tilde{3})$? I'm mot sure how to explain it} 
    is feasible for this problem as well. 
    Since the objective of this problem is $(\max z_k)$ and the variable $z_k$ is included only in constraint $(\Tilde{3})$, the objective value of $y$ is determined by $\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i$.
    However, the approximation obtained for this problem during the algorithm run is $z_k$. 
    This implies that the optimal value value for this problem is at most $\frac{1}{(1-\beta)}z_k$.
    But, as we shall see, the objective of $y$ in this problem is higher than the optimal value, which is of course a contradiction.
    \begin{align*}
        &\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i=\sum_{i=1}^{k-1} \valBy{i}{y} - \sum_{i=1}^{k-1} z_i + \valBy{k}{y}\\
        &\geq \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1}{1-\beta} \valBy{k}{\retSol} + \frac{\beta^2}{1-\beta}\frac{1-\beta^k}{1-\beta} \valBy{k}{\retSol}\\
        &\geq \sum_{i=1}^{k-1} \valBy{i}{y} - \sum_{i=1}^{k-1} z_i + \frac{1}{1-\beta} \valBy{k}{\retSol} + \frac{\beta}{1-\beta}\biggl(\sum_{i=1}^{k-1} \beta^{i} \valBy{(k-1)-i+1}{\retSol}\biggl) && \text{Lemma \ref{lemma:beta-sums-to-diff}}\\
        &\geq \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1}{1-\beta} \valBy{k}{\retSol} + \frac{\beta}{1-\beta}\biggl(\sum_{i=1}^{k-1}\valBy{i}{\retSol} - \sum_{i=1}^{k-1}z_i\biggl)\\
        &=\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1}{1-\beta} \valBy{k}{\retSol} + \frac{\beta}{1-\beta}\sum_{i=1}^{k-1}\valBy{i}{\retSol} - \frac{\beta}{1-\beta}\sum_{i=1}^{k-1}z_i\\
        & > \frac{1}{1-\beta} \biggr[\sum_{i=1}^k \valBy{k}{\retSol} - \sum_{i=1}^{k-1}z_i\biggr]
    \end{align*}
\end{proof}
\iffalse
Finally, to complete the picture, the following is an example that shows that the algorithm need not output a $(1-\beta)$ approximate Leximin.
Consider the following example with $n=2$:
    \begin{align*}
        \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
        s.t. \quad  & x_1 \leq 100\\
                    & x_1 + x_2 \leq 200\\
                    & x \in \mathbb{R}^2_{+}
    \end{align*}
    Consider a run of the algorithm with \textsf{OP} that is a $(1-\beta)$ approximate solver, for $\beta=0.1$. 
    In the first iteration, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
    Then, in the second iteration, given $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained with  $x_1=x_2=94.5$.  
    \erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}
    But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,94.5)$ is \emph{not} a $0.9$ approximation of $(94.5,105.5)$.
    \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5) \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition 
    $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}
\fi



==> files/backups/algo-backup-bef-stronger.tex <==

\section{Approximation Algorithm}\label{sec:algo-short}
We now present an algorithm for computing a multiplicative approximate leximin \eden{optimal?}. The algorithm is an adaptation of one of the algorithms of \textcite{Ogryczak_2006} for finding exact Leximin solutions. 
% Accordingly, the bulk of the effort is in proving that the approximate version of the algorithm indeed produces the desired approximate Leximin.

Following the definition of leximin, the core algorithm for finding a leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
Denote by $z_t$ the value of the $i$-th smallest objective in the leximin-optimal solution, where $t\in\{1,\ldots,n\}$. Suppose we have already computed the optimal values $z_1,\ldots, z_{t-1}$. \eden{I'm not sure about it.. since we use the $z_t$ value later as the \textbf{approximation} value I think it could be a bit confusing}
Then,  $z_t$ is the solution to the following single-objective optimization problem (where the variables are the scalar $z$ and the vector $x$):
\eden{need to check if changing $z_t$ to $z$ effect the proofs}
%, in each iteration, $t$, one seeks to maximize $z_t$, given the already calculated optimal values for $z_1,\ldots,z_{t-1}$.  The core, single-valued, optimization problem is thus:
\begin{align}
 \max \quad &z  \;\;
        s.t. &\quad  & (1) \quad x \in S  \tag{P1}\label{eq:basic-OP}\\
              &     & & (2) \quad \valBy{\ell}{x}\geq z_{\ell} & \ell = 1,\ldots,t-1\nonumber \\
               &    & & (3) \quad \valBy{t}{x} \geq z \nonumber   
\end{align} 
Suppose we are given a procedure $\textsf{OP}(z_1,\ldots,z_{t-1})$, which, given  $z_1,\ldots,z_{t-1},$ outputs $(x,z)$ that is the exact optimal solution to \eqref{eq:basic-OP}.  Then, the Leximin optimal solution is obtained by iterating this process for $t=1,\ldots,n$, as described in Algorithm \ref{alg:basic-ordered-Outcomes}.
\begin{algorithm}[!tbp]
\caption{The Ordered Outcomes Algorithm}
\label{alg:basic-ordered-Outcomes}
\begin{algorithmic}[1] %[1] enables line numbers
\FOR{$t=1$ to n}
\STATE \( %\begin{align*}
(x_t,z_t)\leftarrow \textsf{OP}(z_1,\ldots,z_{t-1})
\) %\end{align*} 
\ENDFOR
\STATE return $(z_1,\ldots,z_n)$ 
\end{algorithmic}
\end{algorithm}

However, as is, constraints (2) and (3) of problem \eqref{eq:basic-OP} are not linear even with respect to the objective-functions.
Therefore, it might be difficult to solve. 
\erel{I suggest to move P2-Compact here: it is a natural step between P1 and P2.}
\eden{}
 Thus, \cite{Ogryczak_2006} suggest using a variant of the problem that considers sums instead of individual values, as follows (where the variables are the scalar $z$ and the vector $x$):  
% \eden{maybe we should say it is not a linear program \textbf{with respect to the objective functions}?}
% \erel{I agree. Since the objective functions themselves may be non-linear.}
\begin{align*}
    \max \quad &z_t \tag{P2}\label{eq:sums-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                    & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
Here, the constraints $(2)$ and $(3)$ are replaced with constraints $(\hat{2})$ and $(\hat{3})$, respectively. Constraint $(\hat{2})$ says that for any $\ell<t$, the sum of any $\ell$ objective functions is at least the sum of the first $\ell$ $z_i$'s. Similarly, $(\hat{3})$ says that the sum of any $t$  objective functions is at least the $t$ first $z_i$'s.  So, since we seek to maximize $z_t$, the optimal solution to \eqref{eq:sums-OP} and \eqref{eq:basic-OP} are provably identical (as in both $z_i$ is the $i$-th least objective value, see \cite{Ogryczak_2006} for a formal proof \eden{I'm actually not sure which of the papers to cite as I didn't find a formal proof (only the claim in given in \cite{Ogryczak_2006} and in \cite{Ogryczak2004TelecommunicationsND} Theorem 4)}). As such, in Algorithm \ref{alg:basic-ordered-Outcomes}, a solver for \eqref{eq:sums-OP} can be used (instead of for \eqref{eq:basic-OP}), and the algorithm will still output a Leximin optimal solution. 

Alas, while \eqref{eq:sums-OP} is linear with respect to the objective-functions, it has an exponential number of constraints. 
To overcome this problem, \cite{Ogryczak_2006} employ auxiliary variables ($y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$) to obtain a polynomial-sized program that is provably equivalent to \eqref{eq:sums-OP}:\eden{To myself: should explain "equivalent" in more detail, maybe to add the alternative proof}
\begin{align}
    \max \quad &z_t\tag{P3}\label{eq:vsums-OP}\\
        s.t. \quad  & (1) \quad x \in S \nonumber\\
                    & (2) \quad \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq \sum_{i=1}^{\ell}  z_i && \ell = 1, \ldots,t-1 \nonumber \\
                    & (3) \quad t y_t - \sum_{j=1}^{n} m_{t,j} \geq \sum_{i=1}^{t}  z_i  \nonumber \\
                    & (4) \quad m_{\ell,j} \geq y_{\ell} - f_j(x)  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber \\
                    & (5) \quad m_{\ell,j} \geq 0  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber
\end{align}
So, in Algorithm \ref{alg:basic-ordered-Outcomes} using a solver for \eqref{eq:vsums-OP}, the algorithm will output a Leximin optimal solution. 

All of the above is for exact solutions.  The question is what happens when we consider approximation procedures? It is easy to see that if \textsf{OP} is a $(1-\beta)$ approximation algorithm to \eqref{eq:basic-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-\beta)$ approximation of the Leximin. 
\erel{
To say this, we first have to define the notion of "approximation algorithm". It is known, but we still have to define it formally. Maybe in the "preliminaries" section.
} 
However, for approximations, \eqref{eq:sums-OP}, and the equivalent \eqref{eq:vsums-OP}, are no longer equivalent to \eqref{eq:basic-OP}. Indeed, the following example shows that if \textsf{OP} is a $(1-\beta)$ approximation procedure for \eqref{eq:vsums-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} may output a solution that is \emph{not} a $1-\beta$ approximation to the Leximin.
\erel{Maybe it is better to move the example to here, to motivate our proof.}
Consider the following multi-objective optimization problem with $n=2$:
\begin{align*}
    \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
    s.t. \quad  & x_1 \leq 100\\
                & x_1 + x_2 \leq 200\\
                & x \in \mathbb{R}^2_{+}
\end{align*}
According to these settings, the problem \eqref{eq:vsums-OP} becomes:
\begin{align*}
    \max \quad &z_t \\
    s.t. \quad  & (1.1) \quad  x_1 \leq 100\\
                & (1.2) \quad  x_1 + x_2 \leq 200\\
                & (1.3) \quad  x \in \mathbb{R}^2_{+}\\
                & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
The following is a possible run of the algorithm with \textsf{OP} that is a $(1-\beta)$ approximate solver, for $\beta=0.1$. 
In the first iteration, $t=1$, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
Then, in the second iteration, $t=2$, given that $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained with  $x_1=x_2=94.5$.  
\erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}\eden{is it more clear now?}
But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,105.5)\xPreferred{\frac{1}{0.9}}(94.5,94.5)$.
Therefore, by definition, the returned solution $(94.5,94.5)$ is \emph{not} a $0.9$ approximately-optimal solution.
% \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5)  \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition  $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}

 %On the other hand, \eqref{eq:vsums-OP} is the most solvable variant of the problem.  
So, using an approximate solver to \eqref{eq:vsums-OP}, what guarantee can we provide for the overall resulting solution? 
\begin{theorem}
\label{th:main}
Let $\beta<1/2$, and \textsf{OP} be a procedure that outputs a $(1-\beta)$ approximation to \eqref{eq:vsums-OP}. Then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-2\beta)$-approximate Leximin solution.  
\end{theorem}

\eden{maybe we should also include the proof of the additive variant somewhere? if so. where?}
\erel{
Since the proof is not explicitly mentioned anywhere, I think it is good to include a proof for comparison. Maybe in an appendix.
}
\eden{if we want to do so we should also describe the additive variant definition, maybe to put them both in the appendix? I added appendix \ref{sec:additive}}
The remainder of this section is dedicated to proving the theorem.
To this end, we introduce yet another equivalent representation of \eqref{eq:sums-OP}. 
\erel{This variant should move upwards, between P1 and P2.}
\begin{align*}
    \max \quad &z_t \tag{P2-compact}\label{eq:compact-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\Tilde{2}) \quad \sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell}  z_i && \ell = 1,\ldots, t-1 \nonumber\\
                    & (\Tilde{3}) \quad \sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t}  z_i
\end{align*}
In this program, constraints $(\hat{2})$ and $(\hat{3})$ are replaced by  $(\Tilde{2})$ and $(\Tilde{3})$, respectively.  In  $(\hat{2})$, for each $\ell$, one gives a lower bound on the sum for \emph{any} set of $\ell$ objective functions.  In $(\Tilde{2})$, on the other hand, one only considers the sum of the $\ell$ \emph{smallest} such values.  However, since the constraints set the same lower bound on this sum, the constraints are equivalent.  Similarly for $(\hat{3})$ and $(\Tilde{3})$.  So, \eqref{eq:compact-OP} and \eqref{eq:sums-OP} are equivalent, which, in turn, is equivalent to \eqref{eq:vsums-OP}.  So, in proving the theorem we may assume that \textsf{OP} is an approximation procedure for \eqref{eq:compact-OP}.  This will simplify the proofs.

\erel{*** I do not understand. We say that P1 and P2 are equivalent with an exact solver, but not with an approximate solver. 
Here, we claim that P3 and P2-compact are equivalent, but this is true only with an exact solver. Don't we have to prove that they are equivalent also with an approximate solver? ***}

\er{We denote $\retSol := x_n$ = the solution $x$ attained at the last iteration ($t=n$) of the algorithm.}

% OVERALL EXPLANATION
%We first establish our motivation by demonstrating, in Lemma \ref{lemma:not-beta-approx}, that $\retSol$ is not necessarily a $1-\beta$ Leximin approximation.\eden{wasn't sure were to put lemma \ref{lemma:not-beta-approx}, before or after}
% However, we then prove it is actually not that far off, it is a $1-2\beta$ approximation. 
Lemmas \ref{lemma:mult-fk-lower-bound}-\ref{lemma:mult-special-z_k-upper-bound} establish a relationship between the $k$-th least objective value at 
% the returned solution ($\retSol$)
$\retSol$
% solution  returned by Algorithm \ref{alg:basic-ordered-Outcomes} ($\retSol$) 
and the value $z_k$. 
In particular, the main conclusion is that the first is at least $\frac{1-2\beta}{1-\beta}$ of the second.
Theorem \ref{th:main} then uses this lower bound to prove that the existence of another solution that would be $\frac{1}{1-2\beta}$-preferred over $\retSol$ would lead to a contradiction.

% LEMMAS.
% BLAH BLAH.


\begin{lemma}\label{lemma:mult-fk-lower-bound}
    For any $1 < k \leq n \colon \quad \valBy{k}{\retSol} \geq z_k - \frac{\beta}{1-\beta} z_{k-1}$.
\end{lemma}

\begin{proof}
    Since $\retSol$ is a feasible solution of \eqref{eq:compact-OP} in iteration $n$, it is also a feasible solution of \eqref{eq:compact-OP} in any iteration $t\leq n$, as each iteration only adds new constraints. 
    Consider the problem solved in iteration $t$.
    Since its objective is $(\max z_t)$ and the only constraint that includes the variable $z_t$ is constraint $(\Tilde{3})$ (i.e., $\sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t}  z_i$), the objective value that $\retSol$ yields in this problem is: 
    \begin{align}\label{eq:obj-retSol-in-prob-t}
        \sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i
    \end{align}
    However, during the algorithm run, the value obtained as a $(1 - \beta)$ approximation for this problem is \eden{the constant} $z_t$.
    This implies that the objective value of any feasible solution is at most $\frac{1}{1-\beta} z_t$.
    As $\retSol$ is feasible, equation \ref{eq:obj-retSol-in-prob-t} allows us to conclude the following:
    \begin{align}\label{equ:mult-other-sol-to-OP-upper-bound}
    	\sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i \leq \frac{1}{1-\beta} z_t.
    \end{align}

    Now, let $1 < k \leq n$. 
    By considering the problem solved in the last iteration $n$, it is easy to see that $\sum_{i=1}^t \valBy{i}{\retSol} \geq \sum_{i=1}^{t} z_i$ (by constraint $(\Tilde{2})$ if $k<n$ and $(\Tilde{3})$ otherwise).
 % \erel{These constraints are not in P2-Compact.   What program do you refer to?}).
    As a result, the claim can concluded by isolating $\valBy{k}{\retSol}$:
    \begin{align*}
        \valBy{k}{\retSol} &\geq \sum_{i=1}^k z_i - \sum_{i=1}^{k-1} \valBy{i}{\retSol} \\
        & = z_k + z_{k-1} - \Bigr[\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-2} z_i \Bigr] \geq \\
        & \geq z_k + z_{k-1} - \frac{1}{1-\beta}z_{k-1}  && \text{(by equation \eqref{equ:mult-other-sol-to-OP-upper-bound})}
        \\
        & = z_k - \frac{\beta}{1-\beta} z_{k-1}
    \end{align*}
\end{proof}


% ----- lemma 2 
\begin{lemma}\label{lemma:mult-zk-upper-bound}
    For any $1 < k \leq n \colon \quad z_k \leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol}$.
\end{lemma}


\begin{proof}
    The proof is by induction on $k$.
    For $k=2$, applying Lemma \ref{lemma:mult-fk-lower-bound} and rearranging it results in $z_2 \leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} z_{1}$. 
    However, constraint $(\Tilde{2})$ for $\ell = 1$ in the problem solved in iteration $n$ ensures that $\valBy{1}{\retSol} \geq z_1$.
    % \erel{In iteration $t=1$? In what constraint?}
    Accordingly, the claim can easily concluded:
    \begin{align*}
        z_2 &\leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} z_{1} \leq \valBy{2}{\retSol} + \frac{\beta}{1-\beta} \valBy{1}{\retSol} = \sum_{i=1}^2 \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{2-i+1}{\retSol}
    \end{align*}
    Next, assuming that the claim holds for $2, \dots, k-1$, by rearranging Lemma \ref{lemma:mult-fk-lower-bound}, it follows that it also holds for $k$:
    \begin{align*}
        z_k &\leq \valBy{k}{\retSol} + \frac{\beta}{1-\beta} z_{k-1}\\
        & \leq \valBy{k}{\retSol} + \frac{\beta}{1-\beta} \sum_{i=1}^{k-1} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-1-i+1}{\retSol} && \text{induction assumption}\\
        & \leq \valBy{k}{\retSol} + \sum_{i=1}^{k-1} \biggr[\frac{\beta}{1-\beta}\biggr]^{(i+1)-1} \valBy{k-(i+1)+1}{\retSol}\\
        & = \valBy{k}{\retSol} + \sum_{i=2}^{k} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol} && \text{index change (sum)}\\
        & = \sum_{i=1}^{k} \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol}
    \end{align*}
\end{proof}


% ---------- lemma 3 
\begin{lemma}\label{lemma:mult-special-z_k-upper-bound}
    For any $1 \leq k \leq n \colon \quad 
        \frac{1-\beta}{1-2\beta} \cdot \valBy{k}{\retSol} \geq z_k$
\end{lemma}

\eden{we should decide if we include the following: \textit{"We prove a slightly stronger result: the approximation ratio is at most $\phi\cdot \beta$, where $\phi=$..."} I'm not sure where to put it....}

\begin{proof}
    Let $1 \leq k \leq n$. 
    If $k=1$ the claim is trivial since $\valBy{1}{\retSol} \geq z_1$ (direct constraint) and $\frac{1-\beta}{1-2\beta} \geq 1$ (as $\beta \geq 0$).
    For $k>1$, however, as $\beta < 1/2$ implies that $0 \leq \frac{\beta}{1-\beta} < 1$, by considering the sum of the infinite geometric series with this ratio and a first element $1$, we get that:
    \begin{align*}
        \sum_{i=1}^k \Bigr[\frac{\beta}{1-\beta}\Bigr]^{i-1} &< \lim_{k \rightarrow \infty} \sum_{i=1}^k \Bigr[\frac{\beta}{1-\beta}\Bigr]^{i-1} =  \frac{1}{1-\Bigr[\frac{\beta}{1-\beta}\Bigr]} = \frac{1-\beta}{1-2\beta}
    \end{align*}
    Therefore, as $k-i+1 \leq k$ for any $1\leq i \leq k$, the claim can be concluded from Lemma \ref{lemma:mult-zk-upper-bound}:
    \begin{align*}
        z_k \leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k-i+1}{\retSol} \leq \sum_{i=1}^k \biggr[\frac{\beta}{1-\beta}\biggr]^{i-1} \valBy{k}{\retSol} < \frac{1-\beta}{1-2\beta} \valBy{k}{\retSol} 
    \end{align*}
\end{proof}

%------
% thm.

We are now ready to prove the Theorem \ref{th:main}.
\begin{proof}[Proof of Theorem \ref{th:main}]
Suppose for contradiction that $\retSol$ is not a $(1 - 2\beta)$-approximate Leximin solution.
    By definition, this means there exists a solution $y$  that is $\frac{1}{(1 - 2\beta)}$-preferred over it.
    That is, there exists an integer $1 \leq k \leq n$ such that:
    \begin{align*}
        \forall j < k \colon &\valBy{j}{y} \geq \valBy{j}{\retSol};\\
        & \valBy{k}{y} > \frac{1}{(1 - 2\beta)} \cdot \valBy{k}{\retSol}.
    \end{align*}
    Since $\retSol$ is a solution to the optimization problem that was solved in iteration $k$, and as $y$'s $k$ least objective values are higher, $y$ is also a solution to this problem. 
    But, as we shall see, the objective value of $y$ in this problem is higher than the optimal value, which is of course a contradiction:
    \begin{align*}
        &\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i && \text{objective isolating \erel{What is "objective isolating"?} }\\
        &=  \valBy{k}{y} + \Bigr[\sum_{i=1}^{k-1} \valBy{i}{y} - \sum_{i=1}^{k-1} z_i\Bigr] \\
        & \geq  \valBy{k}{y} +0&& \text{constraint (2) for } \ell=k-1\\
        &> \frac{1}{(1 - 2\beta)} \cdot \valBy{k}{\retSol} && \text{$y$'s definition for } k\\
        & = \frac{1}{1-\beta} \biggr[\frac{1 - \beta}{(1 - 2\beta)} \cdot \valBy{k}{\retSol}\biggr] \\
        &\geq \frac{1}{1-\beta} z_k && \text{Lemma \ref{lemma:mult-special-z_k-upper-bound}}
    \end{align*}
\end{proof}
\iffalse
Finally, to complete the picture, the following is an example that shows that the algorithm need not output a $(1-\beta)$ approximate Leximin.
Consider the following example with $n=2$:
    \begin{align*}
        \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
        s.t. \quad  & x_1 \leq 100\\
                    & x_1 + x_2 \leq 200\\
                    & x \in \mathbb{R}^2_{+}
    \end{align*}
    Consider a run of the algorithm with \textsf{OP} that is a $(1-\beta)$ approximate solver, for $\beta=0.1$. 
    In the first iteration, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
    Then, in the second iteration, given $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained with  $x_1=x_2=94.5$.  
    \erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}
    But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,94.5)$ is \emph{not} a $0.9$ approximation of $(94.5,105.5)$.
    \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5) \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition 
    $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}
\fi



==> files/backups/algo-with-n-0303.tex <==

\section{Approximation Algorithm}\label{sec:algo-short}
We now present an algorithm for computing an approximately-optimal leximin solution. The algorithm is an adaptation of one of the algorithms of \textcite{Ogryczak_2006} for finding exact leximin solutions. 

% \eden{yonatan}    
% Following the \emph{definition} of leximin, the core \emph{algorithm} for finding a leximin optimal solution is interative, wherein one first maximizes the least objective function, then the second, and so forth. 
% Specifically, donating by $z_i$ the $i$-th smallest objective value, in each iteration, $t$, one seeks to maximize $z_t$, given the already calculated optimal values for $z_1,\ldots,z_{t-1}$.  The core, single-valued, optimization problem is thus:
%
% \eden{erel} 
% Following the definition of leximin, the core algorithm for finding a leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
% Denote by $z_t$ the value of the $i$-th smallest objective in the leximin-optimal solution, where $t\in\{1,\ldots,n\}$. Suppose we have already computed the optimal values $z_1,\ldots, z_{t-1}$. \eden{I'm not sure about it.. since we use the $z_t$ value later as the \textbf{approximation} value I think it could be a bit confusing}
% Then,  $z_t$ is the solution to the following single-objective optimization problem (where the variables are the scalar $z$ and the vector $x$):

\eden{how is this? I tried to combine the two versions}
Following the definition of leximin, the core algorithm for finding a leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
In each iteration, $t=1,\ldots,n$, it looks for the value that maximizes the $t$-th smallest objective, $z_t$, given that for any $i < t$ the $i$-th smallest objective is at least $z_i$ (the value that was computed in the $i$-th iteration).
The core, single-objective optimization problem is thus:
\begin{align}
 \max \quad &\ztVar{x}  \;\;
        s.t. &\quad  & (1) \quad x \in S  \tag{P1}\label{eq:basic-OP}\\
              &     & & (2) \quad \valBy{\ell}{x}\geq z_{\ell} & \ell = 1,\ldots,t-1\nonumber \\
               &    & & (3) \quad \valBy{t}{x} \geq \ztVar{x} \nonumber   
\end{align} 
where the variables are the scalar $\ztVar{x}$ and the vector $x$, and $z_1, \ldots z_{t-1}$ are constants.

Suppose we are given a procedure $\textsf{OP}(z_1,\ldots,z_{t-1})$, which, given  $z_1,\ldots,z_{t-1},$ outputs $(x,z)$ that is the exact optimal solution to \eqref{eq:basic-OP}.  
Then, the \emph{leximin} optimal solution is obtained by iterating this process for $t=1,\ldots,n$, as described in Algorithm \ref{alg:basic-ordered-Outcomes}.
\begin{algorithm}[!tbp]
\caption{The Ordered Outcomes Algorithm}
\label{alg:basic-ordered-Outcomes}
\begin{algorithmic}[1] %[1] enables line numbers
\FOR{$t=1$ to n}
\STATE \( %\begin{align*}
(x_t,z_t)\leftarrow \textsf{OP}(z_1,\ldots,z_{t-1})
\) %\end{align*} 
\ENDFOR
\STATE return $(z_1,\ldots,z_n)$ 
\end{algorithmic}
\end{algorithm}

However, it might be difficult to solve the problem \eqref{eq:basic-OP} as is, since constraints (2) and (3) are not linear even with respect to the objective-functions. 
 Thus, \cite{Ogryczak_2006} suggest using a variant of the problem that considers sums instead of individual values, which described as follows (similarly, the variables are $\ztVar{x}$ and $x$, and $z_1, \ldots z_{t-1}$ are constants):  
\begin{align*}
    \max \quad &\ztVar{x} \tag{P2}\label{eq:sums-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                    & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
Here, the constraints $(2)$ and $(3)$ are replaced with constraints $(\hat{2})$ and $(\hat{3})$, respectively. 
Constraint $(\hat{2})$ says that for any $\ell<t$, the sum of any $\ell$ objective functions is at least the sum of the first $\ell$ $z_i$'s. 
Similarly, $(\hat{3})$ says that the sum of any $t$  objective functions is at least the sum of the $t$ first $z_i$'s.
The program \eqref{eq:sums-OP} is important in the context of leximin since (\cite{Ogryczak2004TelecommunicationsND} Theorem 4):
\begin{lemma}\label{lemma:alg-1-can-use-sums-exact}
    In Algorithm \ref{alg:basic-ordered-Outcomes}, a solver for \eqref{eq:sums-OP} can be used (instead of for \eqref{eq:basic-OP}), and the algorithm will still output a leximin optimal solution. 
\end{lemma}
\noindent For the completeness of this paper, in Appendix \ref{sec:equivalent-proofs}, we provide an alternative proof of this claim.



Alas, while \eqref{eq:sums-OP} is linear with respect to the objective-functions, it has an exponential number of constraints. 
To overcome this challenge, \cite{Ogryczak_2006} employ auxiliary variables ($y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$) to obtain a polynomial-sized program that can be used in the same way as \eqref{eq:sums-OP} (\cite{Ogryczak_2006} Theorem 1):
% (where the variables are $\ztVar{x}$, $x$, and $y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$; and $z_1, \ldots z_{t-1}$ are constants)
\begin{align}
    \max \quad &z_t\tag{P3}\label{eq:vsums-OP}\\
        s.t. \quad  & (1) \quad x \in S \nonumber\\
                    & (2) \quad \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq \sum_{i=1}^{\ell}  z_i && \ell = 1, \ldots,t-1 \nonumber \\
                    & (3) \quad t y_t - \sum_{j=1}^{n} m_{t,j} \geq \sum_{i=1}^{t}  z_i  \nonumber \\
                    & (4) \quad m_{\ell,j} \geq y_{\ell} - f_j(x)  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber \\
                    & (5) \quad m_{\ell,j} \geq 0  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber
\end{align}
In Appendix \ref{sec:equivalent-proofs}, we prove a stronger claim:
\begin{lemma}
    The programs \eqref{eq:sums-OP} and \eqref{eq:vsums-OP} are equivalent\footnote{Recall that two programs are considered \emph{equivalent} if they have the same set of feasible solutions (Section \ref{sec:preliminaries}).}.
\end{lemma}
\noindent When programs are equivalent, a solver for one can be used as a solver for the other (Lemma \ref{}). 
Together with Lemma \ref{lemma:alg-1-can-use-sums-exact} this means that a solver for \eqref{eq:vsums-OP} can also be used in Algorithm \ref{alg:basic-ordered-Outcomes} to obtain a leximin optimal solution. 

Notice that none of these claims asserts that \eqref{eq:basic-OP} is equivalent to either \eqref{eq:sums-OP} or \eqref{eq:vsums-OP}; in fact, we will show that  \eqref{eq:basic-OP} is not equivalent.
In practice, the reason that solvers for these programs can be used interchangeably inside algorithm \ref{alg:basic-ordered-Outcomes} is that they all have the same optimal value when the constants $z_1,\ldots,z_{t-1}$ are the \emph{optimal} values of the previous iterations $1, \ldots, (t-1)$ respectively.

% All of the above is for exact solvers.  
The question is what happens when we consider approximation procedures? 
That is, when the constants $z_1,\ldots,z_{t-1}$ are \emph{approximations} obtained in the previous iterations.
It is easy to see that if \textsf{OP} is a $(\multError, \additiveError)$-approximation algorithm\footnote{See Section \ref{sec:preliminaries} for $(\multError, \additiveError)$-approximation algorithm formal definition.} to \eqref{eq:basic-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(\multError, \additiveError)$-approximately-optimal leximin solution\footnote{See Section \ref{sec:approx-leximin-def} for $(\multError, \additiveError)$-approximately-optimal leximin solution formal definition.} (formal proof in Appendix \ref{sec:equivalent-proofs}). 
% \erel{ To say this, we first have to define the notion of "approximation algorithm". It is known, but we still have to define it formally. Maybe in the "preliminaries" section. } 
However, if \textsf{OP} approximates \eqref{eq:sums-OP}, or the equivalent \eqref{eq:vsums-OP}, the algorithm may behave differently.
In the following example, \textsf{OP} is a $(\multError, \additiveError)$-approximation procedure for \eqref{eq:sums-OP}, and Algorithm \ref{alg:basic-ordered-Outcomes} outputs a solution that is \emph{not} $(\multError, \additiveError)$-approximately-optimal.
Consider the following multi-objective optimization problem with $n=2$:
\begin{align*}
    \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
    s.t. \quad  & x_1 \leq 100\\
                & x_1 + x_2 \leq 200\\
                & x \in \mathbb{R}^2_{+}
\end{align*}
Accordingly, the problem \eqref{eq:vsums-OP} becomes:
\begin{align*}
    \max \quad &z_t \\
    s.t. \quad  & (1.1) \quad  x_1 \leq 100\\
                & (1.2) \quad  x_1 + x_2 \leq 200\\
                & (1.3) \quad  x \in \mathbb{R}^2_{+}\\
                & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
The following is a possible run of the algorithm with \textsf{OP} that is a $(\multError, \additiveError)$-approximate solver for $\multError=0.1$ and $\additiveError = 0$. 
Notice that for simplicity, we use an example in which $\additiveError=0$; however, this also allows us to demonstrate that even when there is only a multiplicative error, the algorithm behaves differently.
In the first iteration, $t=1$, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
Then, in the second iteration, $t=2$, given that $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained (for example) with  $x_1=x_2=94.5$.  
\erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}\eden{is it more clear now?}
Since $n=2$, the algorithm ends after this iteration and returns the solution $(94.5,94.5)$.
But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,105.5) \alphaBetaPreferredParams{0.1}{0} (94.5,94.5)$.
Therefore, by definition, the returned solution is \emph{not} $(0.1,0)$-approximately-optimal.
% \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5)  \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition  $(94.5,94.5)$ is not a $0.9$-approximation"}
% \erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}

 %On the other hand, \eqref{eq:vsums-OP} is the most solvable variant of the problem.  
So, using an approximate solver to \eqref{eq:sums-OP} or \eqref{eq:vsums-OP}, what guarantee can we provide for the overall resulting solution? 

\begin{theorem}\label{th:main}
Let $\multError\in [0,1)$, $\additiveError \geq 0$, and \textsf{OP} be a $(\multError, \additiveError)$-approximation procedure to \eqref{eq:vsums-OP}. Then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $\left(\frac{1}{1-\multError +\multError^2}\multError, \frac{1-\multError^2}{1-\multError +\multError^2}\additiveError\right)$-approximately-optimal leximin solution.  
\end{theorem}

% \eden{should we explain somewhere about the consequences on the cases where only multiplicative or additive error are present? if so, where?}
\noindent Notice that this result also implies that if \textsf{OP} only has a multiplicative error $\multError$, the solution returned by Algorithm \ref{alg:basic-ordered-Outcomes} will only have a multiplicative error of $\frac{\multError}{1-\multError +\multError^2}$, and if \textsf{OP} only has an additive error $\additiveError$, the solution returned by Algorithm \ref{alg:basic-ordered-Outcomes} will have only the same additive error $\additiveError$.

The remainder of this section is dedicated to proving the theorem.
To this end, we use another equivalent representation of \eqref{eq:sums-OP} (proof in Appendix \ref{sec:equivalent-proofs}), which was also introduced by \cite{Ogryczak_2006}. 
% \erel{This variant should move upwards, between P1 and P2.}
% (here also, the variables are $\ztVar{x}$ and $x$, and $z_1, \ldots z_{t-1}$ are constants)
\begin{align*}
    \max \quad &z_t \tag{P2-compact}\label{eq:compact-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\Tilde{2}) \quad \sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell}  z_i && \ell = 1,\ldots, t-1 \nonumber\\
                    & (\Tilde{3}) \quad \sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t}  z_i
\end{align*}
In this program, constraints $(\hat{2})$ and $(\hat{3})$ are replaced by  $(\Tilde{2})$ and $(\Tilde{3})$, respectively.  
In  $(\hat{2})$, for each $\ell$, one gives a lower bound on the sum for \emph{any} set of $\ell$ objective functions.  
In $(\Tilde{2})$, on the other hand, one only considers the sum of the $\ell$ \emph{smallest} such values.  
% However, since the constraints set the same lower bound on this sum, the constraints are equivalent.  
Similarly for $(\hat{3})$ and $(\Tilde{3})$.  
Recall that when two programs are equivalent, a solver, either exact or approximate, for one can be used as a solver, with the same level of accuracy, for the other (Lemma \ref{}). 
Therefore, as \eqref{eq:compact-OP} is equivalent to \eqref{eq:sums-OP}, which, in turn, is equivalent to \eqref{eq:vsums-OP}, in proving the theorem we may assume that \textsf{OP} is an approximation procedure for \eqref{eq:compact-OP}.  
This will simplify the proofs.

\erel{*** I do not understand. We say that P1 and P2 are equivalent with an exact solver, but not with an approximate solver. 
Here, we claim that P3 and P2-compact are equivalent, but this is true only with an exact solver. Don't we have to prove that they are equivalent also with an approximate solver? ***}

We denote $\retSol := x_n$ = the solution $x$ attained at the last iteration ($t=n$) of the algorithm. 

Following are some observations regarding the set of feasible solutions in each iteration, their objective values, and the solution $\retSol$ that will be useful later on.
First, notice that any solution $x \in S$ that satisfies constraint $(\Tilde{2})$ of \eqref{eq:compact-OP} is feasible to this problem.
This is because any solution $x \in S$ can satisfy constraint $(\Tilde{3})$ with a small enough assignment to the variable $z_t$. \eden{I'm not sure how to explain it....}
\begin{observation}\label{obs:feasi-and-constraint2}
Any solution $x \in S$ that satisfies constraint $(\Tilde{2})$ is feasible to \eqref{eq:compact-OP}.
\end{observation}

Since $\retSol$ is a feasible solution of \eqref{eq:compact-OP} in iteration $n$, and as each
iteration only adds new constraints to $(\Tilde{2})$, it follows that $\retSol$ is also a feasible solution of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$. 
\begin{observation}\label{obs:retSol-solves-any-t}
$\retSol$ is a feasible solution of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$.
\end{observation}

Now, consider the problem \eqref{eq:compact-OP} that was solved in iteration $t$.
Here, $z_t$ is a \emph{variable} and $z_1, \ldots z_{t-1}$ are constants.
The objective of this problem is $(\max z_t)$ and the only constraint that includes the variable $z_t$ is constraint $(\Tilde{3})$.
Therefore, rearranging it to $\sum_{i=1}^{t} \valBy{i}{x} - \sum_{i=1}^{t-1}  z_i\geq z_t$, allows us to conclude that the objective value is determined by the left side of this inequality (as $z_k$ is maximized when the inequality turns to equality).
\begin{observation}\label{obs:obj-value}
The objective value obtained by a feasible solution $x$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is $\sum_{i=1}^{t} \valBy{i}{x} - \sum_{i=1}^{t-1}  z_i$.
\end{observation}

Lastly, as the value obtained as a $(\multError, \additiveError)$-approximation for this problem is the \emph{constant} $z_t$, the optimal value is at most $\frac{1}{1-\multError} (z_t+\additiveError)$. 
Consequently, the objective value of any feasible solution is at most this value.
Since $\retSol$ is feasible for any iteration $t$ (Observation \ref{obs:retSol-solves-any-t}) and since its objective is $\sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i$ (Observation \ref{obs:obj-value}), we can conclude:

\begin{observation}\label{obs:obj-xt-to-zt}
    The objective value obtained by $\retSol$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is at most $\frac{1}{1-\multError} (z_t+\additiveError)$. That is:
    \begin{align*}
        \sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i \leq \frac{1}{1-\multError} \left(z_t+\additiveError \right)
    \end{align*}
\end{observation}

% This conclusion also implies that for any $1 \leq t \leq n$, the solution $(x_t, z_t)$ that that was outputted for \eqref{eq:compact-OP} in iteration $t$, satisfies constraint $(\Tilde{3})$ as equality. That is:
% \begin{observation}\label{obs:equality-xt-zt}
% For any $1 \leq t \leq n$,  $\sum_{i=1}^{t} \valBy{i}{x_t} = \sum_{i=1}^{t}  z_i$.
% \end{observation}



%%%
% OVERALL EXPLANATION
%We first establish our motivation by demonstrating, in Lemma \ref{lemma:not-beta-approx}, that $\retSol$ is not necessarily a $1-\multError$ leximin approximation.\eden{wasn't sure were to put lemma \ref{lemma:not-beta-approx}, before or after}
% However, we then prove it is actually not that far off, it is a $1-2\multError$ approximation. 
We start by Lemma \ref{lemma:retSol-approx-all-t} \eden{To myself: to do}
Then, Lemmas \ref{lemma:mult-fk-lower-bound}-\ref{lemma:mult-special-z_k-upper-bound} establish a relationship between the $k$-th least objective value at 
% the returned solution ($\retSol$)
$\retSol$
% solution  returned by Algorithm \ref{alg:basic-ordered-Outcomes} ($\retSol$) 
and the value $z_k$. 
% In particular, the main conclusion is that the first is at least $\frac{1-2\multError}{1-\multError}$ of the second.
Theorem \ref{th:main} then uses this relation to prove that the existence of another solution that would be $\frac{1}{1-2\multError}$-preferred over $\retSol$ would lead to a contradiction.

% LEMMAS.
% BLAH BLAH.

\begin{lemma}\label{lemma:beta-vk}
    Let $1 \leq k \leq n$. Then:
    \begin{align*}
        \multError \valBy{k}{\retSol} \geq \left(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\right) -\multError \left(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\right) -\additiveError
    \end{align*}
\end{lemma}

\begin{proof}
    The claim follows from Observation \ref{obs:obj-xt-to-zt}:
    \begin{align*}
         &\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i \leq \frac{1}{1-\multError} \left(z_k + \additiveError \right)\\
         &\Rightarrow z_k +\additiveError \geq (1-\multError) \left(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\right)\\
        &\Rightarrow z_k +\additiveError\geq \left(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\right) - \multError \left(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\right)\\
        &\Rightarrow \multError \valBy{k}{\retSol} \geq \left(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\right) -\multError \left(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\right) -\additiveError
    \end{align*}
\end{proof}


\begin{lemma}\label{lemma:beta-sums-to-diff}
    Let $1 \leq k \leq n$. Then:
    \begin{align*}
        \sum_{i=1}^k \multError^{i} \valBy{k-i+1}{\retSol} \geq \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k} z_i -\additiveError
    \end{align*}
\end{lemma}

\begin{proof}
    The proof is by induction on $k$.
    For $k=1$ the claim follows directly from Lemma \ref{lemma:beta-vk}.
    Assuming that the claim is true for $1,\ldots k-1$, then it is true also for $k$:
    \begin{align*}
        &\sum_{i=1}^k \multError^{i} \valBy{k-i+1}{\retSol} = \multError \valBy{k}{\retSol} + \sum_{i=2}^k \multError^{i} \valBy{k-i+1}{\retSol}\\
        &= \multError \valBy{k}{\retSol} + \sum_{i=1}^{k-1} \multError^{i+1} \valBy{k-(i+1)+1}{\retSol} \\
        &= \multError \valBy{k}{\retSol} + \multError \sum_{i=1}^{k-1} \multError^{i} \valBy{(k-1) -i+1}{\retSol}\\
        &= \multError \valBy{k}{\retSol} + \multError \left(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\right) && \text{Induction assumption}\\
        &\geq \left(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\right) -\multError \left(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\right)-\additiveError  \\
        & \quad +  \multError \left(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\right) && \text{Lemma \ref{lemma:beta-vk}} \\
        &\geq \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k} z_i -\additiveError
    \end{align*}
\end{proof}


\begin{lemma}\label{lemma:fk-to-all}
    Let $1 \leq k \leq n$. Then:
    \begin{align*}
        \frac{1-\multError +\multError^2(1-\multError^{n})}{1-\multError} \valBy{k}{\retSol} \geq \valBy{k}{\retSol} + \multError\left(\sum_{i=1}^{k-1}\valBy{i}{\retSol} - \sum_{i=1}^{k-1}z_i - \additiveError \right)
    \end{align*}
\end{lemma}

\begin{proof}
First, notice that since $k \geq (k-1)-i+1$ for any $1\leq i \leq k$ and as the function $\valBy{i}$ represents the $i$-th smallest objective value, also:
    \begin{align}\label{eq:increase-by-obj-size}
        \forall 1\leq i \leq k \colon \quad \valBy{k}{\retSol} \geq \valBy{(k-1)-i+1}{\retSol}
    \end{align}
    In addition, consider the geometric series with a first element $1$, a ratio $\multError$, and a length $k-1$. 
    As $\multError \neq 1$, its sum can be described as:
    \begin{align}\label{eq:geometric-series-beta}
        \sum_{i=1}^{k-1} \multError^{i-1} = \frac{1-\multError^k}{1-\multError}
    \end{align}
    
    Now, the claim can be concluded as follows:
    \begin{align*}
        &\frac{1-\multError +\multError^2(1-\multError^{n})}{1-\multError} \valBy{k}{\retSol} = \left(1 + \frac{\multError^2(1-\multError^k)}{1-\multError}\right) \valBy{k}{\retSol} \\
        &= \valBy{k}{\retSol} + \multError^2 \left(\frac{1-\multError^k}{1-\multError} \valBy{k}{\retSol} \right)\\
        & = \valBy{k}{\retSol} + \multError^2 \left(\sum_{i=1}^{k-1} \multError^{i-1} \valBy{k}{\retSol} \right) && \text{Equation \ref{eq:geometric-series-beta}}\\
        & \geq \valBy{k}{\retSol} + \multError^2 \left(\sum_{i=1}^{k-1} \multError^{i-1} \valBy{(k-1)-i+1}{\retSol} \right) && \text{Equation \ref{eq:increase-by-obj-size}}\\
        &= \valBy{k}{\retSol} + \multError \sum_{i=1}^{k-1} \multError^{i} \valBy{(k-1)-i+1}{\retSol} \\
        &\geq \valBy{k}{\retSol} + \multError\left(\sum_{i=1}^{k-1}\valBy{i}{\retSol} - \sum_{i=1}^{k-1}z_i - \additiveError \right) && \text{Lemma \ref{lemma:beta-sums-to-diff}}
\end{align*}
\end{proof}



%------
% thm.

We are now ready to prove the Theorem \ref{th:main}.
\begin{proof}[Proof of Theorem \ref{th:main}]
\eden{should decide whether to keep this part}
Recall that the claim is that $\retSol$ is a $\left(\frac{1}{1-\multError +\multError^2}\multError, \frac{1-\multError^2}{1-\multError +\multError^2}\additiveError\right)$-approximation.
However, we prove a slightly stronger result: the solution $\retSol$ is $\left(\Delta^{mult}_n \multError, \Delta^{add}_n\additiveError\right)$ approximately-optimal, where:
\begin{align*}
    &\Delta^{mult}_n=\frac{1-\multError+\multError(1-\multError^n)}{1-\multError +\multError^2(1-\multError^n)}, &&\Delta^{add}_n = \frac{1-\multError^2}{1-\multError + \multError^2(1-\multError^n)}
\end{align*}
% $\Delta^{mult}_n=\frac{1-\multError+\multError(1-\multError^n)}{1-\multError +\multError^2(1-\multError^n)}$ and $\Delta^{add}_n = \frac{1-\multError^2}{1-\multError + \multError^2(1-\multError^n)}$.
Since $\multError < 1$, when the numbers of objectives, $n$, increases and tends to infinity, the value of $\multError^n$ tends to zero, and therefore $\Delta^{mult}_n$ tends to $\frac{1-\multError+\multError}{1-\multError +\multError^2} = \frac{1}{1-\multError +\multError^2}$ and $\Delta^{add}_n$ tends to $\frac{1-\multError^2}{1-\multError +\multError^2}$.
Specifically, since $\lambda_n < \frac{1}{1-\multError +\multError^2}$, proving this claim implies the original one (by Lemma \ref{lemma:beta1-beta2-approx}), while, at the same time, gives us a tighter bound on the approximation ratio with respect to $n$.

We first prove the following equation that will be helpful later:
\begin{align}\label{equ:mu}
\frac{1}{1 - \lambda_n \multError } = \frac{1-\multError +\multError^2(1-\multError^{n})}{(1-\multError)^2}
\end{align}
This is true because:
\begin{align*}
    & 1 - \lambda_n \multError =  1 - \frac{1-\multError+\multError(1-\multError^n)}{1-\multError +\multError^2(1-\multError^n)}\multError && \text{definition of $\mu$} \\
    & = \frac{1-\multError +\multError^2(1-\multError^n) - \multError(1-\multError)- \multError^2(1-\multError^n)}{1-\multError +\multError^2(1-\multError^{n})}\\
    & = \frac{(1-\multError)^2}{1-\multError +\multError^2(1-\multError^{n})}
    \end{align*}
    and therefore,
    \begin{align*}
        & \frac{1}{1 - \lambda_n \multError } = \frac{1-\multError +\multError^2(1-\multError^{n})}{(1-\multError)^2}
    \end{align*}
    In addition, we prove the following equation that will be useful as well:
    \begin{align}\label{eq:additive-error}
        \frac{1}{1 - \lambda_n \multError }\cdot\frac{1-\multError^2}{1-\multError + \multError^2(1-\multError^n)} = \frac{1+\beta}{1-\beta}
    \end{align}
    The reason for this is that:
    \begin{align*}
        &\frac{1}{1 - \lambda_n \multError }\cdot\frac{1-\multError^2}{1-\multError + \multError^2(1-\multError^n)} \\
        &=\frac{1-\multError +\multError^2(1-\multError^{n})}{(1-\multError)^2} \cdot\frac{(1-\multError)(1+\multError)}{1-\multError + \multError^2(1-\multError^n)}&& \text{Equation \ref{equ:mu}}\\
        &= \frac{1+\beta}{1-\beta}
    \end{align*}

    Now, suppose by contradiction that $\retSol$ is not $\left(\lambda_n \multError, (1+\multError)\additiveError\right)$-approximately-optimal.
    By definition, this means there exists a solution $y \in S$  that is $\left(\lambda_n \multError, (1+\multError)\additiveError\right)$-preferred over it.
    That is, there exists an integer $1 \leq k \leq n$ such that:
    \begin{align*}
        \forall j < k \colon &\valBy{j}{y} \geq \valBy{j}{\retSol};\\
        & \valBy{k}{y} > \frac{1}{(1 - \lambda_n \multError)} \left(\valBy{k}{\retSol} + (1+\multError)\additiveError \right).
    \end{align*}

    Since $\retSol$ was obtained in \eqref{eq:compact-OP} that was solved in the last iteration $n$, it is clear that $\sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^{k} z_i$ (by constraint $(\Tilde{2})$ if $k<n$ and $(\Tilde{3})$ otherwise).
    Which implies:
    \begin{align}\label{eq:fk-to-zk}
        \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i \geq z_k
    \end{align}

    Now, consider \eqref{eq:compact-OP} that was solved in iteration $t$.
    By Observation \ref{obs:retSol-solves-any-t}, $\retSol$ is feasible to this problem.
    As $y$'s $(k-1)$ least objective values are at least as high as those of $\retSol$, it is easy to conclude the $y$ satisfies constraint $(\Tilde{2})$ of this problem; since, for any $\ell < k$:
    \begin{align*}
        \sum_{i=1}^{\ell} \valBy{i}{y} \geq\sum_{i=1}^{\ell} \valBy{i}{\retSol} \geq \sum_{i=1}^{\ell} z_i
    \end{align*}
    Therefore, by Observation \ref{obs:feasi-and-constraint2}, $y$ is also feasible to this problem.
    
    However, the approximation obtained for this problem during the algorithm run is $z_k$, and so, the optimal value is at most $\frac{1}{(1-\multError)}\left(z_k+\additiveError\right)$.
    But, as we shall see, the objective $y$ yields in this problem, $\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i$ (by Observation \ref{obs:obj-value}), is higher than this value, which is of course a contradiction:
    \begin{align*}
        &\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i=\sum_{i=1}^{k-1} \valBy{i}{y} - \sum_{i=1}^{k-1} z_i + \valBy{k}{y}\\
        &\geq \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \valBy{k}{y} && \text{$y$'s definition for $j<k$}\\
        &> \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1}{(1 - \lambda_n \multError)} \left(\valBy{k}{\retSol} + (1+\multError)\additiveError \right) && \text{$y$'s definition for $k$}\\
        &= \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1-\multError +\multError^2(1-\multError^{n})}{(1-\multError)^2} \valBy{k}{\retSol}\emark{+\frac{1+\multError}{1-\multError}\additiveError} && \text{equitation \ref{equ:mu}}\\
        &\geq\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1}{1-\multError} \valBy{k}{\retSol} + \frac{\multError}{1-\multError}\left(\sum_{i=1}^{k-1}\valBy{i}{\retSol} - \sum_{i=1}^{k-1}z_i\emark{-\additiveError}\right) \emark{+\frac{1+\multError}{1-\multError}\additiveError} && \text{Lemma \ref{lemma:fk-to-all}}\\
        & = \frac{1}{1-\multError} \left(\sum_{i=1}^k \valBy{k}{\retSol} - \sum_{i=1}^{k-1}z_i\right) \emark{+\frac{1}{1-\multError}\additiveError} \geq \frac{1}{1-\multError} z_k \emark{+\frac{1}{1-\multError}\additiveError} && \text{equation \ref{eq:fk-to-zk}}
    \end{align*}
\end{proof}


\iffalse
Finally, to complete the picture, the following is an example that shows that the algorithm need not output a $(1-\multError)$ approximate leximin.
Consider the following example with $n=2$:
    \begin{align*}
        \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
        s.t. \quad  & x_1 \leq 100\\
                    & x_1 + x_2 \leq 200\\
                    & x \in \mathbb{R}^2_{+}
    \end{align*}
    Consider a run of the algorithm with \textsf{OP} that is a $(1-\multError)$ approximate solver, for $\multError=0.1$. 
    In the first iteration, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
    Then, in the second iteration, given $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained with  $x_1=x_2=94.5$.  
    \erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}
    But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,94.5)$ is \emph{not} a $0.9$ approximation of $(94.5,105.5)$.
    \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5) \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition 
    $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}
\fi


==> files/backups/algo-without-eps.tex <==

\section{Approximation Algorithm}\label{sec:algo-short}
We now present an algorithm for computing a multiplicative approximate leximin \eden{optimal?}. The algorithm is an adaptation of one of the algorithms of \textcite{Ogryczak_2006} for finding exact Leximin solutions. 

% \eden{yonatan}
% Following the \emph{definition} of Leximin, the core \emph{algorithm} for finding a Leximin optimal solution is interative, wherein one first maximizes the least objective function, then the second, and so forth. 
% Specifically, donating by $z_i$ the $i$-th smallest objective value, in each iteration, $t$, one seeks to maximize $z_t$, given the already calculated optimal values for $z_1,\ldots,z_{t-1}$.  The core, single-valued, optimization problem is thus:
%
% \eden{erel} 
% Following the definition of leximin, the core algorithm for finding a leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
% Denote by $z_t$ the value of the $i$-th smallest objective in the leximin-optimal solution, where $t\in\{1,\ldots,n\}$. Suppose we have already computed the optimal values $z_1,\ldots, z_{t-1}$. \eden{I'm not sure about it.. since we use the $z_t$ value later as the \textbf{approximation} value I think it could be a bit confusing}
% Then,  $z_t$ is the solution to the following single-objective optimization problem (where the variables are the scalar $z$ and the vector $x$):

\eden{how is this? I tried to combine the two versions}
Following the definition of Leximin, the core algorithm for finding a Leximin optimal solution is iterative, wherein one first maximizes the least objective function, then the second, and so forth. 
In each iteration, $t=1,\ldots,n$, it looks for the value that maximizes the $t$-th smallest objective, $z_t$, given that for any $i < t$ the $i$-th smallest objective is at least $z_i$ (the value that was computed in the $i$-th iteration).
The core, single-objective optimization problem is thus:
\begin{align}
 \max \quad &\ztVar{x}  \;\;
        s.t. &\quad  & (1) \quad x \in S  \tag{P1}\label{eq:basic-OP}\\
              &     & & (2) \quad \valBy{\ell}{x}\geq z_{\ell} & \ell = 1,\ldots,t-1\nonumber \\
               &    & & (3) \quad \valBy{t}{x} \geq \ztVar{x} \nonumber   
\end{align} 
where the variables are the scalar $\ztVar{x}$ and the vector $x$, and $z_1, \ldots z_{t-1}$ are constants.

Suppose we are given a procedure $\textsf{OP}(z_1,\ldots,z_{t-1})$, which, given  $z_1,\ldots,z_{t-1},$ outputs $(x,z)$ that is the exact optimal solution to \eqref{eq:basic-OP}.  
Then, the \emph{leximin} optimal solution is obtained by iterating this process for $t=1,\ldots,n$, as described in Algorithm \ref{alg:basic-ordered-Outcomes}.
\begin{algorithm}[!tbp]
\caption{The Ordered Outcomes Algorithm}
\label{alg:basic-ordered-Outcomes}
\begin{algorithmic}[1] %[1] enables line numbers
\FOR{$t=1$ to n}
\STATE \( %\begin{align*}
(x_t,z_t)\leftarrow \textsf{OP}(z_1,\ldots,z_{t-1})
\) %\end{align*} 
\ENDFOR
\STATE return $(z_1,\ldots,z_n)$ 
\end{algorithmic}
\end{algorithm}

However, it might be difficult to solve the problem \eqref{eq:basic-OP} as is, since constraints (2) and (3) are not linear even with respect to the objective-functions. 
\erel{I suggest to move P2-Compact here: it is a natural step between P1 and P2.}
\eden{}
 Thus, \cite{Ogryczak_2006} suggest using a variant of the problem that considers sums instead of individual values, which described as follows (similarly, the variables are $\ztVar{x}$ and $x$, and $z_1, \ldots z_{t-1}$ are constants):  
% \eden{maybe we should say it is not a linear program \textbf{with respect to the objective functions}?}
% \erel{I agree. Since the objective functions themselves may be non-linear.}
\begin{align*}
    \max \quad &\ztVar{x} \tag{P2}\label{eq:sums-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                    & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
Here, the constraints $(2)$ and $(3)$ are replaced with constraints $(\hat{2})$ and $(\hat{3})$, respectively. 
Constraint $(\hat{2})$ says that for any $\ell<t$, the sum of any $\ell$ objective functions is at least the sum of the first $\ell$ $z_i$'s. Similarly, $(\hat{3})$ says that the sum of any $t$  objective functions is at least the $t$ first $z_i$'s.  So, since we seek to maximize $z_t$, the optimal solution to \eqref{eq:sums-OP} and \eqref{eq:basic-OP} are provably identical (as in both $z_i$ is the $i$-th least objective value, see \cite{Ogryczak_2006} for a formal proof \eden{I'm actually not sure which of the papers to cite as I didn't find a formal proof (only the claim in given in \cite{Ogryczak_2006} and in \cite{Ogryczak2004TelecommunicationsND} Theorem 4)}). As such, in Algorithm \ref{alg:basic-ordered-Outcomes}, a solver for \eqref{eq:sums-OP} can be used (instead of for \eqref{eq:basic-OP}), and the algorithm will still output a Leximin optimal solution. 

Alas, while \eqref{eq:sums-OP} is linear with respect to the objective-functions, it has an exponential number of constraints. 
To overcome this problem, \cite{Ogryczak_2006} employ auxiliary variables ($y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$) to obtain a polynomial-sized program that is provably equivalent to \eqref{eq:sums-OP}:\eden{To myself: should explain "equivalent" in more detail, maybe to add the alternative proof}
% (where the variables are $\ztVar{x}$, $x$, and $y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$; and $z_1, \ldots z_{t-1}$ are constants)
\begin{align}
    \max \quad &z_t\tag{P3}\label{eq:vsums-OP}\\
        s.t. \quad  & (1) \quad x \in S \nonumber\\
                    & (2) \quad \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq \sum_{i=1}^{\ell}  z_i && \ell = 1, \ldots,t-1 \nonumber \\
                    & (3) \quad t y_t - \sum_{j=1}^{n} m_{t,j} \geq \sum_{i=1}^{t}  z_i  \nonumber \\
                    & (4) \quad m_{\ell,j} \geq y_{\ell} - f_j(x)  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber \\
                    & (5) \quad m_{\ell,j} \geq 0  && \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber
\end{align}
So, in Algorithm \ref{alg:basic-ordered-Outcomes} using a solver for \eqref{eq:vsums-OP}, the algorithm will output a Leximin optimal solution. 

All of the above is for exact solutions.  
The question is what happens when we consider approximation procedures? It is easy to see that if \textsf{OP} is a $(1-\beta)$ approximation algorithm to \eqref{eq:basic-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-\beta)$ approximation of the Leximin. 
\erel{
To say this, we first have to define the notion of "approximation algorithm". It is known, but we still have to define it formally. Maybe in the "preliminaries" section.
} 
However, for approximations, \eqref{eq:sums-OP}, and the equivalent \eqref{eq:vsums-OP}, are no longer equivalent to \eqref{eq:basic-OP}. Indeed, the following example shows that if \textsf{OP} is a $(1-\beta)$ approximation procedure for \eqref{eq:vsums-OP}, then Algorithm \ref{alg:basic-ordered-Outcomes} may output a solution that is \emph{not} a $1-\beta$ approximation to the leximin.
% \erel{Maybe it is better to move the example to here, to motivate our proof.}
Consider the following multi-objective optimization problem with $n=2$:
\begin{align*}
    \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
    s.t. \quad  & x_1 \leq 100\\
                & x_1 + x_2 \leq 200\\
                & x \in \mathbb{R}^2_{+}
\end{align*}
Accordingly, the problem \eqref{eq:vsums-OP} becomes:
\begin{align*}
    \max \quad &z_t \\
    s.t. \quad  & (1.1) \quad  x_1 \leq 100\\
                & (1.2) \quad  x_1 + x_2 \leq 200\\
                & (1.3) \quad  x \in \mathbb{R}^2_{+}\\
                & (\hat{2}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i && \forall F' \subseteq \allObjFunc, |F'| < t \\
                & (\hat{3}) \quad \sum_{f_i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  && \forall F' \subseteq \allObjFunc, |F'| = t
\end{align*}
The following is a possible run of the algorithm with \textsf{OP} that is a $(1-\beta)$ approximate solver for $\beta=0.1$. 
In the first iteration, $t=1$, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
Then, in the second iteration, $t=2$, given that $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained (for example) with  $x_1=x_2=94.5$.  
\erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}\eden{is it more clear now?}
Since $n=2$, the algorithm ends after this iteration and returns this solution $(94.5,94.5)$.
But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,105.5)\xPreferred{\frac{1}{0.9}}(94.5,94.5)$.
Therefore, by definition, the returned solution $(94.5,94.5)$ is \emph{not} a $0.9$ approximately-optimal solution.
% \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5)  \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition  $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}

 %On the other hand, \eqref{eq:vsums-OP} is the most solvable variant of the problem.  
So, using an approximate solver to \eqref{eq:vsums-OP}, what guarantee can we provide for the overall resulting solution? 
\begin{theorem}
\label{th:main}
Let $\beta<1/2$, and \textsf{OP} be a procedure that outputs a $(1-\beta)$ approximation to \eqref{eq:vsums-OP}. Then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-\frac{\beta}{1-\beta +\beta^2})$-approximate Leximin solution.  
\end{theorem}
\eden{Alternative:}
\begin{theorem}
\label{th:main}
Let $\beta<1/2$, and \textsf{OP} be a procedure that outputs a $(1-\beta)$ approximation to \eqref{eq:vsums-OP}. Then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $(1-\beta-\frac{\beta^2(1-\beta)}{1-\beta+\beta^2})$-approximate Leximin solution.  
\end{theorem}
\eden{To myself: need to check whether the assumption $\beta< 1/2$ can be removed}

\eden{maybe we should also include the proof of the additive variant somewhere? if so. where?}
\erel{
Since the proof is not explicitly mentioned anywhere, I think it is good to include a proof for comparison. Maybe in an appendix.
}
\eden{if we want to do so we should also describe the additive variant definition, maybe to put them both in the appendix? I added appendix \ref{sec:additive}}
The remainder of this section is dedicated to proving the theorem.
To this end, we use another equivalent representation of \eqref{eq:sums-OP}, which was also introduced by \cite{Ogryczak_2006}. 
\erel{This variant should move upwards, between P1 and P2.}
% (here also, the variables are $\ztVar{x}$ and $x$, and $z_1, \ldots z_{t-1}$ are constants)
\begin{align*}
    \max \quad &z_t \tag{P2-compact}\label{eq:compact-OP}\\
        s.t. \quad  & (1) \quad x \in S\\
                    & (\Tilde{2}) \quad \sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell}  z_i && \ell = 1,\ldots, t-1 \nonumber\\
                    & (\Tilde{3}) \quad \sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t}  z_i
\end{align*}
In this program, constraints $(\hat{2})$ and $(\hat{3})$ are replaced by  $(\Tilde{2})$ and $(\Tilde{3})$, respectively.  In  $(\hat{2})$, for each $\ell$, one gives a lower bound on the sum for \emph{any} set of $\ell$ objective functions.  In $(\Tilde{2})$, on the other hand, one only considers the sum of the $\ell$ \emph{smallest} such values.  However, since the constraints set the same lower bound on this sum, the constraints are equivalent.  Similarly for $(\hat{3})$ and $(\Tilde{3})$.  So, \eqref{eq:compact-OP} and \eqref{eq:sums-OP} are equivalent, which, in turn, is equivalent to \eqref{eq:vsums-OP}.  So, in proving the theorem we may assume that \textsf{OP} is an approximation procedure for \eqref{eq:compact-OP}.  This will simplify the proofs.

\erel{*** I do not understand. We say that P1 and P2 are equivalent with an exact solver, but not with an approximate solver. 
Here, we claim that P3 and P2-compact are equivalent, but this is true only with an exact solver. Don't we have to prove that they are equivalent also with an approximate solver? ***}

We denote $\retSol := x_n$ = the solution $x$ attained at the last iteration ($t=n$) of the algorithm. 

Following are some observations regarding the problem \eqref{eq:compact-OP} and the solution $\retSol$ that will be useful later.
First, notice that any solution $x \in S$ that satisfies constraint $(\Tilde{2})$ of \eqref{eq:compact-OP} is feasible to this problem.
This is because any solution $x \in S$ can satisfy constraint $(\Tilde{3})$ with a small enough assignment to the variable $z_t$. \eden{I'm not sure how to explain it....}
\begin{observation}\label{obs:feasi-and-constraint2}
Any solution $x \in S$ that satisfies constraint $(\Tilde{2})$ is feasible to \eqref{eq:compact-OP}.
\end{observation}

Since $\retSol$ is a feasible solution of \eqref{eq:compact-OP} in iteration $n$, and as each
iteration only adds new constraints to $(\Tilde{2})$, it follows that $\retSol$ is also a feasible solution of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$. 
\begin{observation}\label{obs:retSol-solves-any-t}
$\retSol$ is a feasible solution of \eqref{eq:compact-OP} in any iteration $1 \leq t\leq n$.
\end{observation}

Now, consider the problem \eqref{eq:compact-OP} that was solved in iteration $t$.
Here, $z_t$ is a \emph{variable} and $z_1, \ldots z_{t-1}$ are constants.
The objective of this problem is $(\max z_t)$ and the only constraint that includes the variable $z_t$ is constraint $(\Tilde{3})$.
Therefore, rearranging it to $\sum_{i=1}^{t} \valBy{i}{x} - \sum_{i=1}^{t-1}  z_i\geq z_t$, allows us to conclude that the objective value is determined by the left side of this inequality (as $z_k$ is maximized when the inequality turns to equality).
\begin{observation}\label{obs:obj-value}
The objective value obtained by a feasible solution $x$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is $\sum_{i=1}^{t} \valBy{i}{x} - \sum_{i=1}^{t-1}  z_i$.
\end{observation}

Lastly, since the value obtained as a $(1 - \beta)$ approximation for this problem is the \emph{constant} $z_t$, the objective value of any feasible solution is at most $\frac{1}{1-\beta} z_t$.
It is particularly true for $\retSol$ since it is feasible for any iteration $t$ (Observation \ref{obs:retSol-solves-any-t}).
Since its objective is $\sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i$ (Observation \ref{obs:obj-value}) we can conclude:

\begin{observation}\label{obs:obj-xt-to-zt}
    The objective value obtained by $\retSol$ to the problem \eqref{eq:compact-OP} that was solved in iteration $t$ is at most $\frac{1}{1-\beta} z_t$. That is:
    \begin{align*}
        \sum_{i=1}^t \valBy{i}{\retSol} - \sum_{i=1}^{t-1} z_i \leq \frac{1}{1-\beta} z_t
    \end{align*}
\end{observation}

% This conclusion also implies that for any $1 \leq t \leq n$, the solution $(x_t, z_t)$ that that was outputted for \eqref{eq:compact-OP} in iteration $t$, satisfies constraint $(\Tilde{3})$ as equality. That is:
% \begin{observation}\label{obs:equality-xt-zt}
% For any $1 \leq t \leq n$,  $\sum_{i=1}^{t} \valBy{i}{x_t} = \sum_{i=1}^{t}  z_i$.
% \end{observation}



%%%
% OVERALL EXPLANATION
%We first establish our motivation by demonstrating, in Lemma \ref{lemma:not-beta-approx}, that $\retSol$ is not necessarily a $1-\beta$ Leximin approximation.\eden{wasn't sure were to put lemma \ref{lemma:not-beta-approx}, before or after}
% However, we then prove it is actually not that far off, it is a $1-2\beta$ approximation. 
We start by Lemma \ref{lemma:retSol-approx-all-t} \eden{To myself: to do}
Then, Lemmas \ref{lemma:mult-fk-lower-bound}-\ref{lemma:mult-special-z_k-upper-bound} establish a relationship between the $k$-th least objective value at 
% the returned solution ($\retSol$)
$\retSol$
% solution  returned by Algorithm \ref{alg:basic-ordered-Outcomes} ($\retSol$) 
and the value $z_k$. 
% In particular, the main conclusion is that the first is at least $\frac{1-2\beta}{1-\beta}$ of the second.
Theorem \ref{th:main} then uses this relation to prove that the existence of another solution that would be $\frac{1}{1-2\beta}$-preferred over $\retSol$ would lead to a contradiction.

% LEMMAS.
% BLAH BLAH.

\begin{lemma}\label{lemma:beta-vk}
    Let $1 \leq k \leq n$. Then:
    \begin{align*}
        \beta \valBy{k}{\retSol} \geq \biggl(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\biggl) -\beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl) \emark{-\epsilon}
    \end{align*}
\end{lemma}

\begin{proof}
    The claim follows from Observation \ref{obs:obj-xt-to-zt}:
    \begin{align*}
         &\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i \leq \frac{1}{1-\beta} z_k \emark{+\frac{1}{1-\beta}\epsilon}\\
         &\Rightarrow z_k \geq (1-\beta) \biggl(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\biggl)\\
        &\Rightarrow z_k \geq \biggl(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\biggl) - \beta \biggl(\sum_{i=1}^{k} \valBy{i}{\retSol} - \sum_{i=1}^{k-1}  z_i\biggl)\\
        &\Rightarrow \beta \valBy{k}{\retSol} \geq \biggl(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\biggl) -\beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl)
    \end{align*}
\end{proof}


\begin{lemma}\label{lemma:beta-sums-to-diff}
    Let $1 \leq k \leq n$. Then:
    \begin{align*}
        \sum_{i=1}^k \beta^{i} \valBy{k-i+1}{\retSol} \geq \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k} z_i
    \end{align*}
\end{lemma}

\begin{proof}
    The proof is by induction on $k$.
    For $k=1$ the claim follows directly from Lemma \ref{lemma:beta-vk}.
    Assuming that the claim is true for $1,\ldots k-1$, then it is true also for $k$:
    \begin{align*}
        &\sum_{i=1}^k \beta^{i} \valBy{k-i+1}{\retSol} = \beta \valBy{k}{\retSol} + \sum_{i=2}^k \beta^{i} \valBy{k-i+1}{\retSol}\\
        &= \beta \valBy{k}{\retSol} + \sum_{i=1}^{k-1} \beta^{i+1} \valBy{k-(i+1)+1}{\retSol} \\
        &= \beta \valBy{k}{\retSol} + \beta \sum_{i=1}^{k-1} \beta^{i} \valBy{(k-1) -i+1}{\retSol}\\
        &= \beta \valBy{k}{\retSol} + \beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl) && \text{induction assumption}\\
        &\geq \biggl(\sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^k z_i\biggl) -\beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl)  && \text{Lemma \ref{lemma:beta-vk}} \\
        & \quad +  \beta \biggl(\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i\biggl)\\
        &\geq \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k} z_i
    \end{align*}
\end{proof}


\begin{lemma}\label{lemma:fk-to-all}
    Let $1 \leq k \leq n$. Then:
    \begin{align*}
        \frac{1-\beta +\beta^2(1-\beta^{n})}{1-\beta} \valBy{k}{\retSol} \geq \valBy{k}{\retSol} + \beta\biggl(\sum_{i=1}^{k-1}\valBy{i}{\retSol} - \sum_{i=1}^{k-1}z_i\biggl)
    \end{align*}
\end{lemma}

\begin{proof}
First, notice that since $k \geq (k-1)-i+1$ for any $1\leq i \leq k$ and as the function $\valBy{i}$ represents the $i$-th smallest objective value, also:
    \begin{align}\label{eq:increase-by-obj-size}
        \forall 1\leq i \leq k \colon \quad \valBy{k}{\retSol} \geq \valBy{(k-1)-i+1}{\retSol}
    \end{align}
    In addition, consider the geometric series with a first element $1$, a ratio $\beta$, and a length $k-1$. 
    As $\beta \neq 1$, its sum can be described as:
    \begin{align}\label{eq:geometric-series-beta}
        \sum_{i=1}^{k-1} \beta^{i-1} = \frac{1-\beta^k}{1-\beta}
    \end{align}
    
    Now, the claim can be concluded as follows:
    \begin{align*}
        &\frac{1-\beta +\beta^2(1-\beta^{n})}{1-\beta} \valBy{k}{\retSol} = \biggl(1 + \frac{\beta^2(1-\beta^k)}{1-\beta}\biggl) \valBy{k}{\retSol} \\
        &= \valBy{k}{\retSol} + \beta^2 \biggl(\frac{1-\beta^k}{1-\beta} \valBy{k}{\retSol} \biggl)\\
        & = \valBy{k}{\retSol} + \beta^2 \biggl(\sum_{i=1}^{k-1} \beta^{i-1} \valBy{k}{\retSol} \biggl) && \text{equation \ref{eq:geometric-series-beta}}\\
        & \geq \valBy{k}{\retSol} + \beta^2 \biggl(\sum_{i=1}^{k-1} \beta^{i-1} \valBy{(k-1)-i+1}{\retSol} \biggl) && \text{equation \ref{eq:increase-by-obj-size}}\\
        &= \valBy{k}{\retSol} + \beta \sum_{i=1}^{k-1} \beta^{i} \valBy{(k-1)-i+1}{\retSol} \\
        &\geq \valBy{k}{\retSol} + \beta\biggl(\sum_{i=1}^{k-1}\valBy{i}{\retSol} - \sum_{i=1}^{k-1}z_i\biggl) && \text{Lemma \ref{lemma:beta-sums-to-diff}}
\end{align*}
\end{proof}



%------
% thm.

We are now ready to prove the Theorem \ref{th:main}.
\begin{proof}[Proof of Theorem \ref{th:main}]
\eden{should decide whether to keep this part}
We prove a slightly stronger result: the returned solution is a $(1 - \mu \beta)$ approximately-optimal, where $\mu=\frac{1-\beta+\beta(1-\beta^n)}{1-\beta +\beta^2(1-\beta^n)}$.
Notice that since $\beta < 1$, when the numbers of objective $n$ increases and tends to infinity the value of $\beta^n$ tends to zero and therefore $\mu$ tends to $\frac{1-\beta+\beta}{1-\beta +\beta^2} = \frac{1}{1-\beta +\beta^2}$.
Specifically, since $\mu < \frac{1}{1-\beta +\beta^2}$, proving that $\retSol$ is $(1 - \mu \beta)$ approximately-optimal also proves that it is $(1 - \frac{1}{1-\beta +\beta^2} \beta)$ approximately-optimal (by Lemma \ref{lemma:beta1-beta2-approx}).
This gives us a tighter bound on the approximation ratio with respect to $n$ and, at the same time, implies the original claim.

We first prove the following equation that will be helpful later:
\begin{align}\label{equ:mu}
\frac{1}{1 - \mu \beta } = \frac{1-\beta +\beta^2(1-\beta^{n})}{(1-\beta)^2}
\end{align}
This is true because:
\begin{align*}
    & 1 - \mu \beta =  1 - \frac{1-\beta+\beta(1-\beta^n)}{1-\beta +\beta^2(1-\beta^n)}\beta && \text{definition of $\mu$} \\
    & = \frac{1-\beta +\beta^2(1-\beta^n) - \beta(1-\beta)- \beta^2(1-\beta^n)}{1-\beta +\beta^2(1-\beta^{n})}\\
    & = \frac{(1-\beta)^2}{1-\beta +\beta^2(1-\beta^{n})}
\end{align*}
and therefore,
\begin{align*}
    & \frac{1}{1 - \mu \beta } = \frac{1-\beta +\beta^2(1-\beta^{n})}{(1-\beta)^2}
\end{align*}

    Now, suppose by contradiction that $\retSol$ is not a $(1 - \mu \beta)$-approximate Leximin solution.
    By definition, this means there exists a solution $y \in S$  that is $\frac{1}{(1 - \mu\beta)}$-preferred over it.
    That is, there exists an integer $1 \leq k \leq n$ such that:
    \begin{align*}
        \forall j < k \colon &\valBy{j}{y} \geq \valBy{j}{\retSol};\\
        & \valBy{k}{y} > \frac{1}{(1 - \mu\beta)} \cdot \valBy{k}{\retSol}.
    \end{align*}

    Recall that $\retSol$ was obtained in \eqref{eq:compact-OP} that was solved in the last iteration $n$.
    Therefore, $\sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^{k} z_i$ (by constraint $(\Tilde{2})$ if $k<n$ and $(\Tilde{3})$ otherwise).
    Which implies:
    \begin{align}\label{eq:fk-to-zk}
        \sum_{i=1}^k \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i \geq z_k
    \end{align}

    Now, consider \eqref{eq:compact-OP} that was solved in iteration $t$.
    By Observation \ref{obs:retSol-solves-any-t}, $\retSol$ is feasible to this problem.
    As $y$'s $(k-1)$ least objective values are at least as high as those of $\retSol$, it is easy to conclude that $y$ satisfies constraint $(\Tilde{2})$ of this problem.
    Therefore, by Observation \ref{obs:feasi-and-constraint2}, $y$ is also feasible.
    
    However, the approximation obtained for this problem during the algorithm run is $z_k$, and so, the optimal value is at most $\frac{1}{(1-\beta)}z_k$.
    But, as we shall see, the objective $y$ yields in this problem, $\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i$ (by Observation \ref{obs:obj-value}), is higher than this value, which is of course a contradiction:
    \begin{align*}
        &\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i=\sum_{i=1}^{k-1} \valBy{i}{y} - \sum_{i=1}^{k-1} z_i + \valBy{k}{y}\\
        &\geq \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \valBy{k}{y} && \text{$y$'s definition for $j<k$}\\
        &> \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1}{(1 - \mu\beta)} \valBy{k}{\retSol} && \text{$y$'s definition for $k$}\\
        &= \sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1-\beta +\beta^2(1-\beta^{n})}{(1-\beta)^2} \valBy{k}{\retSol} && \text{equitation \ref{equ:mu}}\\
        &\geq\sum_{i=1}^{k-1} \valBy{i}{\retSol} - \sum_{i=1}^{k-1} z_i + \frac{1}{1-\beta} \valBy{k}{\retSol} + \frac{\beta}{1-\beta}\biggl(\sum_{i=1}^{k-1}\valBy{i}{\retSol} - \sum_{i=1}^{k-1}z_i\biggl) && \text{Lemma \ref{lemma:fk-to-all}}\\
        & = \frac{1}{1-\beta} \biggl(\sum_{i=1}^k \valBy{k}{\retSol} - \sum_{i=1}^{k-1}z_i\biggl)  \geq \frac{1}{1-\beta} z_k && \text{equation \ref{eq:fk-to-zk}}
    \end{align*}
\end{proof}


\iffalse
Finally, to complete the picture, the following is an example that shows that the algorithm need not output a $(1-\beta)$ approximate Leximin.
Consider the following example with $n=2$:
    \begin{align*}
        \max \quad &\{f_1(x) := x_1, f_2(x) := x_2\} \\
        s.t. \quad  & x_1 \leq 100\\
                    & x_1 + x_2 \leq 200\\
                    & x \in \mathbb{R}^2_{+}
    \end{align*}
    Consider a run of the algorithm with \textsf{OP} that is a $(1-\beta)$ approximate solver, for $\beta=0.1$. 
    In the first iteration, the optimal value of $z_1$ is $100$, so \textsf{OP} may output $z_1=90$.  
    Then, in the second iteration, given $z_1=90$, the optimal value of $z_2$ is $110$, so \textsf{OP} may output $z_2=99$, which is obtained with  $x_1=x_2=94.5$.  
    \erel{Since the objectives are the $x_i$, how can the objective be $99$ and the $x_i$ be $94.5$?}
    But, $(x_1,x_2) = (94.5,105.5)$ is also a feasible solution, and $(94.5,94.5)$ is \emph{not} a $0.9$ approximation of $(94.5,105.5)$.
    \eden{this is not exactly accurate, we are not talking about solution that are approximation of one another, but about the relation. maybe something like "But, $(94.5,105.5)$ is also a feasible solution, and since $(94.5,105.5) \leximinPreferred_{\frac{1}{0.9}} (94.5,94.5)$, by definition 
    $(94.5,94.5)$ is not a $0.9$-approximation"}
\erel{This example does not seem very tight. Can you play with the numbers to get a tighter upper bound on the approximation ratio?}
\fi


==> files/backups/intro-backup0602.tex <==


\section{Introduction}
% title: real life motivation
As people may have divergent interests and perspectives, making a decision that affects many might be a challenging task. 
For instance, when dividing a set of items, the \emph{best} decision depends on the individuals' preferences. 
If each individual wants a different subset of the items, it is easy to see that giving each one the subset it prefers is the best solution.
However, if everyone wants the same item and wants only that item, perhaps joint ownership or rotation would make more sense.

% technical terms
Such a situation can be described as a \emph{multi-objective optimization problem}, which includes defining the set of possible decisions and the different objectives.
Although the best decision may be determined in several different ways, this paper focuses on \emph{Leximin} optimization  which aims to be less offensive to the poorest ones.
A Leximin optimal solution maximizes the smallest objective, subject to this maximizes the second-smallest objective, and so on.

% Algorithms 
Common algorithms for finding a Leximin optimal solution are iterative, solving one or more single-objective optimization problems at each iteration.
When these problems cannot be solved exactly, and particularly if they are NP-hard, what is the best we can do in the terms of Leximin?




\paragraph{Contributions}
This paper studies the problem of Leximin optimization in multi-objective optimization problems under polynomial time restriction.
It focuses on problems that are NP-hard even for the first objective maximization.
Our contribution can be divided into three parts.
First, a new definition of approximate Leximin is presented, which captures multiplicative errors that are commonly associated with approximation algorithms for NP-hard problems.
The definition has several desirable properties, including that a Leximin optimal solution is also approximately-optimal (for any approximation factor), and that the definition is equivalent to the original one in the absence of errors.
Second, an algorithm is provided that, given a single-objective approximation algorithm, computes such an approximation. 
We prove that the accuracy of the returned solution is linearly related to the accuracy of the single-objective approximation algorithm, and that the error factor is at most doubled when moving from the single-objective to the multi-objective setting. 
Importantly, this holds for any number of objectives. 
Lastly, we apply the method to the problem of stochastic allocations of indivisible goods. 
When agents have submodular utilities, approximating the egalitarian value is NP-hard.
We demonstrate that our method enables extending the \cite{kawase_max-min_2020} $(1-\frac{1}{e})$-approximation algorithm for the egalitarian value to approximating the Leximin to with a factor of $(1-\frac{2}{e})$.




\paragraph{Organization} 
Section \ref{sec:approx-leximin-def} presents the definition of approximate Leximin in the presence of \emph{multiplicative} errors.
An algorithm for computing such an approximation is presented in Section \ref{sec:algo-short}.
The problem of stochastic allocations of indivisible goods is considered in Section \ref{sec:app}.
Lastly, Section \ref{sec:future} concludes with future work.





\input{files/related-work.tex}

==> files/equivalent.tex <==
\section{Equivalent Single-objective Optimization Problems in the Presence of Errors}\label{sec:equivalent-proofs}

Many times, when referring to two optimization problems\footnote{In this section,  we consider only single-objective optimization problems.} as equivalent, one means that they have the same optimal value.
When two problems satisfy this relation, it is clear that in order to obtain an optimal \emph{value}, a solver\footnote{It is assumed that a solver (either approximate or exact) for a single-objective optimization problem returns a solution and its objective value.\eden{maybe to explain it better..}} for one can be used as a solver for the other. 
However, if we are interested in an optimal \emph{solution} that yields this value, a solver that returns an optimal solution for another problem with the same optimal value is not enough\eden{reduction to feasibility problem}.
Moreover, when it comes to approximation, even if we are only concerned about the objective value, an approximate solver for one can no longer be used for the other.
To illustrate, consider the following problems:
\begin{align*}
    (E1) \Hquad &\max\quad x                         &&& (E2)\Hquad &  \max\quad x\\
    &\Hquad s.t.\quad  x \in \{0.9,1\}       &&&& \Hquad s.t.\quad x \in \{0.95,1\} 
\end{align*}    
Both problems have the same optimal objective value $1$.
Now, assume that a multiplicative error of $0.1$ is acceptable.
An approximate solver for the problem $(E1)$ may return the objective value $0.9$, which is not a possible value of $(E2)$; similarly, an approximate solver for the problem $(E2)$ may return the objective value $0.95$, which is not a possible value of $(E2)$.
% Thus, although both problems have the same optimal value, an approximate solver for one problem \emph{cannot} be used as an approximate solver for the other.

In this appendix, we present a new definition of equivalent optimization problems, which requires a stronger relationship.
We prove that, according to our definition, when two optimization problems are equivalent, a solver for one, either exact or approximate, can also be used for the other.

\paragraph{Equivalent problems definition} We say that two (single-objective) optimization problems, $OP1 = (S_1,f_1)$ and $OP2 = (S_2,f_2)$, are \emph{equivalent} if they are from the same type --- either both are maximization problems or both are minimization problems; and there exists a bijection, $B \colon S_1 \to S_2$, mapping each solution of $OP1$, $x \in S_1$, to a unique solution of $OP2$, $B(x) \in S_2$, and they have the same objective value $f_1(x) = f_2(B(x))$.

% It is easy to conclude that this relation is symmetric, reflexive and transitive and therefore it is, indeed, an equivalence relation.
The following observation can be easily concluded by the definition:
\begin{observation}
    The equivalent relation between problems is transitive, reflexive and symmetric.
\end{observation}
% \begin{observation}
%     The equivalent relation between problems is transitive.
% \erel{maybe also argue that it is reflexive and symmetric, so it is an equivalence relation.}
% \end{observation}
% \eden{to explain }

If we are only concerned with the objective value, then the following lemma ensures that an approximate solver for one problem can be applied, as is, to the other (it is not necessary to know what the bijection is):

\begin{lemma}\label{lemma:approx-value-equivalent-prob}
    Let $OP1 = (S_1,f_1)$ and $OP2 = (S_2,f_2)$ be equivalent optimization problems, and let $v_1 \in \mathbb{R}$ be an $(\multApprox,\additiveApprox)$-approximation of the optimal objective value of $OP1$.
    Then, $v_1$ is also an $(\multApprox,\additiveApprox)$-approximation of the optimal objective value of $OP2$.
% \erel{Add that the approximation ratios ($\alpha$,$\epsilon$) is the same}
\end{lemma}

\begin{proof}
    For brevity, we prove the claim only for maximization problems, the proof for minimization problems is similar.
    
    Let $x^*\in S_1$ and $y^*\in S_2$ be optimal solutions of the problems $OP1$ and $OP2$ respectively.
    In order to prove that $v_1$ is an $(\multApprox,\additiveApprox)$-approximation of the optimal objective value of $OP2$, we will show that there is a solution $y \in S_2$ with objective value $v_1$, and also that $v_1 \geq \multApprox f_2(y^*) - \additiveApprox$.

    First, since $v_1$ is an $(\multApprox,\additiveApprox)$-approximation of the optimal objective value of $OP1$, there exists a solution $x \in S_1$ such that $f_1(x) = v_1$ and also $v_1 \geq \multApprox f_1(x^*) - \additiveApprox$.
    By definition of equivalent problems, the corresponding solution to $OP2$ by the bijection, $B(X) \in S_2$, has the same objective value $f_2(B(x)) = v_1$.
    
    In addition, we shall now see that both problems have the same optimal objective value.
    Let $B: S_1\to S_2$ be a bijection as described in the definition of equivalent problems.    
    So $f_1(x^*)=f_2(B(x^*))$, and $f_2(B(x^*))\leq f_2(y^*)$ by optimality of $y^*$, so $f_1(x^*)\leq f_2(y^*)$. By analogous arguments $f_2(y^*)\leq f_1(x^*)$, so in fact $f_1(x^*) = f_2(y^*)$.
    
    Therefore, we can conclude that:
    \begin{align*}
        f_2(B(x)) = v_1 \geq \multApprox f_1(x^*) - \additiveApprox =  \multApprox f_2(y^*) - \additiveApprox
    \end{align*}
    as required.
\end{proof}

% \begin{lemma}\label{lemma:solver-equivalent-prob}
%     Let $OP1 = (S_1,f_1)$ and $OP2 = (S_2,f_2)$ be equivalent optimization problems. Then, in order to approximate the optimal value, an $(\multApprox,\additiveApprox)$-approximate solver for one can be used as an $(\multApprox,\additiveApprox)$-approximate solver for the other.
% % \erel{Add that the approximation ratios ($\alpha$,$\epsilon$) is the same}
% \end{lemma}

% \begin{proof}
%     For brevity, we prove the claim only for maximization problems, the proof for minimization problems is similar.
%     Let $x^*\in S_1$ and $y^*\in S_2$ be optimal solutions of the problems $OP1$ and $OP2$ respectively.
%     Let $B: S_1\to S_2$ be a bijection as described in the definition of equivalent problems.    
%     So $f_1(x^*)=f_2(B(x^*))$, and $f_2(B(x^*))\leq f_2(y^*)$ by optimality of $y^*$, so $f_1(x^*)\leq f_2(y^*)$. By analogous arguments $f_2(y^*)\leq f_1(x^*)$, so in fact $f_1(x^*) = f_2(y^*)$.
%     % , since otherwise one of them is higher, and therefore the bijection can be used to obtain a solution to the second problem with value higher than optimal. \eden{need to rewrite it..}
%     Now, 
%     % without loss of generality, 
%     assume that we have an $(\multApprox, \additiveApprox)$-approximate solver for $OP1$, for some $\multApprox\in(0,1]$ and $\additiveError\geq 0$.
%     That is, the solver returns a solution $x \in S_1$ such that $f_1(x) \geq \multApprox \cdot f_1(x^*) - \additiveError$. 
%     Consider the corresponding solution to $OP2$ by the bijection, $B(X) \in S_2$, we know that $f_1(x_1) = f_2(B(x_1))$.
%     It follows that $B(x)$ is an $(\multApprox, \additiveApprox)$-approximation to $OP2$:
%     \begin{align*}
%         f_2(B(x)) = f_1(x) \geq \multApprox \cdot f_1(x^*) - \additiveError = \multApprox \cdot f_2(y^*) - \additiveError
%     \end{align*}
% \end{proof}

Notice that the approximation value is obtained by the corresponding solution ($B(X)$), and therefore, we can also conclude the following result:
% Therefore, if we also have access to procedures to calculate the bijection and its inverse, then we can use a solver for one problem to find the solution to the other, that is:
\begin{corollary}\label{corollary:solver-equivalent-prob}
    Let $OP1 = (S_1,f_1)$ and $OP2 = (S_2,f_2)$ be equivalent optimization problems, and let $P_{1\to 2}$ be a procedure that, given a solution to $OP1$, returns the corresponding solution to $OP2$.
    Then, an $(\multApprox, \additiveApprox)$-approximate solver for $OP1$ can be used to obtain a \emph{solution} that is an $(\multApprox, \additiveApprox)$-approximation for $OP2$.
\end{corollary}

If the procedure from $OP1$ to $OP2$ operates in polynomial time we say that $OP1$ is \emph{polynomial-time equivalent} to $OP2$. 

\eden{how is the name "polynomial-time equivalent"?}

% \eden{If we will have time: "Further, if the bijection is given and can be calculated in polynomial time, then ....}



\subsection{Relationships Between Single-Objective Problems for Leximin Optimization}
\eden{I'm not sure which title to give}

For clarity, descriptions of all the problems are provided here as well (table \ref{table:prob-des}).

\begin{table}[h!]
\begin{tabular}{l}
\hline
\\
$\begin{aligned}
     \text{(P1)}\Hquad \max \quad &\ztVar{x}  \;\;
        s.t. &\quad  & (1) \quad x \in S \\
              &     & & (2) \quad \valBy{\ell}{x}\geq z_{\ell} & \ell = 1,\ldots,t-1\nonumber \\
               &    & & (3) \quad \valBy{t}{x} \geq \ztVar{x} \nonumber  \\\\
    \text{(P2)}\Hquad\max \quad &\ztVar{x}  \;\;
        s.t. &\quad  & (1) \quad x \in S  \\
        &&& (\hat{2}) \quad \sum_{i \in F'} f_i(x) \geq \sum_{i=1}^{|F'|}  z_i & \forall F' \subseteq [n], |F'| < t \\
        &&& (\hat{3}) \quad \sum_{i \in F'} f_i(x) \geq \sum_{i=1}^{t}  z_i  & \forall F' \subseteq [n], |F'| = t\\\\
     \text{(P3)}\Hquad \max \quad &\ztVar{x}  \;\;
        s.t. &\quad  & (1) \quad x \in S  \\
                    &&& (2) \quad \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq \sum_{i=1}^{\ell}  z_i & \ell = 1, \ldots,t-1 \nonumber \\
                    &&& (3) \quad t y_t - \sum_{j=1}^{n} m_{t,j} \geq \sum_{i=1}^{t}  z_i  \nonumber \\
                    &&& (4) \quad m_{\ell,j} \geq y_{\ell} - f_j(x)  & \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber \\
                    &&& (5) \quad m_{\ell,j} \geq 0  & \ell = 1, \ldots,t,\Hquad j = 1, \ldots,n \nonumber\\\\
    \text{(P2-compact)}& \\
    \max \quad &z_t  \;\;
        s.t. &\quad  & (1) \quad x \in S \\
                    &&& (\Tilde{2}) \quad \sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell}  z_i & \ell = 1,\ldots, t-1 \nonumber\\
                    &&& (\Tilde{3}) \quad \sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t}  z_i\\
\end{aligned}$\\
\\
\hline
\end{tabular}
\caption{Summary description of the problems.}
\label{table:prob-des}
\end{table}


\subsubsection{Equivalence of The Problems \eqref{eq:sums-OP} and \eqref{eq:compact-OP}}\label{sec:prob-sums-and-comp}
we prove that the \emph{identity function} is an appropriate bijection between \eqref{eq:sums-OP} and \eqref{eq:compact-OP}. Therefore, they are polynomial-time equivalent to each other. 

We start by proving the following lemma:
\begin{lemma}\label{lemma:sums-to-comp-constrants}
    For any $x \in S$, any $\ell \in [n]$ and a constant $c \in \mathbb{R}$ the following two conditions are equivalent:
    \begin{align}\label{eq:sums-to-comp-constrants}
         \forall F' \subseteq [n], |F'| = \ell \colon \sum_{i \in F'} f_i(x) &\geq c 
         \\
         \sum_{i=1}^{\ell} \valBy{i}{x}&\geq c 
    \end{align}
\end{lemma}

\begin{proof}
    For the first direction, recall that the values $ \valBy{1}{x}, \dots,  \valBy{\ell}{x}$ were obtained from $\ell$ objective functions (those who yield the smallest value).
    By the assumption, the sum of any set of function with size $\ell$ is at least $c$; therefore, it is true in particular for the functions corresponding to the values $ (\valBy{1}{x})_{i=1}^{\ell}$.
    For the second direction, assume that $\sum_{i=1}^{\ell} \valBy{i}{x}\geq c$.
    Since $ \valBy{1}{x}, \dots,  \valBy{\ell}{x}$ are the $\ell$ smallest values in $\allValues{x}$, we get that:
    \begin{align*}
       \forall F' \subseteq [n],\Hquad |F'| = \ell \colon \quad \sum_{i \in F'}f_i(x) \geq \sum_{i=1}^s \valBy{i}{x}\geq c.
    \end{align*}
\end{proof}

    Now, let $(x,z_t)$ be a solution to \eqref{eq:sums-OP}. 
    As $x$ satisfies constraint (1) of \eqref{eq:sums-OP}), it is also satisfies constraint (1) of \eqref{eq:compact-OP} (as both constraints are the same, $x \in S$).
    In addition, as $x$ satisfies constraint $(\hat{2})$ of \eqref{eq:sums-OP}, for any $\ell \in [t-1]$, 
    \begin{align*}
        \forall F' \subseteq [n], |F'| = \ell \colon \sum_{i \in F'} f_i(x) \geq \sum_{i=1}^{\ell} z_i
    \end{align*}
    by Lemma \ref{lemma:sums-to-comp-constrants}, also $\sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell} z_i$. Therefore, $x$ satisfies constraint $(\Tilde{2})$ of \eqref{eq:compact-OP}.
    Lastly, as $x$ and $z_t$ satisfy constraint $(\hat{3})$ of \eqref{eq:sums-OP}, 
    \begin{align*}
        \forall F' \subseteq [n], |F'| = t \colon \sum_{i \in F'} f_i(x) \geq \sum_{i=1}^{t} z_i
    \end{align*}
    again, by Lemma \ref{lemma:sums-to-comp-constrants} also $\sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t} z_i$.
    So, $x$ ans $z_t$   satisfy constraint $(\Tilde{3})$ of \eqref{eq:compact-OP}.
    Since we saw that $x$ ans $z_t$ satisfy all the constraints of \eqref{eq:compact-OP}, it is feasible to this problem.

    As in both problems the objective value is determined by $z_t$, it is clear that $(x,z_t)$ obtains the same objective value from both \eqref{eq:sums-OP} and \eqref{eq:compact-OP}.

    Therefore, the identity function (i.e., $B((x,z_t)) = (x,z_t)$) is an appropriate bijection and so, the problems are equivalent.



%--------------------------------------------------
\subsubsection{Equivalence of The  problems \eqref{eq:compact-OP} and \eqref{eq:vsums-OP}} We prove that these problems are equivalent by describing an appropriate bijection.
We will also see that this bijection and its inverse can be calculated in polynomial time and therefore, each problem is polynomial-time equivalent to the other.

We start with the following lemma:
\begin{lemma}\label{lemma:comp-to-p3-m-sums}
    For any $x \in S$ and any constant $c \in C$,
    \begin{align*}
        \sum_{j=1}^n \max(0, c - f_j(x) ) = \sum_{j=1}^n \max(0, c - \valBy{j}{x} )
    \end{align*}
\end{lemma}
\begin{proof}
     Let $(\pi_1, \ldots, \pi_n)$ be a permutation of $\{1,\ldots,n\}$ such that $f_{\pi_i}(x) = \valBy{i}{x}$ for any $i \in [n]$ (notice that such permutation exists by the definition of $\valBy{}{}$).
     That is, the value that $f_{\pi_i}$ obtains is the ${\pi_i}$-th smallest one in the multiset of all values $\allValues{x}$.
    Since each element in the sum $\sum_{j=1}^n \max(0, c - f_j(x))$ is affected by $j$ only through $f_j(x)$, the permutation $\pi$ allows us to conclude the following:
    \erel{This argument is not clear}\eden{better?}
    \begin{align*}
        \sum_{j=1}^n \max(0, c -f_j(x)) &= \sum_{j=\pi_1}^{\pi_n} \max(0,c -f_j(x)\\ 
        &= \sum_{j=1}^n \max(0,c -f_{\pi_i}(x)  = \sum_{j=1}^{n} \max(0,c -\valBy{j}{x})
    \end{align*}
\end{proof}



Following is Lemma \ref{lemma:comp-to-p3-mapping}, which describes a function $B$ and proves that it is a mapping from the feasible region of the problem \eqref{eq:compact-OP} to the feasible region of the problem \eqref{eq:vsums-OP}.
Then, Lemma \ref{lemma:comp-to-p3-is-bij} proves that this mapping is a bijection.
Lastly, Lemma \ref{lemma:comp-to-p3-obj} shows that the same objective value is obtained.

\begin{lemma}\label{lemma:comp-to-p3-mapping}
    Let $(x,z_t)$ be a feasible solution  to \eqref{eq:compact-OP}. Then $B((x,z_t)) = (x, z_t, (y_1,\ldots,y_n), (m_{1,1},\ldots,m_{n,n}))$ is a feasible solution to \eqref{eq:vsums-OP}, where
    \begin{align*}
        \quad y_{\ell} &:= \valBy{\ell}{x} \Hquad\forall \ell \in [n], 
        \\
        m_{\ell,j} &:= \max(0,y_{\ell} -f_j(x)) \Hquad \forall \ell \in [n], \Hquad \forall 1 \leq j \leq n 
    \end{align*}
\end{lemma}

\begin{proof}
    First, since $x$ satisfies constraint (1) of \eqref{eq:compact-OP}, it is also satisfies constraint (1) of \eqref{eq:vsums-OP} (as both constraints are the same).
    Also, as $m_{\ell,j} \geq 0$ and $m_{\ell,j} \geq y_{\ell} - f_j(x)$ for any $\ell \in [n]$ and $j \in [n]$, this assignment satisfies constraints (4) and (5) of \eqref{eq:vsums-OP}.
    
    To show that this assignment also satisfies constraints (2) and (3) of problem \eqref{eq:vsums-OP}, we first prove that for any $\ell \in [n]$ and any constant $c \in \mathbb{R}$ this assignment satisfies the following:
    \begin{align}\label{eq:comp-to-p3}
        \sum_{i=1}^{\ell} \valBy{i}{x}\geq c \Hquad \Longrightarrow \Hquad \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq c
    \end{align}
    As $y_{\ell} = \valBy{\ell}{x}$, also  $m_{\ell,j} = \max(0,\valBy{\ell}{x} -f_j(x))$.
    % in this way it is easy to see that $j$ affects $m$ only through $f_j(x)$.
    And so, by Lemma \ref{lemma:comp-to-p3-m-sums}, it can also be described as $\sum_{j=1}^{n} \max(0,\valBy{\ell}{x} -\valBy{j}{x})$.
    Since $\valBy{\ell}{x}$ is the $\ell$-th smallest objective, it is clear that $\valBy{\ell}{x} - \valBy{j}{x} \leq 0$ for any $j > \ell$, and $\valBy{\ell}{x} - \valBy{j}{x} \geq 0$ for any $j \leq \ell$.
    We can now conclude that $\ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq c$:
    \begin{align*}
        &\ell y_{\ell} - \sum_{j=1}^n m_{\ell,j} = \ell \cdot \valBy{\ell}{x} - \sum_{j=1}^n \max(0,\valBy{\ell}{x} -\valBy{j}{x}) \\
        &= \ell \cdot \valBy{\ell}{x} - \sum_{j=1}^{\ell} \max(0,\valBy{\ell}{x} -\valBy{j}{x}) - \sum_{j=\ell+1}^n \max(0,\valBy{\ell}{x} -\valBy{j}{x}) \\
        &= \ell \cdot \valBy{\ell}{x} - \sum_{j=1}^{\ell} \left(\valBy{\ell}{x} -\valBy{j}{x}\right) - \sum_{j=\ell+1}^n 0 = \ell \cdot \valBy{\ell}{x} - \ell \cdot\valBy{\ell}{x} + \sum_{j=1}^{\ell} \valBy{j}{x}\\
        &= \sum_{j=1}^{\ell} \valBy{j}{x} \geq  c \text{~~~by assumption.}
    \end{align*}

    Now, since $x$ satisfies constraint $(\Tilde{2})$ of \eqref{eq:compact-OP}, for any $\ell \in [t-1]$, $\sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell} z_i$ and so by equation \ref{eq:comp-to-p3}, $\ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq  \sum_{i=1}^{\ell} z_i$
    Therefore, this assignment constraint (2) of problem \eqref{eq:vsums-OP}.
    In addition, as $x$ and $z_t$ satisfy constraint $(\Tilde{3})$ of \eqref{eq:compact-OP}, $\sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t} z_i$ and so by equation \ref{eq:comp-to-p3}, \ref{eq:comp-to-p3}, $t y_{t} - \sum_{j=1}^n m_{t,j}\geq  \sum_{i=1}^{t} z_i$.
    This means that also satisfies constraints (3) of problem \eqref{eq:vsums-OP}.
\end{proof}

\begin{lemma}\label{lemma:comp-to-p3-is-bij}
    The mapping $B$ is a bijection.
\end{lemma}

\begin{proof}
    Injective ($B(a) = B(b) \Rightarrow a = b$) is trivial since $x$ and $z_t$ are part of the solution.
    
    To prove that the mapping is surjective, we will show that for any feasible solution to \eqref{eq:vsums-OP}, that is,
    \begin{align*}
        (x \in S, z_t, y_1, \ldots, y_t, m_{1,1}, \ldots, m_{1,n}, m_{2,1}, \ldots, m_{2,n},\ldots, m_{t,1}, \ldots, m_{t,n})
    \end{align*}
    there is a feasible solution to \eqref{eq:compact-OP} that is  mapped to this solution.
    In fact, we prove that $(x,z_t)$ does.

    It is easy to see that since $x$ satisfies constraint (1) of \eqref{eq:vsums-OP}, it is also satisfies constraint (1) of \eqref{eq:compact-OP} (as both are the same).
    To show that it also satisfies constraints $(\Tilde{2})$ and $(\Tilde{3})$ of \eqref{eq:compact-OP}, we start by proving that for any $\ell \in [n]$ and any constant $c \in \mathbb{R}$:
    \begin{align}\label{eq:p3-to-comp}
         \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq c
         \Hquad \Longrightarrow \Hquad \sum_{i=1}^{\ell} \valBy{i}{x}\geq c
    \end{align}
    Notice that, for any $j\in [n]$ and any $\ell \in [n]$, $m_{\ell,j} \geq y_{\ell} - f_j(x)$ by constraint (4) of \eqref{eq:vsums-OP}, and also $m_{\ell,j} \geq 0$ by constraint (5) of \eqref{eq:vsums-OP}.
    Therefore, $m_{\ell,j} \geq \max(0,y_{\ell} -f_j(x))$.
    And so, by Lemma \ref{lemma:comp-to-p3-m-sums}:
    \begin{align}\label{eq:p3-to-conp-m-sum}
        \sum_{j=1}^n m_{\ell,j} \geq  \sum_{j=1}^n \max(0,y_{\ell} -f_j(x)) = \sum_{j=1}^n \max(0,y_{\ell} -\valBy{j}{x})
    \end{align}
    Now, suppose by contradiction that $\ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq c$ but at the same time $\sum_{i=1}^{\ell} \valBy{i}{x}< c$ (equation \ref{eq:p3-to-comp}).
    Since $\ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq c$, by equation \ref{eq:p3-to-conp-m-sum} also:
    \begin{align*}
        c \leq \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j} \leq \ell y_{\ell} - \sum_{j=1}^n \max(0,y_{\ell} -\valBy{j}{x})
    \end{align*}
    But, as $\sum_{i=1}^{\ell} \valBy{i}{x}< c$ this lead to contradiction:
\begin{align*}
       &\sum_{i=1}^{\ell} \valBy{i}{x} < c \leq \ell y_{\ell} - \sum_{j=1}^n \max(0,y_{\ell} -\valBy{j}{x})\\
       \Rightarrow \Hquad & \ell y_{\ell} - \sum_{i=1}^{\ell} \valBy{i}{x} - \sum_{j=1}^n \max(0,y_{\ell} -\valBy{j} {x}) > 0\\
       \Rightarrow \Hquad & \sum_{i=1}^{\ell} y_{\ell} - \sum_{i=1}^{\ell} \valBy{i}{x} - \sum_{j=1}^n \max(0,y_{\ell} -\valBy{j} {x}) > 0\\
       \Rightarrow \Hquad & \sum_{i=1}^{\ell}\left( y_{\ell} - \valBy{i}{x} \right) - \sum_{j=1}^{\ell} \max(0,y_{\ell} -\valBy{j} {x}) - \sum_{j=\ell+1}^n \max(0,y_{\ell} -\valBy{j} {x}) > 0\\
        \Rightarrow \Hquad &  \sum_{j=1}^{\ell} \underbrace{\left((y_{\ell} - \valBy{j}{x}) - \max(0,y_{\ell} -\valBy{j}{x})\right)}_{\text{each element } \leq 0} - \sum_{j=\ell+1}^n \underbrace{\max(0,y_{\ell} -\valBy{j}{x})}_{\text{each element } \geq 0} >  0\\
     \Rightarrow \Hquad & 0 > 0
   \end{align*}

    Now, as constraint (2) of problem \eqref{eq:vsums-OP} is satisfied, for any $\ell \in [t-1]$,  $\ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq  \sum_{i=1}^{\ell} z_i$, and so by equation \ref{eq:p3-to-comp}, also $\sum_{i=1}^{\ell} \valBy{i}{x} \geq \sum_{i=1}^{\ell} z_i$.
    This implies that $x$ satisfies constraint $(\Tilde{2})$ of \eqref{eq:compact-OP}.
    Similarly, as constraint (3) of problem \eqref{eq:vsums-OP} is satisfied,  $t y_{t} - \sum_{j=1}^n m_{t,j}\geq  \sum_{i=1}^{t} z_i$, and so by equation \ref{eq:p3-to-comp}, also $\sum_{i=1}^{t} \valBy{i}{x} \geq \sum_{i=1}^{t} z_i$.
    This implies that $x$ and $z_t$ satisfy constraint $(\Tilde{3})$ of \eqref{eq:compact-OP}.
\end{proof}


\begin{lemma}\label{lemma:comp-to-p3-obj}
    $(x,z_t)$ and $B((x,z_t))$ obtain the same objective value from the problems \eqref{eq:compact-OP} and \eqref{eq:vsums-OP} respectively.
\end{lemma}

\begin{proof}
    As in both problems the objective value is determined by $z_t$, by the definition of $B$ (the variable $z_t$ is mapped to itself), it is clear that $(x,z_t)$ and $B((x,z_t))$ obtains the same objective value from \eqref{eq:compact-OP} and \eqref{eq:vsums-OP} respectively.
\end{proof}


%--------------------------------------------------
\subsubsection{Relationship Between the Problems \eqref{eq:basic-OP} and \eqref{eq:sums-OP}} 
% Both problems are depended on a set of constants $z_1, \ldots, z_{t-1}$, 
We shall now prove Lemma \ref{lemma:alg-1-can-use-sums-exact} (Section \ref{sec:algo-short}), which says that in Algorithm \ref{alg:basic-ordered-Outcomes}, a solver for \eqref{eq:sums-OP} can be used (instead of for \eqref{eq:basic-OP}), and the algorithm will still output a leximin optimal solution.

\begin{proof}[Proof of Lemma \ref{lemma:alg-1-can-use-sums-exact}]
    Contrariwise, suppose that the returned solution, $x^*$, is not leximin optimal.
    This means that there exists a solution, $y \in S$, that leximin-preferred over it.
    That is, there exists an integer $k \in [n]$ such that:
    \begin{align*}
        \forall j < k \colon &\valBy{j}{y} = \valBy{j}{\retSol};\\
        & \valBy{k}{y} > \valBy{k}{\retSol}.
    \end{align*}
    In addition, since $x^*$ is the returned solution, it is the solution of \eqref{eq:sums-OP} that was solved in the last iteration and therefore $\sum_{i=1}^{s} \valBy{i}{s} \geq \sum_{i=1}^{s} z_i$ for any $s \in [n]$ (by constraint  $(\hat{2})$ for $s<n$ and constraint  $(\hat{3})$ for $s=n$).
    Now, consider \eqref{eq:sums-OP} that was solved in iteration $t$.
    Since $y$ is a solution ($y \in S$) it satisfies constraint (1).
    It is also easy to see that $y$ satisfies constraint $(\hat{2})$ --- for any $s \in [k-1]$:
    \begin{align*}
        &\sum_{i=1}^s \valBy{i}{y} = \sum_{i=1}^s \valBy{i}{\retSol}
        && \text{since } i\leq s<k \text{ and $y$'s def.}\\
        & \geq \sum_{i=1}^s z_i
    \end{align*}
    Moreover, since $z_t$ is a variable in this problem, it satisfies constraint $(\hat{3})$ with any $z_t \geq \sum_{i=1}^t \valBy{i}{y} - \sum_{i=1}^{t-1} z_i$.
    Therefore, it is feasible to this problem. 
    But, the objective value obtained by $y$ is higher than the optimal value, $z_t$, which is a contradiction:
    \begin{align*}
        \sum_{i=1}^t \valBy{i}{y} - \sum_{i=1}^{t-1} z_i > \sum_{i=1}^t \valBy{i}{x^*} - \sum_{i=1}^{t-1} z_i \geq \sum_{i=1}^t z_t - \sum_{i=1}^{t-1} z_i = z_t
    \end{align*}
\end{proof}
% We start by proving that, for $t \in [n]$, when the constants $z_1, \ldots, z_{t-1}$ represent the optimal values of \eqref{eq:basic-OP} in iterations $1, \ldots t$ respectively, the programs \eqref{eq:basic-OP} and \eqref{eq:sums-OP} are equivalent.

\eden{alternative: is this better?
\begin{proof}
    In Section \ref{sec:algo-sec-proofs}, it was proven that if Algorithm \ref{alg:basic-ordered-Outcomes} uses an $(\multApprox, \additiveApprox)$-approximate solver for \eqref{eq:compact-OP} as \textsf{OP}, then the returned solution is an $(\multApprox, \additiveApprox)$-approximation to leximin. 
    This means that, given an exact solver to \eqref{eq:compact-OP}, the algorithm will output a leximin optimal solution.
    However, we saw that \eqref{eq:sums-OP} and \eqref{eq:compact-OP} are equivalent and that the identity function is an appropriate bijection (Section \ref{sec:prob-sums-and-comp}).
    Therefore, in each iteration, a solver for \eqref{eq:sums-OP} will output the same solution and the same result will be obtained.
\end{proof}
}

\eden{in the next version we can also prove it in a maybe more interesting way.. that when the constants $z_1, \ldots, z_{t-1}$ represent the optimal values of \eqref{eq:basic-OP} the programs are equivalent}

==> files/extras/additive-var.tex <==
\section{Additive Variant}\label{sec:additive}

\begin{theorem}\label{thm:leximin-approx-alg-leximin-opt}
    Let $\epsilon \in [0,1]$ and \textsf{OP} be a procedure that outputs a $\epsilon$ \emph{additive} approximation to \eqref{eq:vsums-OP}. Then Algorithm \ref{alg:basic-ordered-Outcomes} outputs a $\epsilon$ additive-approximate Leximin solution.  
\end{theorem}

\begin{proof}
    Contrariwise, suppose that $\retSol$ is not an $\epsilon$-approximately Leximin-optimal solution.
    This means that there exists a solution $y$ that is $\epsilon$-preferred over $\retSol$.
    That is, there exists an integer $k \in [n]$ such that:
    \begin{align*}
        \forall j < k \colon &\valBy{j}{y} \geq \valBy{j}{\retSol};\\
        & \valBy{k}{y} > \valBy{k}{\retSol} + \epsilon.
    \end{align*}
    We get that for all $s \in [k-1]$:
    \begin{align*}
         &\sum_{i=1}^s \valBy{i}{y} \geq \sum_{i=1}^s \valBy{i}{\retSol}
        && \text{since } i\leq s<k \text{ and $y$'s def.}\\
        & \geq \sum_{i=1}^s z_i && \text{constraint (2) for $t=n$.}
    \end{align*}
    Therefore, $y$ is a solution to the OP that was solved when $t = k$.
    \erel{You proved that $y$ satisfies constraint (2), but what about constraint (3)?}
    \eden{I'm not sure how to explain that constraint (3) is not a \textbf{standard} constraint. It determines the objective value $z$, so although it is not always optimal, it is always valid.}
    
    In addition, either $k<n$ or $k=n$. 
    If $k<n$ then constraint (2) for $t=n$ says that:
    \begin{align}\label{equ:approx-sum-k-geq-z-1}
        \sum_{i=1}^k \valBy{i}{\retSol} \geq \sum_{i=1}^k z_i
    \end{align}
    If $k=n$ then since $z=z_n$ constraint (3) says it.
    In both cases, we know that equation \ref{equ:approx-sum-k-geq-z-1} holds.
    
    And so, we get that:
    \begin{align*}
         \sum_{i=1}^k \valBy{i}{y} &= \sum_{i=1}^{k-1} \valBy{i}{y} + \valBy{k}{y}\\
         &  \geq\sum_{i=1}^{k-1}\valBy{i}{\retSol} + \valBy{k}{y} &&  \text{since } i \leq k-1 < k \text{ and $y$'s def.}\\
        & > \sum_{i=1}^{k-1}\valBy{i}{\retSol} + \valBy{k}{\retSol} + \epsilon &&  \text{$y$'s def. for } k
        \\
        & = \sum_{i=1}^{k}\valBy{i}{\retSol} + \epsilon \\
        & \geq \sum_{i=1}^{k} z_i + \epsilon &&  \text{equation } \ref{equ:approx-sum-k-geq-z-1}
    \end{align*}
    Which simply means that:
    \begin{align}\label{equ:sum-y-geq-sum-z-plus-eps}
         \sum_{i=1}^k \valBy{i}{y} > \sum_{i=1}^{k} z_i +\epsilon
    \end{align}
    That means that the $z$ achieved by the solution $y$ in the OP that was solved when $t = k$ is strictly more than the value we achieved $z_k$ plus $\epsilon$:
    \begin{align*}
        &\sum_{i=1}^k \valBy{i}{y} - \sum_{i=1}^{k-1} z_i && \text{insulated } z\\
        &> \sum_{i=1}^{k} z_i + \epsilon - \sum_{i=1}^{k-1} z_i  && \text{equation } \ref{equ:sum-y-geq-sum-z-plus-eps} \\
        &= z_k + \epsilon
    \end{align*}
    But we know that the error in this OP is at most $\epsilon$ --- a contradiction.
\end{proof}

==> files/extras/ellipsoid-variant-through-the-constraints.tex <==

\section{Ellipsoid Method Variant for Approximation}\label{sec:mult-variant-ellipsoid}
This Appendix describes a variant of the ellipsoid method that can be used to approximate  LPs that cannot be solved directly due to a large number of variables.
% It requires an approximate separation oracle for the dual program.
The method combines techniques presented in \cite{grotschel_geometric_1993,grotschel_ellipsoid_1981,karmarkar_efficient_1982}.

\subsection{Using Approximate Separation Oracles (multiple error)}
Our goal is to solve the following linear program (the primal):
\begin{align}
\tag{P}
\begin{split}
\min \quad &c^T \cdot x \\
s.t. \quad &A \cdot x \geq b, \quad x\geq 0;
\end{split}
\end{align}
We assume that (P) has a small number of constraints, but may have a huge number of variables, so we cannot solve (P) directly. We consider its \emph{dual}:
\begin{align}
\tag{D}
\begin{split}
\max \quad & b^T \cdot y \\
s.t. \quad &A^T \cdot y \leq c,\quad y\geq 0.
\end{split}
\end{align}
Assume that both problems have optimal solutions and denote the optimal solutions of (P) and (D) by $x^{*}$ and $y^{*}$ respectively. By the strong duality theorem:
\begin{align}
    c^T \cdot x^{*} = b^T \cdot y^{*}
\end{align}

While (D) has a small number of variables, it has a huge number of constraints, so
we cannot solve it directly either. 
In this Appendix, we show that (p) can be approximated using the following tool:

\begin{definition}
An \emph{approximate separation oracle} with multiplicative error (MASO) for the dual LP is an efficient function parameterized by a constant $\multError \geq 0$.
Given a vector $y$  it returns one of the following two answers:
\begin{enumerate}
\item "$y$ is infeasible". In this case, is returns a violated constraint, that is, a row $a_i^T \in A^T$ such that $a_i^T  y > c_i$.
\item "$y$ is \emph{approximately feasible}". 
That means that $A^T y \leq (1+\multError) \cdot c$
\end{enumerate}

\end{definition}
Given the MASO, we apply the ellipsoid method as follows (this is just a sketch
to illustrate the way we use the MASO; it omits some technical details):
\begin{itemize}
    \item Let $E_0$ be a large ellipsoid, that contains the entire feasible region, that is, all $y \geq 0$ for which $A^T y \leq c$.

    \item For $k = 0,1,\dots, K$ (where $K$ is a fixed constant, as will be explained later):
    \begin{itemize}
        \item Let $y_k$ be the centroid of ellipsoid $E_k$.
        
        \item Run the MASO on $y_k$.
        
        \item If the MASO returns "$y_k$ is infeasible" and a violated constraint $a_i^T$, then make a \emph{feasibility cut} --- keep in $E_{k+1}$ only those $y \in E_k$ for which $a_i^T y \leq c_i$.
        
        \item If the MASO returns "$y$ is approximately feasible", then make an \emph{optimality cut} --- keep in $E_{k+1}$ only those $y \in E_k$ for which $b^T y \geq b^T y_k$.
    \end{itemize}
    
    \item From the set $y_0, y_1, \dots, y_K$, choose the point with the highest $b^T \cdot y_k$ among all the approximately-feasible points.
\end{itemize}
Since both cuts are through the center of the ellipsoid, the ellipsoid dilates by a factor of at least $\frac{1}{r}$ at each iteration, where $r > 1$ is some constant (see \cite{grotschel_ellipsoid_1981} for computation of $r$). Therefore, by choosing $K := \log_2 r \cdot L$, where $L$ is the
number of bits in the binary representation of the input, the last ellipsoid $E_K$ is so small that all points in it can be considered equal (up to the accuracy of the binary representation).


The solution $y'$ returned by the above algorithm satisfies the following two conditions:
\begin{equation} \label{mult:y-star-is-approximetly-feasible}
     A^T y' \leq (1+\multError)\cdot c
\end{equation}
\begin{equation} \label{mult:y-star-obj-geq-opt}
     b^T y' \geq b^T y^{*}
\end{equation}
Inequality \eqref{mult:y-star-is-approximetly-feasible} holds since, by definition, $y'$ is approximately-feasible.

To prove \eqref{mult:y-star-obj-geq-opt}, suppose by contradiction that $b^T y^{*} > b^T y'$. 
Since $y^{*}$ is feasible for (D), it is in the initial ellipsoid. 
It remains in the ellipsoid throughout the algorithm: it is removed neither by a feasibility cut (since it is
feasible), nor by an optimality cut (since its value is at least as large as all values used for optimality cuts).
Therefore, it remains in the final ellipsoid, and it is chosen as the highest-valued feasible point rather than $y'$ --- a contradiction.

Now, we construct a reduced version of (D), where there are only at most $K$ constraints --- only the constraints used to make feasibility cuts.
Denote the reduced constraints by $A_{red}^T \cdot y \leq c_{red}$, where $A_{red}^T$ is a matrix containing a subset of at most $K$ rows of of $A^T$, and $c_{red}$ is a vector containing the corresponding subset of the elements of $c$. The reduced-dual LP is:
\begin{equation}
\tag{RD}
\begin{split}
\max  \quad & b^T y \\
s.t. \quad & A_{red}^T \cdot y \leq c_{red}, \quad y\geq 0
\end{split}
\end{equation}
Notice that it has the same number of variables as the program (D). Further, if we had run this ellipsoid method variant on (RD) (instead of (D)), then the result would have been exactly the same --- $y'$.
Therefore, \eqref{mult:y-star-obj-geq-opt} holds for the (RD) too:
\begin{equation} \label{mult:y-star-to-y-redopt}
    b^T y' \geq b^T y^{*}_{red}
\end{equation}
where $y^{*}_{red}$ is the optimal value of (RD).


As $A_{red}^T$ contains a subset of at most $K$ rows of $A^T$, the matrix $A_{red}$ contains a subset of \emph{columns} of $A$.
Therefore, the dual of (RD) has only at most $K$ variables, which are those who correspond to the remaining columns of $A$:
\begin{equation}
	\tag{RP}
    \begin{split}
     \min \quad &c_{red}^T \cdot x_{red} \\
            s.t. \quad &A_{red} \cdot x_{red} \geq b, \quad x_{red}\geq 0
    \end{split}
\end{equation}
%  reduced-primal
%\er{Note that $A_{red}$ is a matrix with the same number of rows as $A$, but only at most $K$ columns.}
Since (RP) has a polynomial number of variables  and constraints, it can be solved exactly by any LP solver (not necessarily the ellipsoid method).
Denote the optimal solution by $x^{*}_{red}$. 

Let $x'$ be a vector which describes an assignment to the variables of (P), in which all variables that exist in (RP) have the same value as in $x^{*}_{red}$, and all other variables are set to $0$.It follows that $A \cdot x' = A_{red} \cdot x^{*}_{red}$, therefore, since $x^{*}_{red}$ is feasible to (RP), $x'$ is feasible to (P).
% \erel{
% In second reading, I think this should be made more formal.
% Let $x'$ be a solution to (P), in which all variables that exist in (RP) have the same value as in $x^{*}_{red}$, and all other variables are set to 0.
% We have to prove that 
% (1) $x'$ is feasible for (P);
% (2) $c^T x' \leq (1+\epsilon)\cdot c^T\cdot x^{*}$.
% }
% \eden{better?}
Similarly, $c^T \cdot x' = c^T_{red} \cdot x^{*}_{red}$.
We shall now see that this implies that the objective obtained by $x'$ approximates the objective obtained by $x^{*}$:
% \begin{align*} 
%     &\displayComsoc{\quad}c^T \cdot x' = c^T_{red} \cdot x^{*}_{red} \\
% & \text{By strong duality for the reduced LPs:} \\
%     &\displayComsoc{\quad}=  b^T \cdot y^{*}_{red}\\
%  & \text{By Equation (\ref{mult:y-star-to-y-redopt}):}\\
%      &\displayComsoc{\quad}\leq  b^T\cdot y'\\
%  & \text{By the definition of (P):} \\
%      &\displayComsoc{\quad}\leq  (A \cdot x^{*})^T y'\\
% & \text{By properties of transpose and associativity of multiplication:} \displayComsoc{&& \quad \quad \quad}\\
%      &\displayComsoc{\quad}=  (x^{*})^T (A^T\cdot y') \\
%  & \text{By Equation \eqref{mult:y-star-is-approximetly-feasible}:} \\
%      &\displayComsoc{\quad}\leq  (x^{*})^T ((1+\multError)\cdot c)\\
% & \text{By properties of transpose:}\\
%      &\displayComsoc{\quad} = (1+\multError) \cdot (c^T x^{*})
% \end{align*}

\begin{align*} 
    &c^T \cdot x' = c^T_{red} \cdot x^{*}_{red} \\
& \equWithExp{\text{By strong duality for the reduced LPs}}{=  b^T \cdot y^{*}_{red}}\\
 & \equWithExp{\text{By Equation (\ref{mult:y-star-to-y-redopt})}}{\leq  b^T\cdot y'}\\
 & \equWithExp{\text{By the definition of (P)}}{ \leq  (A \cdot x^{*})^T y'}\\
& \equWithExp{\text{By properties of transpose and associativity of multiplication}} {=  (x^{*})^T (A^T\cdot y')} \\
 & \equWithExp{\text{By Equation \eqref{mult:y-star-is-approximetly-feasible}}}{\leq  (x^{*})^T ((1+\multError)\cdot c)}\\
& \equWithExp{\text{By properties of transpose}}{= (1+\multError) \cdot (c^T x^{*})}
\end{align*}
So, $x'$ ($x^{*}_{red}$ with all missing variables set to $0$) is an approximate solution to the primal LP (P) --- as required.

\subsection{Using Half-Randomized Approximate Separation Oracles}
Here, we allow the oracle to also be \emph{half-randomized}, that is, when it says that a solution is infeasible, it is always correct; however, when it says that a solution is approximately feasible, it is only correct with some probability $p \in [0,1]$.

Since the ellipsoid method variant is iterative, and since the oracle calls are independent, there is a probability $p^T$ that the oracle answers correctly in each iteration, and so, the overall process performs as before. 
We shall now explain why, using a half-randomized oracle, this ellipsoid method variant \emph{always} returns a feasible solution to the primal (even if the oracle was incorrect).

First, notice that the oracle is always correct when it determines that a solution is infeasible.
In addition, the construction of (RD) is entirely determined by these constraints.
Therefore, by the same arguments, $x'$ would still be a feasible solution to P (but not necessarily with an approximately-optimal objective value).

This means that given a half-randomized approximate separation oracle for the dual with error $\multError$ and success probability $p$, this ellipsoid method variant can be used as a randomized approximation algorithm for the primal with the same error and success probability $p^I$ (where $I$ is an upper bound on the number of iteration of the method on the given input).

==> files/extras/other-defs.tex <==
%\newpage
\section{Alternative Definitions}\label{sec:other-definitions-short}
In this section, we discuss other potential definitions of Leximin approximation that might be considered intuitive.
\eden{removed ack. for anonymous submission}
% \footnote{We thank Sylvain Bouveret for suggesting definitions \ref{altDef:5} and \ref{altDef:6}.}.
For each alternative, we provide an example that illustrates why we believe it is inappropriate and a conclusion based on that example.
It should be noted that in order to avoid confusion, the error parameter $\gamma \in (0,1)$ is used in the alternative definitions (instead of $\beta$), to emphasize that these are only alternatives we do not use.


\begin{potentialDefinition}\label{altDef:2}
    A solution $x$ is a $(1-\gamma)$-approximately optimal if given a Leximin-optimal solution, $x^*$, there exists an integer $k \in [n]$ such that: 
    \begin{align*}
    \forall j < k: & \valBy{j}{x} \geq (1-\gamma) \cdot \valBy{j}{x^*}\\
    & \valBy{k}{x} > \valBy{k}{x^*}
    \end{align*}
\end{potentialDefinition}

\paragraph{Bad example def. \ref{altDef:2}:} Consider the following example with three objectives:
\begin{align*}
    \max \quad &\{f_i(x) = x_i \mid \forall 1 \leq i \leq 3 \} \\ \tag{E1}\label{eq:alt-def-eaxmple-1}
    s.t. \quad  & 99 x_1 + x_2 \leq 100\\
    &  x_3 \leq 100\\
    & x \in \mathbb{R}^3_{+}
\end{align*}
The Leximin optimal solution $x^*$ is $(1,1, 100)$ and therefore, by taking $k$ to be $2$, we get that any solution that its minimum objective value is at least $(1-\gamma)$ and its second-smallest objective value is more than $1$ is considered $(1-\gamma)$-approximately optimal Leximin solution.
For instance, consider $\gamma = 0.1$, the solution $(0.9, 1.1, 1.1)$ should be considered a $0.9$-approximately optimal according to this definition.
However, it is easy to see that this solution is quite bad for $f_2$ who can achieve $10.9$ (higher by a factor $> 9$) and very bad for $f_3$ who can achieve $100$ (higher by a factor $>90$).
And so, it seem reasonable to require that a good definition will consider as many objectives as possible.
% \erel{What objective values exactly? Do you mean: as many objectives as possible?}
% \eden{yes. To myself: this comment might be relevant to other places..}

\paragraph{Conclusion def. \ref{altDef:2}:} An appropriate definition should take into account as many objectives as possible.

\begin{potentialDefinition}\label{altDef:1}
    A solution $x$ is a $(1-\gamma)$-approximately optimal if for a Leximin-optimal solution, $x^*$, and for each $j = 1, \dots, n$ the following holds: 
    \begin{align*}
        \valBy{j}{x} \geq (1-\gamma) \cdot \valBy{j}{x^*} 
    \end{align*}
\end{potentialDefinition}

\paragraph{Bad example def. \ref{altDef:1}:} 
% An error in the first objective value might cause the other values to increase significantly.
Consider example \eqref{eq:alt-def-eaxmple-1} again.
Here, as the optimal solution is $(1,1, 100)$, any solution that yields at least $(1-\gamma,1-\gamma, (1-\gamma)\cdot 100)$.
However, considering $\gamma = 0.1$, $f_2$ can again achieve $9.1$ which is higher by a factor $> 100$ than the value it got $0.1$.

\paragraph{Conclusion def. \ref{altDef:1}:} An appropriate definition should consider the fact that an error in one objective might change the optimal value of other objectives.
As a consequence, another conclusion is that an appropriate definition should not consider the optimal solution at all.



\begin{potentialDefinition}\label{altDef:3}
    A solution $x$ is a $(1-\gamma)$-approximately optimal 
    if it satisfies the following requirements:
    \begin{enumerate}
        \item The objective-function with the smallest objective value achieves at least its maximum value times $(1-\gamma)$:
        \begin{align*}
            \valBy{1}{x} \geq (1-\gamma) \cdot \valBy{1}{x^*} 
        \end{align*}
        
        \item Given all the solutions that satisfies the first condition, let $m_2$ be the highest second-smallest objective value.
        The objective-function with the second-smallest objective value achieves at least the $m_2$ times $(1-\gamma)$.
        
        \item Given all the solutions that satisfies the former conditions, let $m_3$ be the highest third-smallest objective value.
        The objective-function with the third-smallest objective value achieves at least the $m_3$ times $(1-\gamma)$.
        
        \item and so on.
    \end{enumerate}
\end{potentialDefinition}

\paragraph{Bad example def. \ref{altDef:3}:}
Consider the following example with only two objectives:
\begin{align*}
    \max \quad &\{f_1(x) = x_1, f_2(x)=x_2\} \\
    s.t. \quad  & 99 x_1 + x_2 \leq 100\\
    & x \in \mathbb{R}^2_{+}
\end{align*}
The Leximin-optimal solution is $(1,1)$. Consider $\gamma = 0.1$, according to part (1) of this definition, all solutions in which the smallest objective value is at least $(1-\gamma)=0.9$ should be considered in order to determine $m_2$.
So, in this case, $m_2$ is determined to be $100 - 0.9 \cdot 99 = 10.9$.
Then, according to part (2), in order to be considered a $0.9$-approximately optimal, the second value must be at least $0.9 \cdot 10.9 = 9.81$.
But, even the exact Leximin optimal solution does not satisfy this requirement, so this cannot be considered an approximation to Leximin optimal.

In general, this definition has the disadvantage of favoring solutions that give the lowest bounds to the objective functions considered in the earlier steps,  since this may enable to increase the values of the higher objectives.
According to the Leximin nature, the most important thing is to make the worst-off player as happy as possible (and then the second worst-off and so on), therefore, we emphasize the importance of this characteristic also in the definition of the approximated version.

\paragraph{Conclusion def. \ref{altDef:3}:} An appropriate definition should also capture the Leximin optimal solutions, and maintain the Leximin nature whenever possible.

% \eden{I think this definition is actually equivalent to our current... need to think about it again}
% \begin{potentialDefinition}\label{altDef:4}
%     A solution $x$ is a $\gamma$-approximately-optimal Leximin solution if it can be viewed as the result of this process:
%     \begin{enumerate}
%         \item Choose a solution in which the objective-function with the smallest objective value achieves at least the maximum value minus $\gamma$:
%         \begin{align*}
%             \valBy{1}{x} \geq \valBy{1}{x^*} - \gamma
%         \end{align*}
%         Let $z_1$ be the value it achieves (i.e., $\valBy{1}{x})$.
        
%         \item Consider all the solutions in which the objective-function with the smallest objective value achieves at least $z_1$ and let $m_2$ be the highest second-smallest objective value.
%         Then, choose a solution in which the objective-function with the second-smallest objective value achieves at least the $m_2$ minus $\gamma$.
%         Let $z_2$ be the value it achieves.
%         \item Consider all the solutions in which the objective-function, the smallest objective value achieves at least $z_1$ and the second-smallest objective value achieves at least $z_2$, and let $m_3$ be the highest third-smallest objective value.
%         Then, choose a solution in which the objective-function with the third-smallest objective value achieves at least the $m_3$ minus $\gamma$.
        
%         \item and so on...
%     \end{enumerate}
% \end{potentialDefinition}

% \paragraph{Bad example def. \ref{altDef:3}:} Although in this definition, the Leximin optimal solution is also approximately-optimal as we wanted, another issue arises.

% \begin{itemize}
%     \item \textbf{Bad example:} two solutions that meet this definition, but one of them is strictly better (by more than $\gamma$) than the other from some point.
%     \item \textbf{Conclusion:} an appropriate (good?) definition should determine between two solutions if possible. 
% \end{itemize}

% -----------------------------------
% \subsection{others}
% (From the correspondence of Erel with Lemaitre and Bouveret)

%----------------------------------
% need to think about a corresponding def for mult...
\begin{potentialDefinition}\label{altDef:5}
    A solution $x$ is a $(1-\gamma)$-approximately optimal if for a Leximin-optimal solution, $x^*$, and for each $j = 1, \dots, n$: 
    % in the addive version was $$$
    \begin{align*}
        % |\valBy{j}{x} - \valBy{j}{x^*}| \leq \gamma\\
         \max\{\valBy{j}{y},\valBy{j}{x}\}  \leq \frac{1}{1-\gamma} \cdot \min\{\valBy{j}{y},\valBy{j}{x}\}
    \end{align*}
\end{potentialDefinition}

\paragraph{Bad example and conclusion def. \ref{altDef:5}:}
This definition is close to definition \ref{altDef:1} but weaker, still the same example and conclusion apply.

\begin{potentialDefinition}\label{altDef:6}
    A solution $x$ is a $(1-\gamma)$-approximately optimal if given a Leximin-optimal solution, $x^*$, there exists an integer $k \in [n]$ such that: 
    \begin{align*}
    \forall j < k: & \valBy{j}{x} = \valBy{j}{x^*}\\
    & \valBy{k}{x} > (1-\gamma) \cdot \valBy{k}{x^*}
    \end{align*}
\end{potentialDefinition}
% \eden{I'm not sure it is well defined, since by decreasing $\gamma$ (for example) the second value might become smaller than the first.}

\paragraph{Bad example def. \ref{altDef:6}:} As in the case of definition \ref{altDef:2}, by taking a small $k$, we cannot distinguish between two solutions that satisfy this definition, but one of them should be definitely preferred.
Consider again the following example with three objectives, where:
\begin{align*}
    \max \quad &\{f_i(x) = x_i \mid \forall 1 \leq i \leq 3 \} \\
    s.t. \quad  & 9 x_1 + x_2 \leq 10\\
    &  x_3 \leq 100\\
    & x \in \mathbb{R}^3_{+}
\end{align*}
The Leximin optimal solution $x^*$ is $(1,1, 100)$ and therefore, by taking $k$ to be $2$, we get that any solution that its minimum value is $1$ and its second-smallest objective value is more than $(1-\gamma)$ is considered $(1-\gamma)$-approximately optimal.
As an example, the solution $(1, 1, 1)$ is considered $(1-\gamma)$-approximately-optimal Leximin solution (as $(1-\gamma) < 1$).
But it is easy to see that this solution is quite bad for $f_3$ (who can achieve $100$).

\paragraph{Conclusion def. \ref{altDef:6}:} Same as for def. \ref{altDef:2}, an appropriate definition should take into account as many objectives as possible.

% \begin{potentialDefinition}
%     OWA.
% \end{potentialDefinition}

%--------------------------

\begin{potentialDefinition}\label{altDef:7}
    A solution $x$ is a $(1-\gamma)$-approximately optimal if there is no other solution $y$ that is $(1-\gamma)$-Leximin preferred over it, where this relation is defined as follows: $y$ is preferred over $x$ if  there exists an integer $k \in [n]$ such that:
    \begin{align*}
        \forall j < k \colon \quad &   \max\{\valBy{j}{y},\valBy{j}{x}\}  \leq \frac{1}{(1-\gamma)} \cdot \min\{\valBy{j}{y},\valBy{j}{x}\}\\
        & \valBy{k}{y} > \frac{1}{(1-\gamma)} \cdot 
\valBy{k}{x}
    \end{align*}
     [This relation is related to a one suggested in \cite{kalai_lexicographic_2012}, it is described in more detail in the Related work Section]. 
\end{potentialDefinition}

\paragraph{Bad example and conclusion def. \ref{altDef:7}:} As with definition \ref{altDef:3}, here also, the Leximin optimal solution is not optimal according to this relation and it might favor solutions with lower smallest objective values. 
Consider again the following example:
\begin{align*}
    \max \quad &\{f_1(x) = x_1, f_2(x)=x_2\} \\
    s.t. \quad  & 99 x_1 + x_2 \leq 100\\
    & x \in \mathbb{R}^2_{+}
\end{align*}
Assume that $\gamma = 0.1$, the Leximin-optimal solution is $(1,1)$, but the solution $(0.9,10.9)$ is preferred over it according to this relation (since for $k=2$ we get that $\max\{0.9,1\} \leq \frac{1}{0.9}\cdot\min\{0.9,1\}$ and $10.9 > \frac{1}{0.9} \cdot 1$) and therefore, it is not approximately-optimal.




==> files/extras/saturation-algorithm.tex <==
\section{Saturation Algorithm}\label{sec:saturation-algorithm}
The following algorithm was independently proposed by different researchers for different problems \cite{willson,airiau_portioning_2019,nace_max-min_2008}.
% --- by Willson \cite{willson} for the  problem of fair allocation of divisible items, Airiau et al. \cite{airiau_portioning_2019} for the problem of portioning with ordinal preferences, Bei at el. \cite{bei_truthful_2022} for a variant of cake cutting that they called cake sharing and Nace and Pioro \cite{nace_max-min_2008} for multi-commodity flow problem 
But it can be generalized to capture the following case:
\begin{enumerate}
    \item The feasible region $S$ is \textit{convex}: for any two solutions $x, y \in S$ and for any $\lambda \in [0,1]$, the convex combination of $x$ and $y$ in relation to $\lambda$ is also a solution:
    \begin{align*}
        \forall x, y \in S, \quad \forall \lambda \in [0,1] \colon \quad  
        \bigl(\lambda x + (1-\lambda)y\bigl)\in S
    \end{align*}

    \item The size of the feasible region $S$ is polynomial with respect to $n$.
    % \eden{To myself: to check if this is accurate: i.e., it can be described with a number of variables and constraints that is polynomial to $n$.}

    \item The objective-functions are \textit{additive}: let $x,y,z \in S$ be solutions for which $\alpha,\beta \in \mathbb{R}$ exist such that $z = \alpha x + \beta y$, then for each objective-function $f_i \in \allObjFunc$:
    \begin{align*}
        f_i(z) &= f_i(\alpha x + \beta y) =\\
        &= \alpha f_i(x) + \beta f_i(y)
    \end{align*}
    \erel{ 
    For this condition, we must say that the solutions are vectors (we did not say this so far). Otherwise there is no meaning to adding or multiplying by scalars.
    }

    \item The objective-functions are \textit{concave}: for any objective-function $f_i \in \allObjFunc$ the set $\{f(x) \mid x \in S\}$ is concave (equivalently, the set $\{-f(x) \mid x \in S\}$ is convex). 

    \item There is a black-box for finding  the \textit{next maximin} value (denote by $OP1$): given a subset of objective-functions ($\mathcal{A}\subset \allObjFunc$) for which lower bounds have been set ($\forall f_i \in \mathcal{A} \colon z_i \in \mathbb{R}$), finds the highest value that all other objective functions can achieve simultaneously:
    \begin{align*}
        \max \quad &z\\
        s.t. \quad  & x \in S\\
                    & f_i(x) = z_i   & f_i \in \mathcal{A}\\
                    & f_i(x) \geq z   & f_i \notin \mathcal{A}
    \end{align*}

    \item There is a black-box for solving a saturation test (denote by $OP2$):
    % \eden{I think we should name this process, but I'm not sure if it is the best name...}: 
    For each objective-function $f_k \in \allObjFunc$, a single-objective optimization version of the problem with lower bounds on the values of the other objectives ($\forall f_i \in \mathcal{A} \colon z_i \in \mathbb{R}$ and $z \in \mathbb{R}$):
    \begin{align*}
    \max \quad &f_i(x)\\
    s.t. \quad  & x \in S\\
                    & f_i(x) = z_i   & f_i \in \mathcal{A}\\
                    & f_i(x) \geq z   & f_i \notin \mathcal{A}
    \end{align*}
\end{enumerate}
The algorithm is described in detail (in our terms and notations) in Algorithm \ref{alg:willson-leximin}. 


\begin{algorithm}[!htbp]
\caption{Saturation Algorithm--- for finding the Leximin optimal solution}
\label{alg:willson-leximin}
% \textbf{Input}: A black-box for OP1 and a black-box for OP2\\
% \textbf{Output}: The Lexical optimal solution
\begin{algorithmic}[1] %[1] enables line numbers 
\STATE Initialize the set of \textit{saturated} objective-functions $\mathcal{A} = \{\}$ and initialize $t=0$ (a step counter).

\STATE increase $t$ ($t = t+1$).

\STATE Use the black-box for $OP1$ to solve the following  problem, where the variables are $x$ (a vector) and $v$ (a scalar): 
\begin{align*}
\max \quad &v\\
        s.t. \quad  & x \in S\\
                    & f_i(x) \geq z_i   & f_i \in \mathcal{A}\\
                    & f_i(x) \geq v   & f_i \notin \mathcal{A}
\end{align*}
Let $x_t$ and $v_t$ be the optimal solution. 
    
\FOR{$f_k \notin \mathcal{A}$}
    \STATE Use the black-box for $OP2$ to solve the following problem, where the variables are $x$ (a vector) and $v$ (a scalar):
    \begin{align*}
    \max \quad & v\\
            s.t. \quad  & x \in S\\
                        & f_i(x) \geq z_i   & f_i \in \mathcal{A}\\
                        & f_i(x) \geq v_t   & f_i \notin \mathcal{A}\\
                        & f_k(x) \geq v
    \end{align*}
    Let $x_t^k$ and $v_t^k$ be the optimal solution. 

    \STATE \textbf{if} $v_t^k = v_t$ \textbf{then} set $f_k$ as \textit{saturated}: add it to $\mathcal{A}$ ($\mathcal{A} = \mathcal{A} \cup \{f_k\}$) and set its value to $v_t$ ($z_k = v_t$).
    % \IF{$z_{max}^k = z_{max}$}
        % \STATE Set $f_k$ as saturated: add it to $\mathcal{A}$ ($\mathcal{A} = \mathcal{A} \cup \{f_k\}$) and set its value to $z_{max}$ ($z_k = z_{max}$).
    % \ENDIF
\ENDFOR
\STATE \textbf{if} $|\mathcal{A}| = n$ \textbf{then} return $x_t$ \textbf{else} Goto line 2.
% \IF{$|\mathcal{A}| = n$}
    % \STATE return $x$ \eden{To myself: the return part of all algorithms should be explain better}
% \ENDIF
\end{algorithmic}
\end{algorithm}

The algorithm keeps a set of objective-functions that are saturated ($\mathcal{A}$) and lower bounds on their values ($\forall f_i \in \mathcal{A} \colon z_i \in \mathbb{R}$). 
The set is initially empty. 
At each iteration, at least one function becomes saturated and its lower bound is set.
When all functions become saturated, the algorithm terminates.
Each iteration of the algorithm can be divided into two parts.
In the first part, the first black-box is used to find the \textit{next max-min} value, which is the maximum value that all functions outside of $\mathcal{A}$ can achieve at the same time, given that all functions within $\mathcal{A}$ achieve their lower bounds.
In the second part, \textit{a saturation test} is made.
% \eden{I think we should name this process, but I'm not sure if it is the best name...}
For every function not in $\mathcal{A}$, the second black-box is used to find the maximum value of this function when all saturated functions ($f_i \in \mathcal{A}$) achieve their lower bounds and all other functions (outside of $\mathcal{A}$) achieve at least the max-min value from the first part.
This value is used to determine if this objective function is saturated, that is, if its maximal value from the saturation test is equal to the max-min value obtained in the first fart.
If so, we add it to the set of saturated objective-functions ($\mathcal{A}$) and set its lower bound to this value.

\section{Failed Attempts to Extend the Saturation Algorithm}

An intuitive idea to extend the  saturation algorithm is to considered an objective function as ”saturated” if its maximum attainable value is
close to the maximum $z_t$.

Consider the following example:
\begin{align*}
    \lexmaxmin \quad &\{f_1(x) = x_1, f_2(x)=x_2\} \\
    s.t. \quad  &(1) \Hquad x_1 + x_2 \leq 1, \quad (2) \Hquad x \in \mathbb{R}^2_{+}
\end{align*}

==> files/proofs/app-proofs.tex <==
\section{Proof of Theorem \ref{th:app-main}}\label{sec:app-sec-proofs}
% \eden{should probably change the title}

% Agents are assumed to care only about their own share (allowing us to use the following abuse of notation in which $u_j$ takes a bundle $b$ of items), their utilities are assumed to be normalized ($u_j(\emptyset) = 0$), monotone ($u_j(b_1) \leq u_j(b_2)$ if $b_1 \subseteq b_2$), and submodular ($u_j(b_1) + u_j(b_2) \geq u_j(b_1 \cup b_2) + u_j(b_1 \cap b_2)$ for any bundles $b_1,b_2$).
% It is assumed that each agent assigns a positive utility to the set of all items.
% The utilities $(u_i)_{i=1}^n$ are assumed to be given in the \emph{value oracle model}, meaning that we do not have a direct access to them, but only to an oracle that indicates the value of an agent from a given simple allocation.
% % \eden{z1 > 0}

This section proves Theorem \ref{th:app-main}:
suppose we are given a randomized algorithm that returns a simple allocation that approximates the utilitarian welfare with multiplicative error $\multError$ (with success probability $p$).
Then, Algorithm \ref{alg:basic-ordered-Outcomes} can be used to obtain a stochastic allocation that approximates leximin with a multiplicative error of at most $\frac{\multError}{1-\multError +\multError^2}$ (with the same probability).

% title: the specific problem as P3
As we saw in Section \ref{sec:algo-short}, an approximation to leximin can be obtained by providing a procedure \textsf{OP} to approximate \eqref{eq:vsums-OP}  (Theorem \ref{th:main}), which, under these particular settings, becomes:
% \erel{Why do you call it "configuration LP"? I think this term refers to something else: \url{https://en.wikipedia.org/wiki/Configuration_linear_program}}
\begin{align}
&\max \quad z_t \quad s.t. \tag{\progAppFirst}\label{eq:app-vsums-OP}\\
& (\text{\progAppFirst.1.1}) \Hquad \sum_{A \in \mathcal{A}} p_d(A) = 1 \nonumber\\
& (\text{\progAppFirst.1.2}) \Hquad p_d(A) \geq 0  && \forall A \in \mathcal{A} \nonumber\\
& (\text{\progAppFirst.2}) \Hquad \ell y_{\ell} - \sum_{j=1}^n m_{\ell,j}\geq \sum_{i=1}^{\ell}  z_i && \forXinY{\ell}{t-1} \nonumber \\
& (\text{\progAppFirst.3}) \Hquad t y_t - \sum_{j=1}^{n} m_{t,j} \geq \sum_{i=1}^{t}  z_i \nonumber \\
& (\text{\progAppFirst.4}) \Hquad m_{\ell,j} \geq y_{\ell} - \sum_{A \in \mathcal{A}}p_d(A) \cdot u_j(A)  && \forXinY{\ell}{t},\Hquad \forXinY{j}{n} \nonumber \\
& (\text{\progAppFirst.5}) \Hquad m_{\ell,j} \geq 0  && \forXinY{\ell}{t},\Hquad \forXinY{j}{n} \nonumber
\end{align}
Here the variables are $p_d(A)$ for any simple allocation $A \in \mathcal{A}$, $\ztVar{}$, and $y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$; and the values $z_1, \ldots z_{t-1}$ are constants.
Notice that it is a \emph{linear program} that has a polynomial number of constraints thanks to \eqref{eq:vsums-OP} representation, but an exponential number of variables (since there is a variable $p_d(A)$ for each simple allocation).
So, it is unclear how to approach it directly in polynomial time.
% \eden{here?}
In addition, it means that the output size is exponential in $n$.
To deal with this issue, the solutions are considered in \emph{sparse form} --- a list of the variables with positive values, along with their values.
Accordingly, if a solution has only a polynomial number of variables with positive values it can be represented by a polynomial size.
We will later see that the procedure described in this section returns such a solution in polynomial time.
% \eden{should write something about the output size, as \cite{kawase_max-min_2020}}

% title: baseline
% \erel{I would move the following paragraph upwards}
With $t=1$, \eqref{eq:app-vsums-OP} can be viewed as the problem of egalitarian welfare maximization, indeed, Kawase and Sumita \cite{kawase_max-min_2020} who studied this problem, considered a slightly simpler representation. 
% After proving that approximating the optimal value to a factor better than $(1-\frac{1}{e})$ is NP-hard, they present a dual-based algorithm that achieves this accuracy \er{w.h.p (?)}.
We now show how their dual-based technique can be applied to approximate \eqref{eq:app-vsums-OP} for any $t\geq 1$ while maintaining the same approximation factor.


To begin, consider the following program \eqref{eq:app-ver2-vsums-OP}, which is the result of modifying \eqref{eq:app-vsums-OP} in three ways. 
First, changing the objective-function to $\min 1/z_t$ instead of $\max z_t$. 
Second, dividing all the constraints by $z_t$ (notice that $z_t > 0$ since $z_t \geq z_1$ for any $t \geq 1$ and  $z_1 >0$).
\eden{to myself: maybe to explain why $z_1>0$}
And third, replacing all the original variables and constants, except $z_t$, with new variables that are smaller by a factor $z_t$ (that is, $p'_A = p_d(A)/z_t$ for all $A \in \mathcal{A}$, $,y'_{\ell} = y_{\ell}/z_t,m'_{\ell,j} = m_{\ell,j}/z_t$ for $\ell \in [t]$ and $ j\in [n]$,  and $z'_i = z_i/z_t$ for $i \in [t-1]$). Notice that the $z'_i$'s are variables (while $z_i$ for $1\leq i\leq t-1$ are constants).

\begin{align}
& \min \quad 1/z_t \quad s.t. \tag{\progAppSecond}\label{eq:app-ver2-vsums-OP}\\
& (\text{\progAppSecond.1.1}) \Hquad \sum_{A \in \mathcal{A}} p'_A = 1/z_t \nonumber\\
& (\text{\progAppSecond.1.2}) \Hquad p'_A \geq 0  && \forall A \in \mathcal{A} \nonumber\\
& (\text{\progAppSecond.2}) \Hquad \ell y'_{\ell} - \sum_{j=1}^n m'_{\ell,j}\geq \sum_{i=1}^{\ell}  z'_i && \forXinY{\ell}{t-1} \nonumber \\
& (\text{\progAppSecond.3}) \Hquad t y'_t - \sum_{j=1}^{n} m'_{t,j} \geq \sum_{i=1}^{t-1}  z'_i + 1 \nonumber \\
& (\text{\progAppSecond.4}) \Hquad m'_{\ell,j} \geq y'_{\ell} - \sum_{A \in \mathcal{A}}p'_A \cdot u_j(A)  && \forXinY{\ell}{t},\Hquad \forXinY{j}{n} \nonumber \\
& (\text{\progAppSecond.5}) \Hquad m'_{\ell,j} \geq 0  && \forXinY{\ell}{t},\Hquad \forXinY{j}{n} \nonumber
\end{align}
The programs \eqref{eq:app-vsums-OP} and \eqref{eq:app-ver2-vsums-OP} are related in the following way:
% \erel{I would make this a lemma:}
\begin{lemma}\label{lemma:bijection}
There exists a bijection mapping each solution of 
\eqref{eq:app-vsums-OP} with objective value $V$ to a unique solution of 
\eqref{eq:app-ver2-vsums-OP} with objective value $1/V$.
\end{lemma}
\begin{proof}
Let $p_d(A)$ for $A \in \mathcal{A}$, $\ztVar{}$, and $y_{\ell}$ and $m_{\ell,j}$ for all $\ell \in [t]$ and $ j\in [n]$ be a feasible solution to the program \eqref{eq:app-vsums-OP} with objective value $V$.
It can be easily verified that $p'_A = p_d(A)/z_t$ for $A \in \mathcal{A}$, $z_t$, $y'_{\ell} = y_{\ell}/z_t$ and $m'_{\ell,j} = m_{\ell,j}/z_t$ for all $\ell \in [t]$ and $ j\in [n]$, and $z'_i = z_i/z_t$ for $i \in [t-1]$ is a feasible solution to the program \eqref{eq:app-ver2-vsums-OP} with objective value $1/V$.

In addition, let $p'_A$ for $A \in \mathcal{A}$, $z_t$, $y'_{\ell}$ and $m'_{\ell,j} = $ for all $\ell \in [t]$ and $ j\in [n]$, and $z'_i$ for $i \in [t-1]$ be a feasible solution to the program \eqref{eq:app-ver2-vsums-OP} with objective value $1/V$.
It can also be easily verified that $ = p_d(A) = p'_A\cdot z_t$ for $A \in \mathcal{A}$, $z_t$, and $ y_{\ell} = y'_{\ell}\cdot z_t$ and $ m_{\ell,j} =m'_{\ell,j}\cdot z_t$ for all $\ell \in [t]$ and $ j\in [n]$ is a feasible solution to the program \eqref{eq:app-vsums-OP} with objective value $V$.
\end{proof}
% \eden{maybe to write something about why it is a bijection (or to write that it is straightforward)}

Denote this bijection by $\Psi$, this also implies the following:
\begin{lemma}\label{lemma:approx-acc-by-bijection}
    If a solution approximates the program \eqref{eq:app-ver2-vsums-OP} with a multiplicative error of $\frac{\multError}{1-\multError}$. Then the corresponding solution to \eqref{eq:app-vsums-OP} according to the bijection $\Psi$ approximates this program with a multiplicative error of $\multError$.
\end{lemma}

\begin{proof}
    Let $V^*$ be the optimal objective value of \eqref{eq:app-vsums-OP}. 
    By Lemma \ref{lemma:bijection}, there exists a solution to \eqref{eq:app-ver2-vsums-OP} with value $1/V^{*}$.
    This solution yields the optimal value for \eqref{eq:app-ver2-vsums-OP} --- if there was a solution that had a value \emph{lower} than $1/V^{*}$ (\eqref{eq:app-ver2-vsums-OP} is a minimization problem), then the corresponding solution to \eqref{eq:app-vsums-OP} (by the bijection $\Psi$) would have a value higher than the optimal value $V^*$.
    Now, let the value of the solution that approximates the program \eqref{eq:app-ver2-vsums-OP} with a multiplicative error of $\frac{\multError}{1-\multError}$ be $1/V$. 
    Since \eqref{eq:app-ver2-vsums-OP} is a minimization problem, assuming that $1/V$ approximates $1/V^*$ with a multiplicative error of $\frac{\multError}{1-\multError}$ means that:
    \begin{align*}
        \frac{1}{V} \leq \left(1+\frac{\multError}{1-\multError}\right)\frac{1}{V^*},
    \end{align*}
 which implies that $V \geq (1-\multError)V^*$.
    As \eqref{eq:app-vsums-OP} is a maximization problem, this means that $V$ approximates this problem with multiplicative error $\multError$.
    By Lemma \ref{lemma:bijection}, $V$ is the value of the corresponding solution to \eqref{eq:app-vsums-OP} by the bijection $\Psi$.
\end{proof}

Notice that the variable $z_t$ appears only in the objective function of \eqref{eq:app-ver2-vsums-OP}, $\min 1/z_t$, and in constraint (\progAppSecond.1.1), which says that $\sum_{A \in \mathcal{A}}p'_A = 1/z_t$.
As a result, we can reduce the need for the variable $z_t$ by removing constraint (\progAppSecond.1.1) and changing the objective function to $\min \sum_{A \in \mathcal{A}}p'_A$.
This change makes \eqref{eq:app-ver2-vsums-OP} a \emph{linear} program.
This will allow us to approximate it using its dual, as we will see.

The following observation will be useful later:
\begin{observation}\label{obs:c2-to-c1-in-poly-time}
    If a solution to \eqref{eq:app-ver2-vsums-OP} is given in a sparse form --- a list of the variables with nonzero value and their values, then the corresponding solution to \eqref{eq:app-vsums-OP} in a sparse form can be computed in time polynomial to the number of nonzero variables.
\end{observation}
\noindent For completeness, we briefly outline the process. 
When given a list of variables with nonzero values, we first iterate the list and sum all variables of the form $p'_A$, and then set $z_t$ to be $1$ divided by this sum. 
After, for each variable $\nu'$ in the list, we set the corresponding variable, $\nu$, to $z_t \cdot \nu'$.


% title: dual 
Now, let us consider the dual program of \eqref{eq:app-ver2-vsums-OP}, which can be described as follows:
% \erel{When you present an LP, it can help the reader if you mention what exactly the variables of the LP are.}
\begin{align}
    \max &&& \sum_{\ell=1}^{t-1} q_{\ell} \sum_{i=1}^{\ell} z_i + q_t (\sum_{i=1}^{t-1} z_i +1) \tag{\progAppDual}\label{eq:app-dual}\\
        s.t. &&& (\text{\progAppDual.1}) \Hquad \sum_{j=1}^n u_j(A) \sum_{\ell=1}^t v_{\ell,j} \leq 1  && \forall A \in \mathcal{A} \nonumber\\
                    &&& (\text{\progAppDual.2}) \Hquad \ell q_{\ell} - \sum_{j=1}^n v_{\ell,j} = 0 && \forXinY{\ell}{t} \nonumber \\
                    &&& (\text{\progAppDual.3}) \Hquad q_{\ell} - v_{\ell,j} \leq 0  && \forXinY{\ell}{t},\Hquad \forXinY{j}{n} \nonumber \\
                    &&& (\text{\progAppDual.4}) \Hquad v_{\ell,j} \geq 0  && \forXinY{\ell}{t},\Hquad \forXinY{j}{n} \nonumber \\
                    &&& (\text{\progAppDual.5}) \Hquad q_{\ell} \geq 0  && \forXinY{\ell}{t} \nonumber
\end{align}
Here, the variables are $q_{\ell}$ and $v_{\ell,j}$ for any $\ell \in [t]$ and $j \in [n]$; and the constants are (as before) $z_i$ for $i \in [t-1]$.
Recall that $u_j(A)$ is the utility that agent $j$ assigns to simple allocation $A$, as given by the value oracle.
% title: ellipsoid variant
This problem has an exponential number of constraints --- a constraint for each allocation (in line (\progAppDual.1)) but only a polynomial number of variables.
Using the ellipsoid method \cite{grotschel_ellipsoid_1981}, it could be solved in polynomial time 
if we had a \emph{separation oracle} ---
an oracle that given a vector $\upsilon$ either determines that $\upsilon$ is infeasible and returns a violated constraint, or asserts that $\upsilon$ is feasible.
Unfortunately, as we shall now see, it is NP-hard to compute a separation oracle to this problem.
\begin{lemma}
    Computing a separation oracle to \eqref{eq:app-dual} is NP-hard.
\end{lemma}

% very similar to what they did in yonatan's paper..
\begin{proof}
We prove that a separation oracle for \eqref{eq:app-dual} would allow us to compute a leximin optimal stochastic allocation.
    As discussed previously, computing such an allocation is NP-hard, so the same applies for computing a separation oracle for \eqref{eq:app-dual}.

    First, we prove that such a separation oracle can be used to extract an optimal solution to \eqref{eq:app-ver2-vsums-OP}.
    Assume that the ellipsoid method was operated with the given oracle to solve \eqref{eq:app-dual}.
    Let $C$ be the set of constraints that the oracle determined as being violated.
    Since the ellipsoid method operates in polynomial time, the size of the set $C$ is also polynomial.
    Let $V_C$ be the set of variables of \eqref{eq:app-ver2-vsums-OP} associated with the constraints in $C$.
    By complementary slackness, the variables in $V_C$ are the only ones that may get a \emph{positive} value in the corresponding optimal solution to \eqref{eq:app-ver2-vsums-OP}.
    Therefore, the program \eqref{eq:app-ver2-vsums-OP} with only the variables in $V_C$ (and the other variables equal to zero) has a polynomial size, and therefore can be solved exactly.


    But, by Observation \ref{obs:c2-to-c1-in-poly-time}, this would allow us to find the corresponding optimal solution to \eqref{eq:app-vsums-OP} in polynomial time.
    % \erel{Did we say that $\psi$ can be computed in polynomial time?}\eden{in the way it is written now is not, it iterate over each variable of \eqref{eq:app-vsums-OP} and there are exponential number of them. I need to think how to write it appropriately. maybe "that can be computed in time equals to the number of positive variables"?}
    % \erel{If it is not polynomial, then the reduction is not polynomial, so it does not imply NP-hardness}
    This means the described process can be used as an approximation procedure to \eqref{eq:vsums-OP} (that became \eqref{eq:app-vsums-OP} under the settings of this problem) with $\multError = \additiveError = 0$.
    Therefore, by Theorem \ref{th:main}, this means we can use Algorithm \ref{alg:basic-ordered-Outcomes} to obtain a leximin optimal solution\footnote{Actually, Theorem \ref{th:main} says that Algorithm \ref{alg:basic-ordered-Outcomes} will output a $(1,0)$-leximin-approximation; But Lemma \ref{lemma:absence-of-errors} says that such a solution is, indeed, a leximin optimal solution.}.
\end{proof}


% --- it would allow us to compute a leximin optimal stochastic allocation, which is, as discussed previously, NP-hard.

In Appendix \ref{sec:mult-variant-ellipsoid}, we present another variant of the ellipsoid method, which allows us to approximate the program \eqref{eq:app-ver2-vsums-OP} given a \emph{half-randomized approximate separation oracle} to \eqref{eq:app-dual}.
That is, an oracle that, given a multiplicative error $\multError$, a success probability $p$, and a vector $\upsilon$, either determines that $\upsilon$ is infeasible and returns a violated constraint; or determines that $\upsilon$ is $\multError$-\textit{approximately-feasible}, which means that for any constraint $a \cdot x \leq b$, the vector $\upsilon$ satisfies $a \cdot \upsilon \leq (1+\multError)\cdot b$.
When the oracle says that $\upsilon$ is $\multError$-approximately-feasible, it is correct with probability at least $p$.
Given such an oracle for the dual program, the ellipsoid method variant can be used to output a solution to the primal, that approximates it to the same factor with probability at least $p^I$, where $I$ is an upper bound on the number of iterations in any execution of the ellipsoid method variant on the dual (if it is given a deterministic oracle).
We can therefore conclude the following result:
\begin{lemma}\label{lemma:approx-sep-oracle-to-goal}
    Given a half-randomized approximate separation oracle to the problem \eqref{eq:app-dual}, with a multiplicative error of $\frac{\beta}{1-\beta}$ and a success probability $p$, a stochastic allocation that approximates leximin to a multiplicative error $\frac{\multError}{1-\multError+\multError^2}$ can be obtained with probability $p^{nI}$.
\end{lemma}

\begin{proof}
    % To begin, assume that we are given a deterministic approximate separation oracle (i.e., with failure probability $p=0$).
    As described above, we can use the ellipsoid method variant of Appendix \ref{sec:mult-variant-ellipsoid} with the given oracle to \eqref{eq:app-dual} to obtain a solution to \eqref{eq:app-ver2-vsums-OP},  that approximates it with a multiplicative error of $\frac{\multError}{1-\multError}$ with probability $p^I$.
    Then, by Observation \ref{obs:c2-to-c1-in-poly-time}, this would allow us to find the corresponding solution to \eqref{eq:app-vsums-OP}, that, with probability $p^I$, approximates it with a multiplicative error of $\multError$.
    That is, the described process can be used as a randomized approximation procedure to \eqref{eq:vsums-OP} (that became \eqref{eq:app-vsums-OP} under the settings of this problem).
    % with $\multError = \additiveError = 0$.
    Therefore, by Theorem \ref{th:main}, Algorithm \ref{alg:basic-ordered-Outcomes} can be used to obtain a leximin approximation to the original problem with only a multiplicative error of $\frac{\multError}{1-\multError+\multError^2}$ with probability $p^{nI}$ (Corollary \ref{corollary:main-with-probability}).
\end{proof}

Now, we show that such an oracle can be designed given a randomized approximation algorithm for computing a simple allocation that approximates the utilitarian welfare. Specifically, 

\begin{lemma}\label{lemma:alg-for-utilitarian-to-sep-oracle}
    Given a randomized approximation algorithm for computing a simple allocation that approximates the utilitarian welfare with multiplicative error $\multError$ and a success probability $p$, a half-randomized approximate separation oracle to \eqref{eq:app-dual} can be designed with a multiplicative error of $\frac{\beta}{1-\beta}$ and a success probability at least $\left(1-\frac{1}{nI}(1-p)\right)$.
\end{lemma}

% \eden{should say somewhere that the oracle is polynomial time and therefore everything is?...}
% FROM HERE: https://tex.stackexchange.com/a/675333/20929
\algdef{SE}[REPEATN]{REPEATN}{ENDREP}[1]{\algorithmicrepeat\ #1 \textbf{times}}{\algorithmicend\ \algorithmicrepeat}
\begin{algorithm}[!tbp]
\caption{A Half-Randomized Approximate Separation Oracle to \eqref{eq:app-dual}}
\label{alg:sep-oracle}
INPUT: variables $q_{\ell}$ and $v_{\ell,j}$ for any $\ell \in [t]$ and $j \in [n]$, an $\multApprox$-approximation algorithm for the utilitarian welfare problem (\eqref{eq:utilitarian}) with success probability $p$.
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Iterate over constraints (\progAppDual.2)-(\progAppDual.5). If one of them is  violated, stop and return it.
\STATE \textbf{If} $p=1$ then set $T:=1$; \textbf{else} set $T := 1 + \lceil-\log_{(1-p)}(nI)\rceil$.

\REPEATN{$T$}
    \STATE Operate the algorithm for the utilitarian welfare problem on $n,m,(u'_j)_{j=1}^n$ to obtain an allocation $\Tilde{A}$ with value $\nu$.
    \IF{$\nu > 1$}  
        \STATE Return the corresponding violated constraint $\sum_{j=1}^n u_j(\Tilde{A}) \sum_{\ell=1}^t v_{\ell,j} > 1$
    \ENDIF
\ENDREP
\STATE Return "the assignment is approximately-feasible".

\end{algorithmic}
\end{algorithm}


Algorithm \ref{alg:sep-oracle} describes the oracle.
It accepts as input an assignment to the variables of \eqref{eq:app-dual}, that is, $q_{\ell}$ and $v_{\ell,j}$ for any $\ell \in [t]$ and $j \in [n]$, and an algorithm for approximating the maximum utilitarian welfare.
It starts by verifying constraints (\progAppDual.2)-(\progAppDual.5) one by one (this is possible as their number is polynomial in $n$ and $m$). 
If a violated constraint was found, the oracle simply returns it. Otherwise, it proceeds to check constraints (\progAppDual.1).
Although the number of constraints described by (\progAppDual.1) is exponential in $n$, they can be treated collectively in polynomial time (as in \cite{kawase_max-min_2020}).
% \eden{here maybe to say something about the randomness}.\erel{Maybe mention that \textcite{kawase_max-min_2020} ignored this issue.}
First, notice that in order to determine whether the expression $\sum_{j=1}^n u_j(A) \sum_{\ell=1}^t v_{\ell,j}$ is at most $1$ for all simple allocations ($A \in \mathcal{A}$), it is sufficient to check the allocation that maximizes this expression and compare it to $1$.
Define new utility functions for all $j \in [n]$ and $A \in \mathcal{A}$, 
\begin{align*}
u'_j(A) := \sum_{\ell=1}^t v_{\ell,j} \cdot u_j(A) 
\end{align*}
The above expression can be simplified to $\sum_{j=1}^n u'_j(A)$. An allocation that maximizes this expression is an allocation that maximizes the utilitarian welfare (i.e., the sum of utilities) when the same sets of agents and items is considered but with different utilities%
\footnote{Notice that the utilities $u'_j$ are  normalized, monotone, submodular, and can be computed using $t\leq n$ calls to the value oracle of $u_j$}
($u'_j$ instead of $u_j$ for $j \in [n]$).
Such an allocation cannot be found in polynomial time since approximating the utilitarian welfare up to a factor better than $(1-\frac{1}{e})$ in the case of submodular utilities is known to be NP-hard \cite{khot_inapproximability_2008}.
However, the oracle is given an approximation algorithm to the utilitarian welfare problem as input.
Therefore, an allocation $\Tilde{A}$ with utilitarian value at least $(1-\multError)$ of the optimal can be obtained with probability $p$.
We shall now see that it is enough.


\begin{proof}[Proof of Lemma \ref{lemma:alg-for-utilitarian-to-sep-oracle}]
First, observe that when Algorithm \ref{alg:sep-oracle} returns a violated constraint, it is always correct.
This is obvious for constraints described by (\progAppDual.2)-(\progAppDual.5), since these constraints have been verified directly.
For constraints described by (\progAppDual.1), it means that the algorithm found an allocation $\Tilde{A}$ that satisfies $\sum_{j=1}^n u'_j(\Tilde{A}) > 1$.
    By the definition of $u'$, the constraint corresponding to this allocation is, indeed, violated:
    \begin{align*}
         \sum_{j=1}^n u_j(\Tilde{A}) \sum_{\ell=1}^t v_{\ell,j} = \sum_{j=1}^n u'_j(\Tilde{A}) > 1.
    \end{align*}
Let us assume that the given algorithm for the utilitarian welfare problem is deterministic (i.e., $p=1$) and then revisit the case $p<1$.
    Assume that the oracle said that the assignment is approximately-feasible.
    This means that the algorithm for the utilitarian welfare problem found an allocation $\Tilde{A}$ with value at most $1$.
    Since $\Tilde{A}$ is approximately-optimal, the optimal utilitarian value is at most $1/(1-\multError)\cdot 1$.
    As this is an upper bound of the utilitarian value of any allocation, it follows that all the constraints described bu (\progAppDual.1) are $\frac{\multError}{1-\multError}$-approximately maintained --- that is, for any allocation $A \in \mathcal{A}$ the following holds:
    \begin{align*}
        \sum_{j=1}^n u'_j(A) = \sum_{j=1}^n u_j(A) \sum_{\ell=1}^t v_{\ell,j} \leq \frac{1}{1-\multError}\cdot 1 = \left(1+\frac{\multError}{1-\multError}\right)\cdot1
    \end{align*}
    We get that, in this case, the oracle is also deterministic, and that the success probability is at least $\left(1-\frac{1}{nI}(1-p)\right) = 1$ for $p=1$.

    Assume now that $p<1$. Then, the oracle may be incorrect when it says the assignment is approximately feasible, but only if the algorithm for the utilitarian welfare problem did not return an appropriate approximation in all $T = \lceil-\log_{(1-p)}(nI)\rceil + 1$ operations, that is, with probability at most $(1-p)^T$.
    % as each operation of the oracle is independent
    Notice that $T>1$ since $\log_{(1-p)}(nI) < 0$\footnote{
    % The fact that  $\log_{(1-p)}(nI) < 0$ can be easily concluded 
    Since $(1-p)\in(0,1)$ and $nI>1$ by change of base: $\log_{(1-p)}(nI) = \log(nI)/\log(1-p)$, the numerator is positive and the denominator is negative.}.
    Now, as $T \geq -\log_{(1-p)}(nI) + 1$ and $(1-p)<1$ we get that:
    \begin{align*}
        &(1-p)^T \leq (1-p)\cdot(1-p)^{-\log_{(1-p)}(nI)} = (1-p)(nI)^{-1}
    \end{align*}
    So, the success probability is at least $\left(1-\frac{1}{nI}(1-p)\right)$.
\end{proof}

We can now prove Theorem \ref{th:app-main}.

\begin{proof}[Proof of Theorem \ref{th:app-main}]
    Assume we are given an algorithm that returns a simple allocation that approximates the utilitarian welfare with multiplicative error $\multError$ with success probability $p$.
    By Lemma \ref{lemma:alg-for-utilitarian-to-sep-oracle} this algorithm can be used to obtain an half-randomized approximate separation oracle to \eqref{eq:app-dual} with a multiplicative error $\frac{\multError}{1-\multError}$ with success probability $\left(1-\frac{1}{nI}(1-p)\right)$.
    By Lemma \ref{lemma:approx-sep-oracle-to-goal}, with such an oracle a stochastic allocation that approximates leximin to a multiplicative error of $\frac{\multError}{1-\multError+\multError^2}$ can be obtained with probability $\left(1-\frac{1}{nI}(1-p)\right)^{nI}$.
    If $p=1$ then the success probability is $1$ too (at least $\left(1-\frac{1}{nI}(1-p)\right)^{nI}= 1$).
    However, if $p<1$, then $\frac{1}{nI}(1-p) \in (0,1)$ and therefore the success probability is at least $p$\footnote{For any $\epsilon \in (0,1)$ and $k \in \mathbb{Z}_{+} \colon \Hquad (1 - \epsilon)^k \geq 1 - k \cdot \epsilon$}:
    \begin{align*}
        \left(1-\frac{1}{nI}(1-p)\right)^{nI} \geq \left(1-nI\cdot\frac{1}{nI}(1-p)\right) = p.   \end{align*}
\end{proof}

